NPASA: An algorithm for nonlinear programming -- Local Convergence

In this paper, we provide local convergence analysis for the two phase Nonlinear Polyhedral Active Set Algorithm (NPASA) designed to solve nonlinear programs. In particular, we establish local quadratic convergence of the primal iterates and global error estimator for NPASA under reasonable assumptions. Additionally, under the same set of assumptions we prove that only phase two of NPASA is executed after finitely many iterations. This paper is companion to a paper that provides motivation and global convergence analysis for NPASA.

==> local-phase-one.tex <==
\section{Convergence Analysis for Phase One of NPASA} \label{section:npasa-phase-one}
We begin our convergence analysis by providing a detailed discussion and analysis for phase one of NPASA. Motivation for the global step in phase one is to ensure the robustness of the NPASA algorithm. In particular, phase two of NPASA may encounter problems when the linearization of $\bm{h} (\bm{x})$ at the current iterate requires a large perturbation to be feasible resulting in an unsuccessful minimization of $\| \bm{h} (\bm{x}) \|$ in the Constraint Step. For phase one we have decided to use augmented Lagrangian techniques. First introduced by Hestenes \cite{Hestenes1969} and Powell \cite{Powell1969} and sometimes referred to as the method of multipliers, augmented Lagrangian methods and their convergence properties have since been well studied \cite{bertsekas1995nonlinear, Luo2008, NandW} and have been successful at solving nonlinear programs in practice using software packages such as ALGENCAN \cite{Andreani2008}, ALGLIB \cite{Bochkanov1999}, LANCELOT \cite{Conn1991, Conn2010}, and MINOS \cite{Murtagh1978}. Hence, the choice of an augmented Lagrangian technique is a suitable safeguard to ensure NPASA will converge to a stationary point in the case that problems arise during the constraint step in phase two.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
First, we provide a brief discussion on the multiplier updates given in lines 4 and 5 of the GS pseudocode, Algorithm~\ref{alg:gs}, and the criterion for branching from phase one to phase two in NPASA, Algorithm~\ref{alg:npasa}. Consider the original problem in the form
\begin{align}
&\min_{\bm{x} \in \mathbb{R}^{n}} \hspace{20mm} f(\bm{x}) \nonumber \\
&\ \ \text{s.t.} \ \ \ \ \ \ \ \bm{h}(\bm{x}) = \bm{0}, \ \bm{r} (\bm{x}) \leq \bm{0} \label{prob:phase-one}
\end{align}
which has the Lagrangian function given by $\mathcal{L} (\bm{x}, \bm{\lambda}, \bm{\mu}) = f (\bm{x}) + \bm{\lambda}^{\intercal} \bm{h} (\bm{x}) + \sum_{i = 1}^{m} \mu_i r_i (\bm{x})$. By adding a slack variable, $\bm{z}$, we can reformulate the inequality constraints as equality constraints to obtain the equivalent problem
\begin{align}
&\min_{\bm{x} \in \mathbb{R}^{n}, \bm{z} \in \mathbb{R}^m} \hspace{20mm} f(\bm{x}) \nonumber \\
&\ \ \ \ \ \text{s.t.} \ \ \ \ \ \ \ \bm{h}(\bm{x}) = \bm{0}, \ \bm{r} (\bm{x}) + \bm{z} = \bm{0}, \ \bm{z} \geq \bm{0}. \label{prob:phase-one-slack}
\end{align}
Using Rockafellar's augmented Lagrangian function \cite{Rockafellar1974} for this problem we have
\begin{align*}
\mathcal{L}_q (\bm{x}, \bm{z}, \bm{\lambda}, \bm{\mu}) = f (\bm{x}) + \bm{\lambda}^{\intercal} \bm{h} (\bm{x}) + q \| \bm{h} (\bm{x}) \|^2 + \sum_{i = 1}^{m} \left( \mu_i (r_i (\bm{x}) + z_i ) + q | r_i (\bm{x}) + z_i |^2 \right)
\end{align*}
The first step of the method of multipliers is to fix $\bm{\lambda}$ and $\bm{\mu}$ and minimze over the primal variables $\bm{x}$ and $\bm{z}$. Now suppose we have a current guess for the multipliers $\bm{\lambda}_k$ and $\bm{\mu}_k$ and we compute $\bm{\bar{\lambda}}_k = Proj_{[-\bar{\lambda}, \bar{\lambda}]} (\bm{\lambda}_k)$ and $\bm{\bar{\mu}}_k = Proj_{[0, \bar{\mu}]} (\bm{\mu}_k)$ where $\bar{\lambda}$ and $\bar{\mu}$ are nonnegative scalars. Now taking $\bm{\lambda} = \bm{\bar{\lambda}}_k$, $\bm{\mu} = \bm{\bar{\mu}}_k$ this yields the problem 
\begin{align*}
&\min_{\bm{z} \geq \bm{0}, \ \bm{x}} \quad \mathcal{L}_q (\bm{x}, \bm{z}, \bm{\bar{\lambda}}_k, \bm{\bar{\mu}}_k).
\end{align*}
By the definition of $\mathcal{L}_q (\bm{x}, \bm{z}, \bm{\lambda}, \bm{\mu})$, minimizing over $\bm{z} \geq \bm{0}$ with $\bm{x}$ fixed amounts to solving
\begin{align*}
\min_{z_i \geq 0} \quad \bar{\mu}_{k,i} (r_i (\bm{x}) + z_i ) + q | r_i (\bm{x}) + z_i |^2,
\end{align*}
for $1 \leq i \leq m$. As each of these problems is minimization of a quadratic function with a single nonnegative decision variable, we can derive a closed form expression of the minimizer in terms of $\bm{x}$ which is given by
\begin{align*}
z_i^* = \max \left\{ 0, - \frac{\bar{\mu}_{k,i}}{2 q} - r_i (\bm{x}) \right\},
\end{align*}
for $1 \leq i \leq m$. Substituting the vector $\bm{z}^*$ into the augmented lagrangian simplifies the problem to minimization over $\bm{x}$ as
\begin{align}
&\min_{\bm{x}} \quad \mathcal{L}_q (\bm{x}, \bm{z}^*, \bm{\bar{\lambda}}_k, \bm{\bar{\mu}}_k) \label{prob:phase-one.1},
\end{align}
where we can express
\begin{align*}
\mathcal{L}_q (\bm{x}, \bm{z}^*, \bm{\bar{\lambda}}_k, \bm{\bar{\mu}}_k) = f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \bm{h} (\bm{x}) + q \| \bm{h} (\bm{x}) \|^2 + \frac{1}{4q} \sum_{i = 1}^{m} \left( \left( \max \{ 0, \bar{\mu}_i  + 2 q r_i (\bm{x}) \} \right)^2 - \bar{\mu}_i^2 \right)
\end{align*}
after some simplification. Now suppose that $\bm{x}_{k+1}$ is a local minimizer for problem (\ref{prob:phase-one.1}). As this is an unconstrained minimization problem, the first order optimality conditions yield that $\nabla_x \mathcal{L}_q (\bm{x}, \bm{z}^*, \bm{\bar{\lambda}}_k, \bm{\bar{\mu}}_k) = \bm{0}$, or equivalently
\begin{align*}
\nabla_x f (\bm{x}_{k+1}) + \left( \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}_{k+1}) \right)^{\intercal} \nabla_x \bm{h} (\bm{x}_{k+1}) + \sum_{i = 1}^{m} \max \{ 0, \bar{\mu}_{k,i} + 2 q r_i (\bm{x}_{k+1}) \} \nabla_x r_i (\bm{x}_{k+1}) = \bm{0}. %\label{eq:phase-one.1}
\end{align*}
Recalling the Lagrangian function for problem (\ref{prob:phase-one}), by setting
\begin{align}
\begin{array}{rcl}
\bm{\lambda}_{k+1} &=& \bm{\bar{\lambda}}_k + 2 q \bm{h}(\bm{x}_{k+1}), \vspace{2mm} \\
\mu_{k+1,i} &=& \max \left\{ 0, \bar{\mu}_{k,i} + 2 q r_i (\bm{x}_{k+1}) \right\}, \ \text{for} \ 1 \leq i \leq m,
\end{array} \label{eq:safeguarding-MoM}
\end{align}
it now follows that $\nabla_x \mathcal{L} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1}) = \bm{0}$. Also, by our choice of $\bm{\mu}_{k+1}$ we have that $\bm{\mu}_{k+1} \geq \bm{0}$. Next, we check if the complimentarity condition $\mu_{k+1, i} r_i (\bm{x}_{k+1}) = 0$ holds, for $1 \leq i \leq m$. Recalling the slack version of the problem in (\ref{prob:phase-one-slack}) and our solution for the slack variable $\bm{z}^*$, we have that the active and inactive sets for problem (\ref{prob:phase-one}) can be expressed as $\mathcal{A} = \{ i \in \mathbb{N} : z_i^* = 0 \}$ and $\mathcal{I} = \{ i \in \mathbb{N} : z_i^* = - \frac{\bar{\mu}_i}{2 q} - r_i (\bm{x}) \}$, respectively. Clearly, if $i \in \mathcal{A}$ then $\mu_{k+1, i} r_i (\bm{x}_{k+1}) = 0$. On the other hand, if $i \in \mathcal{I}$ then by the definition of $z_i^*$ we have that $\frac{\bar{\mu}_i}{2 q} + r_i (\bm{x}) < 0$, or equivalently $\bar{\mu}_i + 2 q r_i (\bm{x}) < 0$. By our choice of $\mu_{k+1,i}$ it follows that $\mu_{k+1,i} = 0$ which in turn yields that $\mu_{k+1, i} r_i (\bm{x}_{k+1}) = 0$. Hence, we have that complimentary slackness holds at $(\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1})$ provided that $\bm{r} (\bm{x}_{k+1}) \leq \bm{0}$. 

To ensure that the constraint $\bm{r} (\bm{x}_{k+1}) \leq \bm{0}$ is satisfied, we can instead solve the constrained augmented Lagrangian problem
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x} \in \mathbb{R}^{n}} & \displaystyle f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \bm{h} (\bm{x}) + q \| \bm{h} (\bm{x}) \|^2 + \frac{1}{4q} \sum_{i = 1}^{m} \left( \left( \max \{ 0, \bar{\mu}_i  + 2 q r_i (\bm{x}) \} \right)^2 - \bar{\mu}_i^2 \right) \vspace{2mm} \\
\text{s.t.} & \bm{r} (\bm{x}) \leq \bm{0}
\end{array} \label{prob:aug-lag}
\end{align}
then perform the same updates for $\bm{\lambda}_{k+1}$ and $\bm{\mu}_{k+1}$ given in (\ref{eq:safeguarding-MoM}). Using this formulation, if $\bm{x}_{k+1}$ is a minimizer for problem (\ref{prob:aug-lag}) and $\mathcal{L} (\bm{x}, \bm{\lambda}, \bm{\mu})$ denotes the Lagrangian of problem (\ref{prob:phase-one}) then the iterate $(\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1})$ satisfies all of the following:
\begin{enumerate}
\item[(L.1)] Gradient of Lagrangian equals zero: $\nabla_x \mathcal{L} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1}) = \bm{0}$
\item[(L.2)] Satisfies inequality constraints: $\bm{r} (\bm{x}_{k+1}) \leq \bm{0}$
\item[(L.3)] Nonnegativity of inequality multipliers: $\bm{\mu}_{k+1} \geq \bm{0}$
\item[(L.4)] Complimentary slackness: $\mu_{k+1,i} r_i (\bm{x}_{k+1}) = 0$, for $1 \leq i \leq m$.
\end{enumerate}
Hence, the KKT conditions nearly hold at $(\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1})$ where the only possible violation is that the equality constraints, $\bm{h} (\bm{x}_{k+1}) = \bm{0}$, may not be satisfied. In such an instance, we would like to focus on minimizing the constraint violation while maintaining a relatively low multiplier error which is what phase two of NPASA is designed to accomplish. With this is mind, we now provide justification for the criterion used to branch from phase one to phase two in line 11 of Algorithm~\ref{alg:npasa}. From (L.1) and (L.4) it follows that
\begin{align*}
E_{m,0} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1})^2 = \| \nabla_x \mathcal{L} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1}) \|^2 - \bm{\mu}_{k+1}^{\intercal} \bm{r} (\bm{x}_{k+1}) = \bm{0}
\end{align*}
which implies that the branching criterion given by $E_{m,1} (\bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1}) \leq \theta E_c (\bm{x}_{k+1})$ will always be satisfied when the augmented Lagrangian problem in (\ref{prob:aug-lag}) is solved exactly. In particular, in iterations where the constraint error is nonzero the branching criterion allows us to solve the augmented Lagrangian problem inexactly with the goal of acheiving a balanced reduction of the constraint and multiplier errors in phase two. Once in phase two, the constraint step works to reduce the inequality constraint violation by taking a more agressive approach that has faster local convergence than the augmented Lagrangian method. %Additionally, in phase two the constraint and multiplier steps attempt to attain a balanced reduction of the constraint and multiplier error, respectively.
We now provide a result on convergence for this approach to solving phase one. 

\begin{theorem} \label{thm:rockafellar-aug-lag}
Suppose that $\Omega$ is compact and that $f, \bm{h} \in \mathcal{C}^1 (\Omega)$. Suppose that the following are satisfied:
\begin{enumerate}
\item $\{ \bm{x}_k \}_{k=0}^{\infty}$ is a sequence with $\bm{x}_k \in \Omega$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq \theta E_c (\bm{x}_k)$, for all $k \geq 0$
\item $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}_k \}_{k=0}^{\infty}$ are updated using the formulas in (\ref{eq:safeguarding-MoM})
\item $\{ q_k \}_{k=0}^{\infty}$ is a sequence of real numbers such that $q_k \to \infty $ as $k \to \infty$.
\end{enumerate}
Then any subsequence of $\{ \bm{x}_k \}_{k=0}^{\infty}$ with limit point $\bm{x}^*$ such that assumption (\textbf{LI}) holds at $\bm{x}^*$ satisfies $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*) = E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*) = 0$, where $\bm{\lambda}^*$ and $\bm{\mu}^*$ are the limits of the corresponding subsequences for $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}_k \}_{k=0}^{\infty}$.
\end{theorem}
\begin{proof}
First, we note that the safeguarding update $\mu_{k+1,i} = \max \{ 0, \bar{\mu}_{k,i} + 2 q_k r_i (\bm{x}_{k+1}) \}$, where $\bar{\mu}_{k,i}$ denotes the projection of $\mu_{k,i}$ onto the interval $[0, \bar{\mu}]$, results in the sequence $\{ \bm{\mu}_k \}_{k=0}^{\infty}$ being uniformly bounded. This follows since for each $\bm{x}_k$ we have $r_i (\bm{x}_k) \leq 0$ which yields that
\begin{align*}
\mu_{k+1,i} = \max \{ 0 , \bar{\mu}_{k,i} + 2 q_k r_i (\bm{x}_{k+1}) \}
\leq \max \{ 0 , \bar{\mu} \}.
\end{align*}
Hence $\| \bm{\mu}_k \| \leq \| \bar{\mu} \bm{1} \|$. Next, by our hypothesis that $E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq \theta E_c (\bm{x}_k)$, we have that
\begin{align*}
\| \nabla_x \bm{h} (\bm{x}_k)^{\intercal} \bm{\lambda}_k \| \leq \| \nabla f (\bm{x}_k) + \bm{\mu}_k^{\intercal} \nabla \bm{r} (\bm{x}_k) \| + \sqrt{E_c (\bm{x}_k) + \bm{\mu}_k^{\intercal} \bm{r} (\bm{x}_k)}.
\end{align*}
Now let $\{ \bm{x}_k \}_{k=0}^{\infty}$ denote a subsequence with limit point $\bm{x}^*$ such that (\textbf{LI}) holds at $\bm{x}^*$. As $\{ \bm{\mu}_k \}_{k=0}^{\infty}$ is uniformly bounded, it now follows that $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ is uniformly bounded for $k$ sufficiently large. As the sequence $\{ \bm{\bar{\lambda}}_k \}_{k=0}^{\infty}$ is uniformly bounded by construction, there exists a constant $\Lambda$ such that $\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \| \leq \Lambda$ for all $k$ sufficiently large. Now using the update formula $\bm{\lambda}_{k} = \bm{\bar{\lambda}}_{k-1} + 2 q_k \bm{h} (\bm{x}_{k})$, we have that
\begin{align}
\| \bm{h} (\bm{x}_{k}) \| 
= \frac{\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \|}{2 q_k} 
\leq \frac{\Lambda}{2 q_k}, \label{eq:rockafellar-aug-lag.1}
\end{align}
for all $k$ sufficiently large. So (\ref{eq:rockafellar-aug-lag.1}) together with the hypothesis that $q_k \to \infty$ as $k \to \infty$, yields that
\begin{align*}
\lim_{k \to \infty} E_c (\bm{x}_{k}) = \lim_{k \to \infty} \| \bm{h} (\bm{x}_{k}) \|^2 \leq \lim_{k \to \infty} \frac{\Lambda^2}{4 q_k^2} = 0.
\end{align*}
Now as $E_0 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) = E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) + E_c (\bm{x}_k)$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq \theta E_c (\bm{x}_k)$ for all $k$ by hypothesis, it now follows that $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*) = 0$. Lastly, from Lemma~\ref{lem:E0-E1-relationship} we have that $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*) = 0$ which concludes the proof.
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%Unfortunately, one drawback to solving problem (\ref{prob:aug-lag}) is that the objective function is not twice continuously differentiable everywhere which restricts our approach for solving this problem to first order methods. There is a large body of literature in which alternative augmented Lagrangian methods have been developed where the objective function is twice continuously differentiable \cite{Birgin2005,bertsekas1995nonlinear}, however, we propose an approach that yields an alternative formula for the inequality multipliers $\bm{\mu}_{k}$. To this end, 
Consider the problem given by
\begin{align}
&\min_{\bm{x} \in \mathbb{R}^{n}} \quad \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) = f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \bm{h} (\bm{x}) + q \| \bm{h} (\bm{x}) \|^2 \nonumber \\
&\ \ \text{s.t.} \qquad \qquad \qquad \qquad \bm{r}(\bm{x}) \leq \bm{0} \label{prob:aug-lag-mod}
\end{align}
where $\bm{r} (\bm{x}) = \bm{A} \bm{x} - \bm{b}$ is the linear function from problem (\ref{prob:main-nlp}). %This is similar to problem (\ref{prob:aug-lag}) except we have removed the penalty and Lagrangian terms from the objective corresponding to the inequality multipliers. %As $\bm{r} (\bm{x})$ is a linear function, say $\bm{r} (\bm{x}) = \bm{A} \bm{x}$, 
We can solve this problem using the algorithm PASA \cite{HagerActive}. Note that if PASA converges to a stationary point $\bm{x}_{k+1}$ then by the KKT conditions there exists a $\bm{\mu}_{k+1} \geq \bm{0}$ such that
\begin{align*}
\bm{0} 
&= \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) + \bm{\mu}_{k+1}^{\intercal} \bm{A} \\
&= \nabla f (\bm{x}_{k+1}) + (\bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}_{k+1}))^{\intercal} \nabla \bm{h} (\bm{x}_{k+1}) + \bm{\mu}_{k+1}^{\intercal} \bm{A} \\
&= \nabla \mathcal{L} (\bm{x}_{k+1}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}_{k+1}), \bm{\mu}_{k+1})
\end{align*}
and $\bm{\mu}_{k+1}^{\intercal} \bm{r} (\bm{x}_{k+1}) = 0$. Hence, by the definition of $E_{m,0}$ it follows that
\begin{align*}
E_{m,0} (\bm{x}_{k+1}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}_{k+1}), \bm{\mu}_{k+1}) = 0.
\end{align*}
So if PASA is used to solve problem (\ref{prob:aug-lag-mod}) and it converges to a stationary point then we have that the multiplier error is equal to zero at this point for some $\bm{\mu}_{k+1}$ that we do not explicitly know. The global error estimator used for stopping criterion in PASA at a point $\bm{x} \in \Omega$ is given by $E_{\scaleto{PASA}{4pt}} (\bm{x}) = \| \bm{y} (\bm{x},1) - \bm{x} \|$ where $\bm{y} (\bm{x},\alpha)$ is defined to be the minimizer for the problem
\begin{align}
\min_{\bm{y}} \bigg\{ \frac{1}{2} \| \bm{x} - \alpha \bm{g} (\bm{x}) - \bm{y} \|^2 : \bm{r}(\bm{y}) \leq \bm{0} \bigg\} \label{prob:pasa-error}
\end{align} 
for $\alpha > 0$ and $\bm{g} (\bm{x})$ is the transpose of the gradient of the cost function in the polyhedral constrained problem being solved by PASA. Note that in our case we have 
\begin{align}
\bm{g} (\bm{x})^{\intercal} = \nabla_x \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) = \nabla_x f (\bm{x}) + \bm{\bar{\lambda}}_k^{\intercal} \nabla_x \bm{h} (\bm{x}) + 2 q \bm{h} (\bm{x})^{\intercal} \nabla_x \bm{h} (\bm{x}) \label{eq:aug-lag-mod.0.0}
\end{align} 
but we will continue to write $\bm{g} (\bm{x})$ for simplicity. When an iterate $\bm{x} \in \Omega$ of PASA yields $E_{\scaleto{PASA}{4pt}} (\bm{x})$ is sufficiently small, where the tolerance is set by the user, then PASA terminates. Now fix $\bm{x} \in \Omega$ and consider problem (\ref{prob:pasa-error}). By the KKT conditions, there exists a vector $\bm{\mu}(\bm{x},\alpha)$ such that
\begin{enumerate}
\item[(N.1)] Gradient of Lagrangian equals zero: $(\bm{y}(\bm{x},\alpha) - \bm{x})^{\intercal} + \alpha \bm{g} (\bm{x})^{\intercal} + \bm{\mu}(\bm{x}, \alpha)^{\intercal} \bm{A} = \bm{0}$
\item[(N.2)] Satisfies inequality constraints: $\bm{r}(\bm{y}(\bm{x},\alpha)) \leq \bm{0}$
\item[(N.3)] Nonnegativity of inequality multipliers: $\bm{\mu} (\bm{x},\alpha) \geq \bm{0}$
\item[(N.4)] Complimentary slackness: $\bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{r}(\bm{y}(\bm{x},\alpha)) = 0$.
\end{enumerate}
Our goal is to use the KKT conditions (N.1) -- (N.4) for problem (\ref{prob:pasa-error}) to derive a formula for the multiplier error of our original problem in terms of the current iterate of PASA. Then we will work to bound this expression in terms of the global error estimator of PASA. By recalling that the multiplier error estimator for our original problem is given by
\begin{align*}
E_{m,0} (\bm{x}, \bm{\lambda}, \bm{\mu}) = \| \nabla_x f (\bm{x}) + \bm{\lambda}^{\intercal} \nabla_x \bm{h} (\bm{x}) + \bm{\mu}^{\intercal} \bm{A} \|^2 - \bm{\mu}^{\intercal} \bm{r} (\bm{x})
\end{align*} 
we have that we can express the multiplier error at the PASA iterate $\bm{x}$ by
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}) = \| \bm{g} (\bm{x})^{\intercal} + \bm{\mu}^{\intercal} \bm{A} \|^2 - \bm{\mu}^{\intercal} \bm{r} (\bm{x}). \label{eq:aug-lag-mod.0}
\end{align} 
With this in mind, we now proceed as follows. First, from (N.1) we have that
\begin{align*}
\bm{g} (\bm{x})^{\intercal} + \frac{1}{\alpha} \bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{A} = \frac{1}{\alpha}(\bm{x} - \bm{y}(\bm{x},\alpha))^{\intercal}
\end{align*}
Now taking the norm of both sides and squaring yields
\begin{align}
\left\| \bm{g} (\bm{x})^{\intercal} + \frac{1}{\alpha} \bm{\mu} (\bm{x},\alpha)^{\intercal} \bm{A} \right\|^2 = \frac{1}{\alpha^2} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.1}
\end{align}
Additionally, right multiplying both sides of (N.1) by $\frac{1}{\alpha} (\bm{y}(\bm{x},\alpha) - \bm{x})$ and using (N.4) yields
\begin{align}
- \frac{1}{\alpha} \bm{\mu}(\bm{x},\alpha)^{\intercal} \bm{r}(\bm{x}) = - \frac{1}{\alpha} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2 - \bm{g}(\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}). \label{eq:aug-lag-mod.2}
\end{align}
%Note that as $\bm{x} \in \Omega$ we have that $-\bm{\mu}(\bm{x})^{\intercal} \bm{A} \bm{x} \geq 0$ which implies that $\nabla_x \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x}) - \bm{x}) \leq \bm{0}$. 
Combining (\ref{eq:aug-lag-mod.0}), (\ref{eq:aug-lag-mod.1}), and (\ref{eq:aug-lag-mod.2}) we now have that
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},\alpha)/\alpha) = - \bm{g}(\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}) + \left(\frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.4}
\end{align}
Note that from property P6 in Proposition 2.1 of \cite{Hager2006} we have that for all $\bm{x} \in \Omega$
\begin{align*}
- \bm{g} (\bm{x})^{\intercal} (\bm{y}(\bm{x},\alpha) - \bm{x}) \geq \frac{1}{\alpha} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2.
\end{align*}
Combining this fact with (\ref{eq:aug-lag-mod.4}) yields a lower bound for the multiplier error
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},\alpha)/\alpha) 
\geq \frac{1}{\alpha^2} \| \bm{y}(\bm{x},\alpha) - \bm{x} \|^2. \label{eq:aug-lag-mod.4.1}
\end{align}
In particular, by taking $\alpha = 1$ and recalling (\ref{eq:aug-lag-mod.0.0}) we have
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= - \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x},1) - \bm{x}). \label{eq:aug-lag-mod.4.2}
\end{align}
Additionally, by the definition of $E_{\scaleto{PASA}{4pt}} (\bm{x})$ and Cauchy-Schwarz we have
\begin{align}
E_{\scaleto{PASA}{4pt}} (\bm{x})^2 
\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
\leq \| \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x}). \label{eq:aug-lag-mod.5}
\end{align}
As $E_{\scaleto{PASA}{4pt}} (\bm{x}) = 0$ if and only if $\bm{x}$ is a stationary point, we have $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) = 0$ if and only if $\bm{x}$ is a stationary point. 

Hence, in (\ref{eq:aug-lag-mod.4}) we have derived a closed form expression for the multiplier error estimator for the general nonlinear program in terms of the current iterate of PASA and a known KKT equality multiplier. Additionally, in (\ref{eq:aug-lag-mod.5}) upper and lower bounds for the multiplier error estimator for the general nonlinear program were derived in terms of the global error estimator used by PASA. Thus, we can compute and bound the value of the multiplier error estimator $E_{m,0}$ at $(\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,\alpha))$ by using information already computed by PASA without requiring the inequality multiplier vector $\bm{\mu}(\bm{x}_k,\alpha)$. We now provide the following result which will be useful to note for practical implementations of this approach for augmented Lagrangian problems. The result follows immediately from (\ref{eq:aug-lag-mod.5}) and the definition of the dot product.

\begin{theorem} \label{thm:pasa-aug-lag-conv}
Suppose that PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ such that
\begin{align}
\| \nabla \mathcal{L}_{q} (\bm{u}_i, \bm{\bar{\lambda}}_k) \| \cos (\theta_i) \leq C, \label{result:pasa-aug-lag-conv.1}
\end{align}
for all $i$, where $C$ is some constant and $\theta_i$ is the angle between the vectors $\bm{u}_i - \bm{y}(\bm{u}_i,1)$ and $\mathcal{L}_{q} (\bm{u}_i, \bm{\bar{\lambda}}_k)$. Then
\begin{align*}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0
\end{align*}
if and only if
\begin{align*}
\liminf_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0.
\end{align*}
\end{theorem}
\iffalse
\begin{proof}
By definition of the dot product, it follows from (\ref{eq:aug-lag-mod.4.2}) and our hypothesis that
\begin{align*}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{u}_i,1)) 
&= \| \nabla \mathcal{L}_{q} (\bm{u}_i, \bm{\bar{\lambda}}_k)\| \| \bm{y}(\bm{u}_i,1) - \bm{u}_i \| \cos (\theta_i) \\
&= \| \nabla \mathcal{L}_{q} (\bm{u}_i, \bm{\bar{\lambda}}_k)\| \cos (\theta_i) E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \\
&\leq C E_{\scaleto{PASA}{4pt}} (\bm{u}_i).
\end{align*}
Combining this with the lower bound on $E_{m,0}$ we have that
\begin{align*}
E_{\scaleto{PASA}{4pt}} (\bm{u}_i)^2 
\leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
\leq C E_{\scaleto{PASA}{4pt}} (\bm{u}_i)
\end{align*}
which concludes the proof.
\end{proof}
\fi

Before providing a convergence result for this approach to phase one of NPASA, we consider how convergence of PASA for the subproblem in phase one relates to the multiplier error estimator of the original nonlinear program we are trying to solve. %Consider solving problem (\ref{prob:aug-lag-mod}) using PASA.
In particular, since our branching criterion in phase one of NPASA is given by $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \leq \theta E_c (\bm{x}_k)$, we would like some conditions under which PASA converges to a point $\bm{x}_k$ at which $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k) \approx 0$. The following result is a natural first step as it is a global convergence result for the multiplier error based on the global convergence result for PASA in \cite{Hager2016} that only requires one assumption in addition to those already imposed in \cite{Hager2016} to establish global convergence of PASA.

\begin{theorem} \label{thm:pasa-aug-lag}
Let $\mathcal{S}$ be the level set defined by
\begin{align*}
\mathcal{S} = \{ \bm{u} \in \Omega : \mathcal{L}_q (\bm{u}, \bm{\bar{\lambda}}_k) \leq \mathcal{L}_q (\bm{u}_0, \bm{\bar{\lambda}}_k) \}.
\end{align*}
Suppose that the following conditions hold:
\begin{enumerate}
\item[G1.] $\mathcal{L}_q (\bm{u}, \bm{\bar{\lambda}}_k)$ is bounded from below on $\mathcal{S}$ and $d_{\max} = \sup_{i} \| \bm{d}_i \| < \infty$
\item[G2.] If $\overline{\mathcal{S}}$ is the collection of $\bm{u} \in \Omega$ whose distance to $\mathcal{S}$ is at most $d_{\max}$, then $\nabla_u \mathcal{L}_q (\bm{u}, \bm{\bar{\lambda}}_k)$ is Lipschitz continuous on $\overline{\mathcal{S}}$.
\end{enumerate}
Then PASA with $\varepsilon = 0$ either terminates in a finite number of iterations to a stationary point, $\bm{u}^*$, at which
\begin{align*}
E_{m,0} (\bm{u}^*, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}^*), \bm{\mu} (\bm{u}^*,1)) = 0
\end{align*}
or PASA generates a sequence of points $\{ \bm{u}_i \}_{i=1}^{\infty}$ with the property that 
\begin{align*}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0
\end{align*}
if, in addition to G1 and G2, (\ref{result:pasa-aug-lag-conv.1}) holds for the sequence $\{ \bm{u}_i \}_{i=1}^{\infty}$.
\end{theorem}
\begin{proof}
As the hypotheses of Theorem 3.2 in \cite{Hager2016} are satisfied for problem (\ref{prob:aug-lag-mod}), we have that either PASA converges to a stationary point $\bm{u}^*$, at which $E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0$ or $\liminf_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0$. The result now follows from Theorem~\ref{thm:pasa-aug-lag-conv}.
% (Incorrect argument that thgouht we didn't need boundedness assumption)
\iffalse
Next, note that the set $\bar{\mathcal{L}}$ described in assumption A2 used as a hypothesis for Theorem 3.2 in \cite{Hager2016} is a closed and bounded set. As $\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$ is continuous we have that $\| \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) \|$ attains its maximum value on $\bar{\mathcal{L}}$. Finally, as $\bm{u}_i \in \bar{\mathcal{L}}$ for all $i$, we have that the sequence $\{ \| \nabla \mathcal{L}_q (\bm{u}_i, \bm{\bar{\lambda}}_k) \| \}_{i = 0}^{\infty}$ is uniformly bounded. Now using inequality (\ref{eq:aug-lag-mod.5}) together with (\ref{eq:thm3.2-pasa.1}) and (\ref{eq:thm3.2-pasa.2}) concludes the proof.
\fi
%
\end{proof}

Next, we provide a result that holds when PASA generates an infinite sequence of iterates that converge to a stationary point but does not require as many assumptions as the global convergence result.

\begin{theorem} \label{thm:pasa-aug-lag-degenerate}
If PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ that converge to a stationary point $\bm{u}^*$ then
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i)) = 0. \label{result:aug-lag-degenerate.1}
\end{align}
\end{theorem}
\begin{proof}
As $\bm{u}^*$ is a stationary point, we have that $\bm{y} (\bm{u}^*) = \bm{u}^*$. So by (N.1) - (N.4) we have that $\bm{\mu}(\bm{u}^*) \geq \bm{0}$ satisfies $\nabla \mathcal{L}_{q} (\bm{u}^*, \bm{\bar{\lambda}}_k) + \bm{\mu}(\bm{u}^*)^{\intercal} \bm{A} = \bm{0}$ and $\bm{\mu}(\bm{u}^*)^{\intercal} \bm{A} \bm{u}^* = 0$. Hence, it follows that $E_{m,0} (\bm{u}^*, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}^*), \bm{\mu} (\bm{u}^*)) = 0$. As $\bm{u}_i \to \bm{u}^*$ and $\bm{\mu} (\bm{u}_i) \to \bm{\mu}(\bm{u}^*)$ when $i \to \infty$ and $E_{m,0}$ is continuous, the result in (\ref{result:aug-lag-degenerate.1}) follows.
\end{proof}

In addition to the global convergence result in Theorem~\ref{thm:pasa-aug-lag}, we would like to determine if we can establish an alternative bound on the directional derivative appearing in the formula for the multiplier error (\ref{eq:aug-lag-mod.4.2}) under a different set of assumptions. This is of interest as the upper bound in (\ref{eq:aug-lag-mod.5}) may be problematic if, say, in practice the term $\| \nabla_x \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) \|$ grows larger as $\bm{x}$ gets closer to a stationary point. We now consider the following. First, note that the local error estimator used by PASA for this problem is defined by $e_{\scaleto{PASA}{4pt}} (\bm{x}) = \| \bm{g}^{\mathcal{A}} (\bm{x}) \|$, where 
\begin{align*}
\bm{g}^{\mathcal{A}} (\bm{x}) = \arg\min \{ \| \bm{z} - \bm{g} (\bm{x}) \| : \bm{z} \in \mathbb{R}^n \ \text{and} \ \bm{A}_{\mathcal{A} (\bm{x})} \bm{z} = \bm{0} \},
\end{align*}
where $\mathcal{A} (\bm{x}) = \{ i : (\bm{A} \bm{x})_i = 0 \}$. By this definition, we can decompose $\bm{g} (\bm{x})$ as
\begin{align*}
\bm{g} (\bm{x}) = \bm{g}^{\mathcal{A}} (\bm{x}) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x})
\end{align*}
where $\bm{g}^{\mathcal{A}^{\perp}} (\bm{x}) \perp \mathcal{N} \left( A_{\mathcal{A} (\bm{x})} \right)$. Now using the formula in (\ref{eq:aug-lag-mod.4.2}) yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},1)) 
&= \bm{g} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) \nonumber \\
&= \left( \bm{g}^{\mathcal{A}} (\bm{x}) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x}) \right)^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) \nonumber \\ 
&= \bm{g}^{\mathcal{A}} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)) + \bm{g}^{\mathcal{A}^{\perp}} (\bm{x})^{\intercal} (\bm{x} - \bm{y} (\bm{x},1)). \label{eq:aug-lag-mod.6}
\end{align}
So if at some point $\bm{x} \in \Omega$ we have that $(\bm{x} - \bm{y} (\bm{x},1) ) \in \mathcal{N} (\bm{A}_{\mathcal{A}(\bm{x})})$ then it follows from (\ref{eq:aug-lag-mod.6}) that
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x},1)) \label{eq:aug-lag-mod.7}
\end{align}
and in such a case Cauchy-Schwarz yields
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
\leq e_{\scaleto{PASA}{4pt}} (\bm{x}) E_{\scaleto{PASA}{4pt}} (\bm{x}). \label{eq:aug-lag-mod.8}
\end{align}
% (Old approach that works but requires some more machinery)%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Now let
\begin{align*}
\mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right) = \arg\min \left\{ \frac{1}{2} \| \bm{x} - \bm{g} (\bm{x}) - \bm{y} \|^2 : \bm{y} \in \Omega (\bm{x}) \right\},
\end{align*}
where $\Omega (\bm{x}) = \{ \bm{z} \in \Omega : (\bm{A} \bm{z} - \bm{b} )_i = 0, \ \text{for} \ i \in \mathcal{A} (\bm{x}) \}$. By definition, it follows that the active set of $\mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right)$ contains $\mathcal{A} (\bm{x})$. Hence, we have that 
\begin{align*}
\bm{a}_i^{\intercal} (\bm{x} - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right)) = b_i - b_i = 0,
\end{align*}
for all $i \in \mathcal{A} (\bm{x})$, which yields that
\begin{align*}
\bm{x} - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right) \in \mathcal{N} (\bm{A}_{\mathcal{A} (\bm{x})}).
\end{align*}
Now using the formula in (\ref{eq:aug-lag-mod.4}) yields
\begin{align*}
E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}^{\mathcal{A}} (\bm{x})) 
&= \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right)) \\
&= \left( \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) + \nabla \mathcal{L}_{q}^{\mathcal{A}^{\perp}} (\bm{x}, \bm{\bar{\lambda}}_k) \right) (\bm{x} - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right)) \\ 
&= \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right))
\end{align*}
Now by adding and subtracting $\mathcal{P}_{\Omega} \left( \bm{x} - \bm{g} (\bm{x}) \right)$ we get
\begin{align}
E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}^{\mathcal{A}} (\bm{x})) 
&= \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \mathcal{P}_{\Omega} \left( \bm{x} - \bm{g} (\bm{x}) \right)) \nonumber \\
& \quad + \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\mathcal{P}_{\Omega} \left( \bm{x} - \bm{g} (\bm{x}) \right) - \mathcal{P}_{\Omega(\bm{x})} \left( \bm{x} - \bm{g} (\bm{x}) \right)). \label{eq:aug-lag-mod.6}
\end{align}
So if at some point $\bm{x} \in \Omega$ we have that $\bm{y} (\bm{x}) \in \mathcal{A} (\bm{x})$ then it follows from (\ref{eq:aug-lag-mod.6}) that
\begin{align}
E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x})) 
= \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x})) \label{eq:aug-lag-mod.7}
\end{align}
and in such a case Cauchy-Schwarz yields
\begin{align}
E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x})) 
\leq e_{\scaleto{PASA}{4pt}} (\bm{x}) E_{\scaleto{PASA}{4pt}} (\bm{x}). \label{eq:aug-lag-mod.8}
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the case that PASA converges to a nondegenerate stationary point, we have the following result.
\begin{theorem} \label{thm:pasa-aug-lag-nondegenerate}
If PASA with $\varepsilon = 0$ generates an infinite sequence of iterates $\{ \bm{u}_i \}_{i=1}^{\infty}$ that converge to a nondegenerate stationary point $\bm{u}^*$, then there exists an integer $M$ such that 
\begin{align}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
\leq e_{\scaleto{PASA}{4pt}} (\bm{u}_i) E_{\scaleto{PASA}{4pt}} (\bm{u}_i), \label{result:aug-lag-nondegenerate.1}
\end{align}
for all $i \geq M$. 
% (Not necessary since better result established)
\iffalse
, and we have that
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) = 0. \label{result:aug-lag-nondegenerate.2}
\end{align}
\fi
%
\end{theorem}
\begin{proof}
By equations (5.3) and (5.4) in Theorem 5.1 of \cite{Hager2016}, there exists an integer $M$ such that 
\begin{align*}
\mathcal{A} (\bm{u}_i) \subseteq \mathcal{A} (\bm{y}(\bm{u}_i,1))
\end{align*}
for all $i \geq M$. Hence, for all $i \geq M$ we have that $(\bm{u}_i - \bm{y} (\bm{u}_i,1)) \in \mathcal{N}(\bm{A}_{\mathcal{A}(\bm{u}_i)})$ since
\begin{align*}
\bm{A}_{\mathcal{A}(\bm{u}_i)} (\bm{u}_i - \bm{y} (\bm{u}_i,1))
= \bm{b}_{\mathcal{A}(\bm{u}_i)} - \bm{b}_{\mathcal{A}(\bm{u}_i)}
= \bm{0}.
\end{align*}
By (\ref{eq:aug-lag-mod.7}), we now have
\begin{align*}
E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i,1)) 
&= \nabla \mathcal{L}_{q}^{\mathcal{A}} (\bm{u}_i, \bm{\bar{\lambda}}_k) (\bm{u}_i - \bm{y} (\bm{u}_i,1)),
\end{align*}
for all $i \geq M$. Now applying Cauchy-Schwarz to the right hand side of this equation and recalling the definition of $e_{\scaleto{PASA}{4pt}} (\cdot)$ and $E_{\scaleto{PASA}{4pt}} (\cdot)$ yields (\ref{result:aug-lag-nondegenerate.1}), for all $i \geq M$.
% (Proof for unnecessary result)
\iffalse
As $\bm{u}_i \to \bm{u}^*$ and $E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0$, we have that there exists a constant $C$ such that
\begin{align}
E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \leq C, \label{eq:aug-lag-nondegenerate.1}
\end{align}
for $i \geq M$. By Theorem 5.1 in \cite{Hager2016}, only phase two of PASA is executed within a finite number of iterations so we focus on the LCO method used in phase two of PASA. From condition F2 for phase two of PASA in \cite{Hager2016} and the fact that $\bm{u}_i$ is finite dimensional it follows that $\mathcal{A} (\bm{u}_i)$ is fixed for $i$ sufficiently large. Hence, by condition F3 for phase two of PASA in \cite{Hager2016} we have that
\begin{align}
\liminf_{i \to \infty} e_{\scaleto{PASA}{4pt}} (\bm{u}_i) = 0. \label{eq:aug-lag-nondegenerate.2}
\end{align}
Now (\ref{eq:aug-lag-nondegenerate.1}) and (\ref{eq:aug-lag-nondegenerate.2}) together with (\ref{result:aug-lag-nondegenerate.1}) yields (\ref{result:aug-lag-nondegenerate.2}).
\fi
%
% (I believe the following version is not always true since e(x) may not be bounded)
\iffalse
As $\bm{u}_i \to \bm{u}^*$ and 
\begin{align*}
E_{\scaleto{PASA}{4pt}} (\bm{u}^*) = 0, 
\end{align*}
it now follows from (\ref{eq:aug-lag-nondegenerate.1}) that
\begin{align*}
\liminf_{i \to \infty} E_m (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu} (\bm{u}_i)) \leq \left( \liminf_{i \to \infty} e_{\scaleto{PASA}{4pt}} (\bm{u}_i) \right) \left( \lim_{i \to \infty} E_{\scaleto{PASA}{4pt}} (\bm{u}_i) \right) = 0
\end{align*}
which concludes the proof.
\fi
%
\end{proof}

If we include second order assumptions then we can obtain an upper bound for the multiplier error in degenerate problems. This result follows from some standard analysis and an application of Lemma 6.4 from \cite{Hager2016}.
\begin{theorem} \label{thm:pasa-aug-lag-degenerate2}
Suppose that $\mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$ is twice continuously differentiable in a neighborhood of a local minimizer $\bm{x}^*$ where the active constraint gradients are linearly independent and the strong second-order sufficient optimality conditions hold. Then there exists a $\rho > 0$ such that for all $\bm{x} \in \mathcal{B}_{\rho} (\bm{x}^*)$ 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x})) = O \left( E_{\scaleto{PASA}{4pt}} (\bm{x}) \right), \label{result:aug-lag-degenerate2.1}
\end{align}
where $\kappa$ is a Lipschitz constant for $\nabla \mathcal{L}_{q} (\bm{x}, \bm{\lambda})$ on $\mathcal{B}_{\rho} (\bm{x}^*)$.
\end{theorem}
\begin{proof}
Using the formula in (\ref{eq:aug-lag-mod.4}) we have that
\begin{align*}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&= \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x})) \\
&= \left( \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) - \nabla \mathcal{L}_{q} (\bm{x}^*, \bm{\bar{\lambda}}_k) \right) (\bm{x} - \bm{y}(\bm{x})) + \nabla \mathcal{L}_{q} (\bm{x}^*, \bm{\bar{\lambda}}_k) (\bm{x} - \bm{y}(\bm{x}))
\end{align*}
which when applying Cauchy-Schwarz, the triangle inequality, and the Lipschitz continuity of $\nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k)$ yield
\begin{align*}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&\leq \kappa \| \bm{x} - \bm{x}^* \| E_{\scaleto{PASA}{4pt}} (\bm{x}) + \| \nabla_x \mathcal{L}_{q} (\bm{x}^*, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x}).
\end{align*}
Finally, applying Lemma 6.4 from \cite{Hager2016} yields
\begin{align*}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x}))
&\leq \kappa \sqrt{1 + \left( \frac{2 (1 + \kappa) ( 3 + \kappa)}{\sigma} \right)} E_{\scaleto{PASA}{4pt}} (\bm{x})^2 + \| \nabla_x \mathcal{L}_{q} (\bm{x}^*, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x}).
\end{align*}
which concludes the proof.
\end{proof}

With Theorems~\ref{thm:pasa-aug-lag} -- \ref{thm:pasa-aug-lag-degenerate2} established, it seems that this is a suitable approach for solving the subproblem in phase one of NPASA that allows us to still compute the multiplier error estimator. We now provide a result on convergence of phase one of NPASA when using this approach for solving each subproblem.

\begin{theorem} \label{thm:pasa-aug-lag-global-conv}
Suppose that $\Omega$ is compact and that $f, \bm{h} \in \mathcal{C}^1 (\Omega)$. Suppose that the following are satisfied:
\begin{enumerate}
\item $\{ \bm{x}_k \}_{k=0}^{\infty}$ is a sequence with $\bm{x}_k \in \Omega$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$, for all $k \geq 0$
\item $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ is updated using the formula for $\bm{\lambda}'$ in GS algorithm, Algorithm~\ref{alg:gs}
\item $\{ q_k \}_{k=0}^{\infty}$ is a sequence of real numbers such that $q_k \to \infty $ as $k \to \infty$.
\end{enumerate}
Then any subsequence of $\{ \bm{x}_k \}_{k=0}^{\infty}$ with limit point $\bm{x}^*$ such that assumption (\textbf{LI}) holds at $\bm{x}^*$ satisfies $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*,1)) = E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*,1)) = 0$, where $\bm{\lambda}^*$ is the limit of the corresponding subsequence for $\{ \bm{\lambda}_k \}$.
\end{theorem}
\begin{proof}
Let $\{ \bm{x}_k \}_{k=0}^{\infty}$ be a subsequence with limit point $\bm{x}^*$ and let $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ be corresponding subsequences of multipliers. First, we show that $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. Rearranging the terms in equation (N.1) with $\alpha = 1$ we have that 
\begin{align*}
\begin{bmatrix}
\nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{A}^{\intercal}
\end{bmatrix} \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix}
= \bm{x}_k - \bm{y}(\bm{x}_k,1) - \nabla f (\bm{x}_k)^{\intercal}
\end{align*}
By our hypothesis that (\textbf{LI}) holds at $\bm{x}^*$, there exists a $N$ such that the matrix $\begin{bmatrix} \nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{A}^{\intercal} \end{bmatrix}$ is of full column rank, for all $k \geq N$. Hence, there exists a constant $M$ such that
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix} \right\|
\leq M \| \bm{x}_k - \bm{y}(\bm{x}_k,1) - \nabla f (\bm{x}_k)^{\intercal} \|, \label{eq:phase-one-convergence.1}
\end{align}
for $k$ sufficiently large. From property P6 in Proposition 2.1 of \cite{Hager2006} we have that
\begin{align*}
\| \bm{x}_k - \bm{y}(\bm{x}_k,1) \|^2 \leq \nabla_x \mathcal{L}_{q} (\bm{x}_k, \bm{\bar{\lambda}}_{k-1})^{\intercal} (\bm{x}_k - \bm{y}(\bm{x}_k,1)).
\end{align*}
Hence, using the hypothesis that $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$ together with (\ref{eq:aug-lag-mod.4}) it follows that
\begin{align*}
\| \bm{x}_k - \bm{y}(\bm{x}_k,1) \|^2 
\leq E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) 
\leq E_c (\bm{x}_k).
\end{align*}
As $E_c (\bm{x}_k) = \| \bm{h} (\bm{x}_k) \|^2$, the inequality in (\ref{eq:phase-one-convergence.1}) now yields
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k,1)
\end{bmatrix} \right\|
\leq M \left( \| \bm{h} (\bm{x}_k) \| + \| \nabla f (\bm{x}_k) \| \right), \label{eq:phase-one-convergence.2}
\end{align}
for $k$ sufficiently large. As $f, \bm{h} \in \mathcal{C}^1$, it follows from (\ref{eq:phase-one-convergence.2}) that the sequences $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}(\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. As the sequence $\{ \bm{\bar{\lambda}}_k \}_{k=0}^{\infty}$ is uniformly bounded by construction, there exists a constant $\Lambda$ such that $\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \| \leq \Lambda$ for all $k$ sufficiently large. Now using the update formula $\bm{\lambda}_{k} = \bm{\bar{\lambda}}_{k-1} + 2 q_k \bm{h} (\bm{x}_{k})$, we have that
\begin{align}
\| \bm{h} (\bm{x}_{k}) \| 
= \frac{\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \|}{2 q_k} 
\leq \frac{\Lambda}{2 q_k}, \label{eq:phase-one-convergence.3}
\end{align}
for all $k$ sufficiently large. So (\ref{eq:phase-one-convergence.3}) together with the hypothesis that $q_k \to \infty$ as $k \to \infty$, yields that
\begin{align*}
\lim_{k \to \infty} E_c (\bm{x}_{k}) = \lim_{k \to \infty} \| \bm{h} (\bm{x}_{k}) \|^2 \leq \lim_{k \to \infty} \frac{\Lambda^2}{4 q_k^2} = 0.
\end{align*}
As $E_0 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))^2 = E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) + E_c (\bm{x}_k)$ and $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1)) \leq \theta E_c (\bm{x}_k)$ for all $k$ by hypothesis, it now follows that $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*,1)) = 0$. Lastly, from Lemma~\ref{lem:E0-E1-relationship} it follows that $E_1 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*,1)) = 0$ which concludes the proof.
\end{proof}

%
\iffalse
\begin{theorem}
Suppose that the following are satisfied
\begin{enumerate}
\item $\{ \bm{x}_k \}_{k=0}^{\infty}$ is a sequence with $\bm{x}_k \in \Omega$ and $E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu}(\bm{x}_k)) \leq \theta E_c (\bm{x}_k)$, for all $k \geq 0$
\item There exists a scalar $\eta < \infty$ such that $\sup_{k \geq 0} E_{\scaleto{PASA}{4pt}} (\bm{x}_k) \leq \eta$
\item $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ is updated using the formula described after Algorithm~\ref{alg:npasa}
\item $\{ q_k \}_{k=0}^{\infty}$ is a sequence of reals numbers such that $q_k \to \infty $ as $k \to \infty$.
\end{enumerate}
Then any subsequence of $\{ \bm{x}_k \}_{k=0}^{\infty}$ with limit point $\bm{x}^*$ such that $\nabla \bm{h} (\bm{x}^*)$ and $\nabla \bm{r} (\bm{x}^*)$ are of full rank satisfies $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu}(\bm{x}^*)) = 0$, where $\bm{\lambda}^*$ is the limit of the corresponding subsequence for $\{ \bm{\lambda}_k \}$.
\end{theorem}
\begin{proof}
Let $\{ \bm{x}_k \}_{k=0}^{\infty}$ be a subsequence with limit point $\bm{x}^*$ and let $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ be corresponding subsequences of multipliers. First, we show that $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu} (\bm{x}_k,1) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. Rearranging the terms in equation (N.1) we have that 
\begin{align*}
\begin{bmatrix}
\nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \nabla \bm{r} (\bm{x}_k)^{\intercal}
\end{bmatrix} \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k)
\end{bmatrix}
= \bm{x}_k - \bm{y}(\bm{x}_k) - \nabla f (\bm{x}_k)^{\intercal}
\end{align*}
By our hypothesis that $\nabla \bm{h} (\bm{x}^*)$ and $\nabla \bm{r} (\bm{x}^*)$ are of full rank, there exists a $N$ such that the matrix $\begin{bmatrix} \nabla \bm{h} (\bm{x}_k)^{\intercal} \ \vert \ \bm{r} (\bm{x}_k)^{\intercal} \end{bmatrix}$ is of full rank, for all $k \geq N$. Hence, there exists a constant $M$ such that
\begin{align}
\left\| \begin{bmatrix}
\bm{\lambda}_k \\
\bm{\mu} (\bm{x}_k)
\end{bmatrix} \right\|
\leq M \| \bm{x}_k - \bm{y}(\bm{x}_k) - \nabla f (\bm{x}_k)^{\intercal} \| 
\leq M ( \eta + \| \nabla f (\bm{x}_k) \|), \label{eq:phase-one-convergence.1}
\end{align}
for $k$ sufficiently large, where the final inequality follows from the triangle inequality together with $\sup_{k \geq 0} E_{\scaleto{PASA}{4pt}} (\bm{x}_k) \leq \eta$. As $f \in \mathcal{C}^1$ it follows from (\ref{eq:phase-one-convergence.1}) that the sequences $\{ \bm{\lambda}_k \}_{k=0}^{\infty}$ and $\{ \bm{\mu}(\bm{x}_k) \}_{k=0}^{\infty}$ are uniformly bounded for $k$ sufficiently large. As the sequence $\{ \bm{\bar{\lambda}}_k \}_{k=0}^{\infty}$ is uniformly bounded by construction, there exists a constant $\alpha$ such that $\| \bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1} \| \leq \alpha$ for all $k$ sufficiently large. Now using the update formula $\bm{\lambda}_{k} = \bm{\bar{\lambda}}_{k-1} + 2 q_k \bm{h} (\bm{x}_{k})$, we have that
\begin{align*}
\bm{h} (\bm{x}_{k}) = \frac{\bm{\lambda}_{k} - \bm{\bar{\lambda}}_{k-1}}{2 q_k}.
\end{align*}
which, together with the hypothesis that $q_k \to \infty$ as $k \to \infty$, yields that
\begin{align*}
\lim_{k \to \infty} E_c (\bm{x}_{k}) = \lim_{k \to \infty} \| \bm{h} (\bm{x}_{k}) \|^2 \leq \lim_{k \to \infty} \frac{\alpha^2}{2 q_k} = 0.
\end{align*}
Finally, as $E_0 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k))^2 = E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k)) + E_c (\bm{x}_k)$ and $E_m (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k)) \leq \theta E_c (\bm{x}_k)$ for all $k$ by hypothesis, it now follows that $E_0 (\bm{x}^*, \bm{\lambda}^*, \bm{\mu} (\bm{x}^*)) = 0$.
\end{proof}
\fi
%

Next, we provide a note on implementation of this augmented Lagrangian method using PASA. Traditionally, the stopping criterion in PASA at the iterate $\bm{x}$ is given by $E_{\scaleto{PASA}{4pt}} (\bm{x}) \leq \varepsilon$, where $\varepsilon$ is a user provided stopping tolerance value. From our analysis in this section, we noted that $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) \leq \| \nabla \mathcal{L} (\bm{x}, \bm{\bar{\lambda}}_k) \| E_{\scaleto{PASA}{4pt}} (\bm{x})$. So if PASA terminates using its regular stopping criterion at a point $\bm{x}$ where $\| \nabla \mathcal{L} (\bm{x}, \bm{\bar{\lambda}}_k) \| > 1$ then it is possible that $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) > \varepsilon$. With this in mind, we propose an update to the stopping criterion for PASA when used with this augmented Lagrangian scheme. Using the formula in (\ref{eq:aug-lag-mod.4.2}) we propose that PASA terminates when
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) = - \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x},1) - \bm{x}) \leq \varepsilon. \label{eq:pasa-aug-lag-stop-crit1}
\end{align}
Note that both of the vectors required for the dot product are already available at each iteration of PASA due to the use of the gradient of the cost function and the need to check the regular stopping criterion for PASA. Alternatively, to ensure that the branching criterion between for phase one to phase two NPASA is satisfied, we could instead terminate when 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu} (\bm{x},1)) 
= - \nabla \mathcal{L}_{q} (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y}(\bm{x},1) - \bm{x}) 
\leq \min \left\{ \varepsilon, \theta E_c (\bm{x}) \right\}. \label{eq:pasa-aug-lag-stop-crit2}
\end{align}
where $E_c (\bm{x}) = \| \bm{h} (\bm{x}) \|^2$. In addition to an evaluation of the dot product for the left hand side of the inequality, this would require an evaluation of the equality constraints for the right hand side. However, as updating the multipliers $\bm{\bar{\lambda}}_k$ requires evaluating the equality constraints then we can compute the norm after evaluating these constraints to check the branching criterion. Note that if the hypotheses of Theorem~\ref{thm:pasa-aug-lag-conv} hold then the new stopping criterion in (\ref{eq:pasa-aug-lag-stop-crit1}) will be satisfied for any augmented Lagrangian problem in which the original stopping criterion, $E_{\scaleto{PASA}{4pt}}(\bm{x}) \leq \varepsilon$, will be satisfied.

Our next discussion in this section focuses on establishing a global convergence result for the augmented Lagrangian problem like Theorem~\ref{thm:pasa-aug-lag} but that does not require assumption (\ref{result:pasa-aug-lag-conv.1}). To this end, we propose a slight modification to the PASA algorithm, Algorithm 2 in \cite{Hager2016}, that requires replacing all instances of $E_{\scaleto{PASA}{4pt}} (\bm{x})$ with $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},1)) = -\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},1) - \bm{x})$. This modification is provided in detail in Algorithm~\ref{alg:pasa-aug-lag}. First, we provide a necessary lemma that considers the relationship of the multiplier error estimator $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha)$ to $E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta)$ for various values of $0 < \alpha \leq \beta$. 
\begin{lemma} \label{thm:aug-lag-mult-error}
For a given $\bm{x}$, let $\bm{\mu} (\bm{x}, \alpha)$ satisfy the KKT conditions in (N.1) -- (N.4)
\begin{enumerate}
\item[(\ref{thm:aug-lag-mult-error}.1)] For $0 < \alpha \leq \beta$,
\begin{align*}
-\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\alpha) - \bm{x}) 
\leq -\nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\beta) - \bm{x}).
\end{align*}
\item[(\ref{thm:aug-lag-mult-error}.2)] For $0 < \alpha \leq \beta$,
\begin{align*}
- \alpha \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\beta) - \bm{x}) 
\leq - \beta \nabla \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k) (\bm{y} (\bm{x},\alpha) - \bm{x}).
\end{align*}
\item[(\ref{thm:aug-lag-mult-error}.3)] If $0 < \alpha \leq \beta \leq 1$ then
\begin{align*}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha).
\end{align*}
\item[(\ref{thm:aug-lag-mult-error}.4)] If $1 \leq \alpha \leq \beta \leq 3$ then
\begin{align*}
\alpha E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq \beta E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha).
\end{align*}
% Don't know $\alpha$ which minimizes multiplier error
%\item[(\ref{thm:aug-lag-mult-error}.4)] $\displaystyle E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},1)) = \min_{\alpha > 0} \left\{ E_m (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha) \right\}$.
\end{enumerate}
\end{lemma}
\begin{proof}
Suppose $0 < \alpha \leq \beta$. Let $\bm{d}^{\alpha} (\bm{x}) = \bm{y} (\bm{x}, \alpha) - \bm{x}$. By P1 in \cite{Hager2006} with $\bm{x} \gets \bm{x} - \alpha \bm{g} (\bm{x})$ and $\bm{y} \gets \bm{y} (\bm{x}, \beta)$, we have that
\begin{align*}
0 
&\leq (\bm{y} (\bm{x}, \alpha) - (\bm{x} - \alpha \bm{g} (\bm{x})))^{\intercal} (\bm{y} (\bm{x}, \beta) - \bm{y} (\bm{x},\alpha)) \\
&= ( \bm{d}^{\alpha} (\bm{x}) + \alpha \bm{g} (\bm{x}))^{\intercal} (\bm{d}^{\beta} (\bm{x}) - \bm{d}^{\alpha} (\bm{x})) \\
&= \bm{d}^{\alpha} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \| \bm{d}^{\alpha} (\bm{x}) \|^2 + \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}).
\end{align*}
Rearranging terms and dividing both sides by $\alpha$ yields
\begin{align*}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{1}{\alpha} \bm{d}^{\alpha} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2.
\end{align*}
It now follows from Cauchy-Schwarz that
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \| \| \bm{d}^{\beta} (\bm{x}) \| - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.1}
\end{align}
By swapping $\alpha$ and $\beta$ in the construction of (\ref{eq:aug-lag-mult-error.1}), we obtain the inequality
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \| \| \bm{d}^{\alpha} (\bm{x}) \| - \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.1.1}
\end{align}

As $\alpha \leq \beta$, by P4 in \cite{Hager2006} we have that $\| \bm{d}^{\alpha} (\bm{x}) \| \leq \| \bm{d}^{\beta} (\bm{x}) \|$. Substituting this into (\ref{eq:aug-lag-mult-error.1.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2 - \frac{1}{\beta} \| \bm{d}^{\beta} (\bm{x}) \|^2 
= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}). \label{eq:aug-lag-mult-error.2.1}
\end{align}
which is equivalent to (\ref{thm:aug-lag-mult-error}.1). 

By P5 in \cite{Hager2006}, we have that $\| \bm{d}^{\beta} (\bm{x}) \| \leq \frac{\beta}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|$ which combined with (\ref{eq:aug-lag-mult-error.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{\beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \nonumber \\
&= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{\beta - \alpha}{\alpha} \right) \frac{\| \bm{d}^{\alpha} (\bm{x}) \|^2}{\alpha}. \label{eq:aug-lag-mult-error.2.2}
\end{align}
By P6 in \cite{Hager2006} and the fact that $\beta - \alpha \geq 0$, we have that
\begin{align}
\left( \frac{\beta - \alpha}{\alpha} \right) \frac{\| \bm{d}^{\alpha} (\bm{x}) \|^2}{\alpha}
\leq \left( \frac{\beta - \alpha}{\alpha} \right) \left( - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) \right)
= \left( 1 - \frac{\beta}{\alpha} \right) \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}). \label{eq:aug-lag-mult-error.2.3}
\end{align}
Now (\ref{eq:aug-lag-mult-error.2.2}) and (\ref{eq:aug-lag-mult-error.2.3}) yield
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) 
&\leq - \frac{\beta}{\alpha}  \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) \label{eq:aug-lag-mult-error.2.4}
\end{align}
which is equivalent to (\ref{thm:aug-lag-mult-error}.2).

Now suppose that $\alpha \leq \beta \leq 1$. By P5 in \cite{Hager2006}, we have that $\| \bm{d}^{\beta} (\bm{x}) \| \leq \frac{\beta}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|$. Substituting this into (\ref{eq:aug-lag-mult-error.1}) yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x})
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \frac{\beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1}{\alpha} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \nonumber \\
&= - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 - \frac{1 - \beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.3}
\end{align}
Again, by P5 in \cite{Hager2006} we have that $-\frac{1}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \leq - \frac{1}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|$ and since $1 - \beta \geq 0$ it follows that 
\begin{align}
- \frac{1 - \beta}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 
\leq - \frac{1 - \beta}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|^2
= - \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2. \label{eq:aug-lag-mult-error.3.1}
\end{align}
Combining (\ref{eq:aug-lag-mult-error.3}) and (\ref{eq:aug-lag-mult-error.3.1}) and rearranging terms yields
\begin{align}
- \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2
&\leq - \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 \label{eq:aug-lag-mult-error.3.2}
\end{align}
which by (\ref{eq:aug-lag-mod.4}) is equivalent to 
\begin{align}
E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha) \label{eq:aug-lag-mult-error.2.0}
\end{align}
Hence, (\ref{thm:aug-lag-mult-error}.3) holds.

Now suppose that $1 \leq \alpha \leq \beta \leq 3$. By P5 in \cite{Hager2006}, we have that $-\frac{1}{\alpha^2} \| \bm{d}^{\alpha} (\bm{x}) \|^2 \leq - \frac{1}{\beta^2} \| \bm{d}^{\beta} (\bm{x}) \|$. Combining this with $\frac{1 - \beta}{\beta^3} \leq \frac{1 - \alpha}{\alpha^3} \leq 0$ for $1 \leq \alpha \leq \beta \leq 3$ yields
\begin{align}
\alpha \left(\frac{1 - \beta}{\beta^2} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2 
\leq \beta \left( \frac{1 - \alpha}{\alpha^2} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2.
\label{eq:aug-lag-mult-error.4}
\end{align}
As $\alpha \leq \beta$, combining (\ref{thm:aug-lag-mult-error}.2) with (\ref{eq:aug-lag-mult-error.4}) it follows that
\begin{align}
- \alpha \bm{g} (\bm{x})^{\intercal} \bm{d}^{\beta} (\bm{x}) + \alpha \left( \frac{1}{\beta^2} - \frac{1}{\beta} \right) \| \bm{d}^{\beta} (\bm{x}) \|^2
&\leq - \beta \bm{g} (\bm{x})^{\intercal} \bm{d}^{\alpha} (\bm{x}) + \beta \left( \frac{1}{\alpha^2} - \frac{1}{\alpha} \right) \| \bm{d}^{\alpha} (\bm{x}) \|^2 \label{eq:aug-lag-mult-error.4.1}
\end{align}
By the formula for $E_{m,0}$ in (\ref{eq:aug-lag-mod.4}), we have
\begin{align}
\alpha E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\beta)/\beta) 
\leq \beta E_{m,0} (\bm{x}, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{x}), \bm{\mu}(\bm{x},\alpha)/\alpha) \label{eq:aug-lag-mult-error.4.2}
\end{align}
which shows that (\ref{thm:aug-lag-mult-error}.4) holds.
\end{proof}

With this lemma established, we now provide the following convergence result for the gradient projection algorithm in phase one of PASA. This result is similar to Theorem 2.2 in \cite{Hager2006}.

\begin{theorem} \label{thm:ngpa-conv}
Suppose that G1 and G2 from Theorem~\ref{thm:pasa-aug-lag} are satisfied. If the nonmonotone gradient projection algorithm (NGPA) in \cite{Hager2006} with $\varepsilon = 0$ is used to solve problem (\ref{prob:aug-lag-mod}) then NGPA either terminates in a finite number of iterations at a stationary point, or generates a sequence of iterates $\{ \bm{u}_i \}_{i=0}^{\infty}$ satisfying
\begin{align*}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0.
\end{align*}
\end{theorem}
\begin{proof}
Let $F(\bm{x}) = \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$. First, note that from (3.6) in \cite{Hager2016}, the stepsize $s_k$ in the Armijo line search is bounded below by
\begin{align}
s_k \geq \min \left\{ 1, \frac{2 \eta (1 - \delta)}{\kappa \alpha_{\max}} \right\} =: c,
\end{align}
where $\kappa$ is the Lipschitz constant for $\nabla_x \mathcal{L}_q (\bm{x}, \bm{\bar{\lambda}}_k)$. From equation (2.16) in \cite{Hager2006} we have that
\begin{align}
- \delta c \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i) \leq F_i^r - F (\bm{u}_{i+1}), \label{eq:gpa-conv.1}
\end{align}
for some $\bar{\alpha}_i \in [\alpha_{\min}, \alpha_{\max}]$. We now proceed by way of contradiction. Accordingly, suppose that 
\begin{align*}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > 0.
\end{align*}
Then there exists a constant $\tau > 0$ such that 
\begin{align}
\tau \leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) 
= - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i), \label{eq:gpa-conv.2}
\end{align}
for all $i \geq 0$. Suppose $\bar{\alpha}_i \geq 1$. By (\ref{thm:aug-lag-mult-error}.1) in Theorem~\ref{thm:aug-lag-mult-error} with $\alpha = 1$ and $\beta = \bar{\alpha}_i$, we have
\begin{align}
\tau \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) 
\leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.3}
\end{align}
On the other hand, if $\bar{\alpha}_i \in (0,1)$ then by (\ref{thm:aug-lag-mult-error}.3) in Theorem~\ref{thm:aug-lag-mult-error} with $\alpha = \bar{\alpha}_i$ and $\beta = 1$ we have
\begin{align}
- \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) 
\leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i) + \left( \frac{1}{\bar{\alpha}_i} - 1 \right) \frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i}. \label{eq:gpa-conv.4}
\end{align}
From P6 in \cite{Hager2006} we have that 
\begin{align}
\frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i} \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i). \label{eq:gpa-conv.5}
\end{align}
As $\bar{\alpha}_i \in (0,1)$, we have that $\left( \frac{1}{\bar{\alpha}_i} - 1 \right) > 0$ which combined with (\ref{eq:gpa-conv.5}) yields
\begin{align}
\left( \frac{1}{\bar{\alpha}_i} - 1 \right) \frac{\| \bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i \|^2}{\bar{\alpha}_i} 
&\leq \left( \frac{1}{\bar{\alpha}_i} - 1 \right) \left( - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) \right) \nonumber \\
&= \left( 1 - \frac{1}{\bar{\alpha}_i} \right) \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i). \label{eq:gpa-conv.6}
\end{align}
From (\ref{eq:gpa-conv.4}) and (\ref{eq:gpa-conv.6}) it now follows that
\begin{align}
- \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i) \leq - \frac{1}{\bar{\alpha}_i} \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.7}
\end{align}
As $\bar{\alpha}_i \geq \alpha_{\min}$, (\ref{eq:gpa-conv.2}) and (\ref{eq:gpa-conv.7}) now yield
\begin{align}
\alpha_{\min} \tau \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.8}
\end{align}
Hence, by observing (\ref{eq:gpa-conv.3}) and (\ref{eq:gpa-conv.8}) we have established that for any choice of $\bar{\alpha}_i \in [\alpha_{\min}, \alpha_{\max}]$ there exists a constant $\nu$ such that
\begin{align}
\nu \leq - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, \bar{\alpha}_i) - \bm{u}_i). \label{eq:gpa-conv.9}
\end{align}
Combining (\ref{eq:gpa-conv.1}) and (\ref{eq:gpa-conv.9}) yields
\begin{align}
F (\bm{u}_{i+1}) \leq F_i^r - \delta c \nu \label{eq:gpa-conv.10}
\end{align}
which, by the same argument in the proof of Theorem 2.2 of \cite{Hager2006}, results in a contradiction. Thus, we have
\begin{align*}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0,
\end{align*}
which concludes the proof.
\end{proof}

With this convergence theorem established for the nonmonotone gradient projection algorithm (NGPA) in \cite{Hager2006}, we now provide Algorithm~\ref{alg:pasa-aug-lag} which is PASA with modified stopping and branching criterion designed for the augmented Lagrangian problem (\ref{prob:aug-lag-mod}). The only change here is that we have replaced all instances of $E_{\scaleto{PASA}{4pt}} (\bm{x})$ by the multiplier error estimator.
\begin{center}
\begin{algorithm}
%	\algsetup{linenosize=\notsotiny}
%	\notsotiny
	\caption{Modified PASA Algorithm for GS Augmented Lagrangian Problem} \label{alg:pasa-aug-lag} 
    % Initialize parameters
	{\bfseries Inputs:} Initial guess $\bm{x}_k$ and scalar parameters $\theta \in (0,1)$, $\gamma \in (0,1)$, $\varepsilon > 0$\\
	Set $\bm{u}_{0} = \bm{x}_{k}$, $\bm{u}_1 = \mathcal{P}_{\Omega} (\bm{u}_0)$, and $i = 1$\\
    % Phase one
	\textbf{Phase one}:\\
    \While{$E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > \varepsilon$}{
        Set $\bm{u}_{i+1} \gets GPA(\bm{u}_i)$ and $i \gets i+1$\\
        \If{$\mathcal{U} (\bm{u}_i) = \emptyset$ \textbf{and} $e_{\scaleto{PASA}{4pt}} (\bm{u}_i) < \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
            Set $\theta \gets \gamma \theta$
        }
        \If{$e_{\scaleto{PASA}{4pt}} (\bm{u}_i) \geq \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
    	    \textbf{goto} phase two
        }
    }
    % Phase two 
	\textbf{Phase two}:\\ 
    \While{$E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) > \varepsilon$}{
        Set $\bm{u}_{i+1} \gets LCO(\bm{u}_i)$ and $i \gets i+1$\\
        \If{$e_{\scaleto{PASA}{4pt}} (\bm{u}_i) < \theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1))$}{
       	    \textbf{goto} phase one
        }
    }
    \textbf{Return} $\bm{u}_i$
\end{algorithm}
\end{center}
We now consider a global convergence result for Algorithm~\ref{alg:pasa-aug-lag} which is similar to Theorem 3.2 in \cite{Hager2016}. The benefit to using Algorithm~\ref{alg:pasa-aug-lag} to solve problem (\ref{prob:aug-lag-mod}) instead of the original version of PASA in \cite{Hager2016} is that when using Algorithm~\ref{alg:pasa-aug-lag} we no longer require the additional assumption that the sequence $\{ \bm{u}_i \}_{i=1}^{\infty}$ generated by PASA satisfies (\ref{result:pasa-aug-lag-conv.1}) that was required in Theorem~\ref{thm:pasa-aug-lag} to establish global convergence for the multiplier error.

\begin{theorem} \label{thm:pasa-aug-lag-mod-global-conv}
Suppose that G1 and G2 from Theorem~\ref{thm:pasa-aug-lag} are satisfied. If Algorithm~\ref{alg:pasa-aug-lag} with $\varepsilon = 0$ is used to solve problem (\ref{prob:aug-lag-mod}) then Algorithm~\ref{alg:pasa-aug-lag} either terminates in a finite number of iterations at a stationary point, or generates a sequence of iterates $\{ \bm{u}_i \}_{i=0}^{\infty}$ satisfying
\begin{align}
\liminf_{i \to \infty} E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = 0. \label{result:pasa-aug-lag-mod-global-conv}
\end{align}
\end{theorem}
\begin{proof}
The proof is split into three cases.\\
{\bfseries Case 1: Phase two of Algorithm~\ref{alg:pasa-aug-lag} is executed a finite number of times.} In this case, only phase one of Algorithm~\ref{alg:pasa-aug-lag} is executed for $i$ sufficiently large. As such, from Theorem~\ref{thm:ngpa-conv} it follows that (\ref{result:pasa-aug-lag-mod-global-conv}) holds. \\
{\bfseries Case 2: Phase one of Algorithm~\ref{alg:pasa-aug-lag} is executed a finite number of times.} Here, only phase two is executed for $i$ sufficiently large. Since phase two eventually does not branch back to phase one, by the branching criterion in phase two we have that
\begin{align*}
\theta E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) \leq e_{\scaleto{PASA}{4pt}} (\bm{u}_i)
\end{align*}
for $i$ sufficiently large. Using an argument found in the proof of Theorem 3.2 from \cite{Hager2016} we have that (\ref{result:pasa-aug-lag-mod-global-conv}) holds. \\
{\bfseries Case 3: Phases one and two of Algorithm~\ref{alg:pasa-aug-lag} are executed an infinite number of times.} By way of contradiction, assume that (\ref{result:pasa-aug-lag-mod-global-conv}) does not hold. Then there exists a constant $\tau > 0$ such that 
\begin{align*}
\tau \leq E_{m,0} (\bm{u}_i, \bm{\bar{\lambda}}_k + 2 q \bm{h} (\bm{u}_i), \bm{\mu}(\bm{u}_i,1)) = - \bm{g} (\bm{u}_i)^{\intercal} (\bm{y} (\bm{u}_i, 1) - \bm{u}_i).
\end{align*}
Letting $F (\bm{u}_{i+1}) = \mathcal{L}_q (\bm{u}_{i+1}, \bm{\bar{\lambda}}_k)$ and applying the same argument as in the proof of Theorem~\ref{thm:ngpa-conv}, we have that there exists a constant $\nu$ such that
\begin{align}
F (\bm{u}_{i+1}) \leq F (\bm{u}_i) - \delta c \nu \label{eq:pasa-aug-lag-mod-global-conv.10}
\end{align}
for each iteration of GPA when $i$ is sufficiently large. Additionally, by property F1 of the LCO in \cite{Hager2016}, we have that $F (\bm{u}_{i+1}) \leq F (\bm{u}_i)$. Since there are an infinite number of iterations in phase one, it follows that the cost function is unbounded from below which contradictions assumption G1. Thus, (\ref{result:pasa-aug-lag-mod-global-conv}) holds.
\end{proof}

Based on the analysis in this section, we note that we plan on using Algorithm~\ref{alg:pasa-aug-lag} to solve the augmented Lagrangian problem in the GS algorithm in phase one of NPASA. As we were able to establish a global convergence result for the multiplier error of the original nonlinear program with the same set of assumptions required for global convergence of the PASA error estimator, Algorithm~\ref{alg:pasa-aug-lag} is more suitable for problem (\ref{prob:aug-lag-mod}) than the original version of PASA for solving the nonlinear program.

At this point, we have addressed nearly every step of phase one of NPASA. However, throughout the analysis in this section we have treated $\bm{\mu} (\bm{x}_k, 1)$ as a vector that exists but that is not explicitly known. While the formula for $E_{m,0} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))$ provided in (\ref{eq:aug-lag-mod.4.2}) proved useful in establishing convergence of the augmented Lagrangian problem phase one of NPASA and allows the user to compute an error estimator without requiring the value of $\bm{\mu} (\bm{x}_k,1)$, to establish desirable global convergence properties for NPASA in Section~\ref{section:npasa-global-convergence} we need to compute $E_{m,1} (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k,1))$ at the end of phase one of NPASA. As the vector $\bm{\mu} (\bm{x}_k, 1)$ is required to compute $E_1 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k, 1))$, we now discuss how to construct the vector $\bm{\mu} (\bm{x}_k, 1)$ using information already computed internally by PASA when solving the augmented Lagrangian problem in (\ref{prob:aug-lag-mod}). When checking the stopping criterion for the original PASA algorithm \cite{HagerActive} or for the modified PASA algorithm presented here in Algorithm~\ref{alg:pasa-aug-lag}, it is necessary to solve problem (\ref{prob:pasa-error}) with $\alpha = 1$, restated here as
\begin{align}
\begin{array}{cc}
\min & \displaystyle \frac{1}{2} \| \bm{x} - \bm{g} (\bm{x}) - \bm{y} \|^2 \vspace{2mm}\\
\text{s.t.} & \bm{y} \in \Omega
\end{array} \label{prob:pasa-construct-mult}
\end{align}
where $\bm{x}$ is fixed and we let $\Omega$ be of the general form $\Omega = \{ \bm{y} : \bm{\ell} \leq \bm{A} \bm{y} \leq \bm{u}, \bm{lo} \leq \bm{y} \leq \bm{hi} \}$. In implementation, this problem is solved using a dual technique with the algorithm PPROJ \cite{Hager2016}. From equation (1.5) in \cite{Hager2016} PPROJ computes a solution for the dual variable, which we will denote by $\bm{\pi}^*$, that is used to reconstruct the primal solution, $\bm{y} (\bm{\pi}^*)$. Letting $\bm{a}_i$ denote the $i$th column of $\bm{A}$ and $\bm{a}_j^{\intercal}$ denote the $j$th row of $A$, using equation (1.5) in \cite{Hager2016} we have that this primal solution satisfies
\begin{align}
y_i (\bm{\pi}^*) = \left\{
	\begin{array}{lll}
	lo_i & : & x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* \leq lo_i \vspace{0.8mm} \\
	hi_i & : & x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* \geq hi_i \vspace{0.8mm} \\
    x_i - g_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* & : & \text{otherwise}
	\end{array}
	\right. \label{eq:pasa-construct-mult.1}
\end{align}
and
\begin{align}
\bm{a}_j^{\intercal} \bm{y} (\bm{\pi}^*) = \left\{
	\begin{array}{lll}
	\ell_j & : & \pi_j^* > 0 \\
	u_j & : & \pi_j^* < 0
	\end{array}
	\right., \label{eq:pasa-construct-mult.2}
\end{align}
for $1 \leq i \leq n$ and $1 \leq j \leq m$. Now consider the Lagangian for problem (\ref{prob:pasa-construct-mult}) given by
\begin{align}
L (\bm{y}, \bm{\gamma}_1, \bm{\gamma}_2, \bm{\upsilon}_1, \bm{\upsilon}_2) 
&= \frac{1}{2} \| \bm{x} - \bm{g} (\bm{x}) - \bm{y} \|^2 + \bm{\gamma}_1^{\intercal} (\bm{\ell} - \bm{A} \bm{y}) + \bm{\gamma}_2^{\intercal} (\bm{A} \bm{y} - \bm{u}) \nonumber \\
&\quad + \bm{\upsilon}_1^{\intercal} (\bm{lo} - \bm{y}) + \bm{\upsilon}_2^{\intercal} ( \bm{y} - \bm{hi}). \label{eq:pasa-construct-mult.3}
\end{align}
It follows that
\begin{align}
\nabla_y L (\bm{y}, \bm{\gamma}_1, \bm{\gamma}_2, \bm{\upsilon}_1, \bm{\upsilon}_2)^{\intercal} 
&= \bm{y} - (\bm{x} - \bm{g} (\bm{x}))  - \bm{A}^{\intercal} \bm{\gamma}_1 + \bm{A}^{\intercal} \bm{\gamma}_2 - \bm{\upsilon}_1 + \bm{\upsilon}_2. \label{eq:pasa-construct-mult.4}
\end{align}
%Letting $\bm{y}^* = \bm{y} (\bm{\pi}^*)$, we proceed by partitioning $\bm{y}^*$ into three parts, denoted $\bm{y}_{\mathcal{S}_1}^*$, $\bm{y}_{\mathcal{S}_2}^*$, and $\bm{y}_{\mathcal{S}_3}^*$, where the index sets used to construct the partition of $\bm{y}^*$ are defined by $\mathcal{S}_1 = \{ i \in \mathbb{N} : \bm{y}_i^* = lo_i \}$, $\mathcal{S}_2 = \{ i \in \mathbb{N} : \bm{y}_i^* = hi_i \}$, and $\mathcal{S}_3 = \{ i \in \mathbb{N} : lo_i < \bm{y}_i^* < hi_i \}$. 
Now let $\bm{y}^* = \bm{y} (\bm{\pi}^*)$ and define the index sets $\mathcal{S}_1 = \{ i \in \mathbb{N} : \bm{y}_i^* = lo_i \}$, $\mathcal{S}_2 = \{ i \in \mathbb{N} : \bm{y}_i^* = hi_i \}$, and $\mathcal{S}_3 = \{ i \in \mathbb{N} : lo_i < \bm{y}_i^* < hi_i \}$. Using $\bm{y}^*$, $\bm{\pi}^*$, and the sets $\mathcal{S}_j$, for $j \in \{ 1, 2, 3 \}$, we work to construct multiplier vectors $\bm{\gamma}_1^*$, $\bm{\gamma}_2^*$, $\bm{\upsilon}_1^*$, and $\bm{\upsilon}_2^*$ that satisfy the KKT conditions for problem (\ref{prob:pasa-construct-mult}) given by:
\begin{enumerate}
\item[(M.1)] Gradient of Lagrangian equals zero: $\nabla_y L (\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)^{\intercal} = \bm{0}$
\item[(M.2)] Satisfies problem constraints: $\bm{y}^* \in \Omega$
\item[(M.3)] Nonnegativity of inequality multipliers: $\bm{\gamma}_1^*, \bm{\gamma}_2^* \in \mathbb{R}_{\geq 0}^{m}$ and $\bm{\upsilon}_1^*, \bm{\upsilon}_2^* \in \mathbb{R}_{\geq 0}^{n}$
\item[(M.4)] Complimentary slackness: $(\bm{\ell} - \bm{A} \bm{y}^*)^{\intercal} \bm{\gamma}_1^* = 0$, $(\bm{A} \bm{y}^* - \bm{u})^{\intercal} \bm{\gamma}_2^* = 0$, $(\bm{lo} - \bm{y}^*)^{\intercal} \bm{\upsilon}_1^* = 0$, and $(\bm{y}^* - \bm{hi})^{\intercal} \bm{\upsilon}_2^* = 0$.
\end{enumerate}
Note that (M.2) is already satisfied. First, we define the components of vectors $\bm{\gamma}_1^*$ and $\bm{\gamma}_2^*$ by
\begin{align}
\gamma_{1,j}^* := \left\{
	\begin{array}{cll}
	\pi_j^* & : & \pi_j^* > 0 \\
	0 & : & \text{otherwise}
	\end{array}
	\right. \label{eq:pasa-construct-mult.5}
\end{align}
and
\begin{align}
\gamma_{2,j}^* := \left\{
	\begin{array}{cll}
	-\pi_j^* & : & \pi_j^* < 0 \\
	0 & : & \text{otherwise}
	\end{array}
	\right., \label{eq:pasa-construct-mult.6}
\end{align}
respectively, for $1 \leq j \leq m$. By definition, we have that $\bm{\gamma}_1^*, \bm{\gamma}_2^* \in \mathbb{R}_{\geq 0}^{m}$. Also, it follows from definition that
\begin{align}
\bm{\gamma}_1^* - \bm{\gamma}_2^* 
= \bm{\pi}^*. \label{eq:pasa-construct-mult.6.1}
\end{align}
Additionally, combining (\ref{eq:pasa-construct-mult.2}), (\ref{eq:pasa-construct-mult.5}), and (\ref{eq:pasa-construct-mult.6}) it follows that $(\bm{\ell} - \bm{A} \bm{y}^*)^{\intercal} \bm{\gamma}_1^* = 0$ and $(\bm{A} \bm{y}^* - \bm{u})^{\intercal} \bm{\gamma}_2^* = 0$. Next, we define vectors $\bm{\upsilon}_1^*$ and $\bm{\upsilon}_2^*$ componentwise by
\begin{align}
\upsilon_{1,i}^* := \left\{
	\begin{array}{lll}
	lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^* & : & i \in \mathcal{S}_1 \\
	0 & : & i \in \mathcal{S}_2 \cup \mathcal{S}_3
	\end{array}
	\right. \label{eq:pasa-construct-mult.7}
\end{align}
and
\begin{align}
\upsilon_{2,i}^* := \left\{
	\begin{array}{lll}
	-hi_i + x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^* & : & i \in \mathcal{S}_2 \\
	0 & : & i \in \mathcal{S}_1 \cup \mathcal{S}_3
	\end{array}
	\right., \label{eq:pasa-construct-mult.8}
\end{align}
respectively. By the definition of $\mathcal{S}_1$ and (\ref{eq:pasa-construct-mult.1}), we have that
\begin{align}
lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^* \geq 0, \quad \text{for all $i \in \mathcal{S}_1$.} \label{eq:pasa-construct-mult.9}
\end{align}
As $\upsilon_{1,i}^* = 0$ for $i \in \mathcal{S}_2 \cup \mathcal{S}_3$ it now follows that $\bm{\upsilon}_1^* \in \mathbb{R}_{\geq 0}^{n}$. Similarly, by the definition of $\mathcal{S}_2$ and (\ref{eq:pasa-construct-mult.1}) it follows that
\begin{align}
-hi_i + (x_i - \bm{g}_i (\bm{x})) + \bm{a}_i^{\intercal} \bm{\pi}^* \geq 0, \quad \text{for all $i \in \mathcal{S}_2$.} \label{eq:pasa-construct-mult.10}
\end{align}
As $\upsilon_{2,i}^* = 0$ for $i \in \mathcal{S}_1 \cup \mathcal{S}_3$ it now follows that $\bm{\upsilon}_2^* \in \mathbb{R}_{\geq 0}^{n}$. Hence, (M.3) holds. Next, combining (\ref{eq:pasa-construct-mult.2}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) it follows that $(\bm{lo} - \bm{y}^*)^{\intercal} \bm{\upsilon}_1^* = 0$ and $(\bm{y}^* - \bm{hi})^{\intercal} \bm{\upsilon}_2^* = 0$. Hence, (M.4) holds. Lastly, it remains to show that (M.1) holds. Combining (\ref{eq:pasa-construct-mult.4}) and (\ref{eq:pasa-construct-mult.6.1}) we have that
\begin{align}
\nabla_y L (\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)^{\intercal} 
&= \bm{y}^* - (\bm{x} - \bm{g} (\bm{x}))  - \bm{A}^{\intercal} \bm{\pi}^* - \bm{\upsilon}_1^* + \bm{\upsilon}_2^*. \label{eq:pasa-construct-mult.11}
\end{align}
To show that (M.1) holds, we need to show that
\begin{align}
\bm{y}_i^* - (x_i - \bm{g}_i (\bm{x}))  - \bm{a}_i^{\intercal} \bm{\pi}^* - \upsilon_{1,i}^* + \upsilon_{2,i}^*
&= 0. \label{eq:pasa-construct-mult.12}
\end{align}
for $1 \leq i \leq n$. Accordingly, fix $i \in \{1, 2, \ldots, n \}$. Suppose $i \in \mathcal{S}_1$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = lo_i$, $\upsilon_{1,i}^* = lo_i - (x_i - \bm{g}_i (\bm{x})) - \bm{a}_i^{\intercal} \bm{\pi}^*$, and $\upsilon_{2,i}^* = 0$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_1$. Next suppose $i \in \mathcal{S}_2$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = hi_i$, $\upsilon_{1,i}^* = 0$, and $\upsilon_{2,i}^* = -hi_i + x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^*$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_2$. Lastly, suppose $i \in \mathcal{S}_3$. Then using (\ref{eq:pasa-construct-mult.1}), (\ref{eq:pasa-construct-mult.9}), and (\ref{eq:pasa-construct-mult.10}) we have that $\bm{y}_i^* = x_i - \bm{g}_i (\bm{x}) + \bm{a}_i^{\intercal} \bm{\pi}^*$, $\upsilon_{1,i}^* = 0$, and $\upsilon_{2,i}^* = 0$, respectively. Hence, (\ref{eq:pasa-construct-mult.12}) holds for $i \in \mathcal{S}_3$. As $\mathcal{S}_1 \cup \mathcal{S}_2 \cup \mathcal{S}_3 = \{ 1, 2, \ldots, n \}$, we conclude that (M.1) holds. Thus, $(\bm{y}^*, \bm{\gamma}_1^*, \bm{\gamma}_2^*, \bm{\upsilon}_1^*, \bm{\upsilon}_2^*)$ is a KKT point for problem (\ref{prob:pasa-construct-mult}). As our goal was to construct the inequality multiplier $\bm{\mu} (\bm{x}, 1)$, we now note that $\bm{y}^* = \bm{y} (\bm{x}^*, 1)$. Hence, when the polyhedral constraints for the original problem are in the standard format
\begin{align}
\bm{r} (\bm{x}) = \begin{bmatrix}
\bm{\ell} - \bm{A} \bm{x} \\
\bm{A} \bm{x} - \bm{u} \\
\bm{lo} - \bm{x} \\
\bm{x} - \bm{hi}
\end{bmatrix} \nonumber
\end{align}
then it follows that we should construct $\bm{\mu} (\bm{x}^*, 1)$ by
\begin{align}
\bm{\mu} (\bm{x}^*, 1) := \begin{bmatrix}
\bm{\gamma}_1^* \\ 
\bm{\gamma}_2^* \\
\bm{\upsilon}_1^* \\
\bm{\upsilon}_2^*
\end{bmatrix}. \label{eq:pasa-construct-mult.13}
\end{align}
As $\bm{y}^*$ and $\bm{\pi}^*$ are available when completing PPROJ, we can always perform this construction. Note that this construction only needs to be performed once after terminating PASA in phase one since we only need $\bm{\mu} (\bm{x}_k, 1)$ to compute $E_1 (\bm{x}_k, \bm{\lambda}_k, \bm{\mu} (\bm{x}_k, 1))$ at the end of phase one. 

With this construction completed, we have addressed all of the necessary steps for implementing phase one of NPASA as outlined in Algorithms~\ref{alg:gs} and \ref{alg:npasa}. We now turn our attention to phase two of NPASA.


==> local-phase-two-no-A.tex <==
\section{Convergence Analysis for Phase Two of NPASA} \label{section:npasa-phase-two}
In this section, we provide conditions under which phase two of NPASA satisfies desirable local convergences properties. From the pseodocode of Algorithm~\ref{alg:npasa}, recall that phase two of NPASA consists of the constraint and multiplier steps. First, we prove fast local convergence properties of the constraint step in Section~\ref{subsec:constraint-step-analysis}. Then we provide a local convergence analysis of the multiplier step of NPASA in Section~\ref{subsec:multiplier-step-analysis}. Lastly, we use our analysis of both steps to provide a local convergence result for the CMS algorithm in Section~\ref{subsec:npasa-phase-two-local-conv}. 
%To establish our convergence result we make use of some sensitivity analysis from \cite{Robinson} which require the following assumptions:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For several results in this section we will require some subset of the assumptions (\textbf{LI}), (\textbf{SCS}), (\textbf{SOSC}), and (\textbf{SSOSC}) provided in Section~\ref{section:introduction}. We will clearly specify which assumptions are used in the statement of each convergence result. Additionally, note that for the purposes of simplifying the analysis for several results in Sections~\ref{subsec:constraint-step-analysis} and \ref{subsec:multiplier-step-analysis}, we will express the polyhedral constraint set for problem (\ref{prob:main-nlp}), originally defined by $\Omega = \{ \bm{x} : \bm{r}(\bm{x}) \leq \bm{0} \}$, in an equivalent form $\Omega = \{ \bm{x} : \bm{g} (\bm{x}) = \bm{0} \}$, for some function $\bm{g} (\bm{x})$. Note that this equivalent formulation of $\Omega$ can be constructed by adding a slack variable to the inequality constraints in problem (\ref{prob:main-nlp}) and performing a change of variables to define $\bm{g} (\cdot)$, as illustrated in Section 3.3.2 of \cite{bertsekas1995nonlinear}. Further, using this approach we have that $\nabla \bm{g}(\bm{x})$ is of full row rank provided that $\bm{A}$ is of full row rank. It should be noted that in the actual implementation of this method we will still use the definition of the set $\Omega$ as originally defined in Section~\ref{section:introduction}.% so that problem %(\ref{NewtonYScheme}) 
%in line 5 of Algorithm~\ref{alg:cms}, the CMS algorithm, can be solved using PPROJ \cite{Hager2016}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ------------- INFEASIBILITY DETECTION FOR CONSTRAINT STEP ------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithm with Infeasibility Detection for Solving Constraint Step} \label{subsec:infeas}
\iffalse
In order to simplify the notation in our discussion of this problem, we express the linearized constraint set as
\begin{align*}
\left\{ \bm{w} \in \mathbb{R}^n : \bm{M} (\bm{w} - \bar{\bm{w}}) = \bm{c}, \bm{w} \geq \bm{0} \right\}
\end{align*}
supposing that we are given $\bm{M} \in \mathbb{R}^{m \times n}$, $\bm{c} \in \mathbb{R}^m$, and $\bar{\bm{w}} \in \mathbb{R}^n$. Ideally, we would like to determine the solution to the problem 
\begin{align}
&\min_{\bm{w} \in \mathcal{S}} \ \frac{1}{2} \| \bm{w} - \bar{\bm{w}} \|^2, \label{Sprob}
\end{align}
%\begin{align}
%&\min_{x \geq 0} \ \frac{1}{2} \| b - A(x - \bar{x}) \|^2, \label{FeasibilityProb}
%\end{align}
%%%given $A$, $b$, and $\bar{x}$. 
%Ideally, if we knew a solution to problem (\ref{FeasibilityProb}) then we would know whether or not $\mathcal{F}_0 = \emptyset$ since $\mathcal{F}_0 = \emptyset$ if and only if $\| b - A(x - \bar{x}) \| > 0$ for all $x \geq 0$. 
where $\mathcal{S} = \arg\min_{\bm{w} \geq \bm{0}} \left\{ \| \bm{c} - \bm{M} (\bm{w} - \bar{\bm{w}}) \|^2 \right\}$. Since problem (\ref{Sprob}) involves minimizing a strongly convex objective function over a convex set, there exists a unique solution which we will denote by $\bm{w}_{\infty}$. As such, every search direction from $\bm{w}_{\infty}$ leading to a point in $\mathcal{S}$ must be an ascent direction. Hence, the first order optimality conditions for $\bm{w}_{\infty}$ can be expressed as 
\begin{align}
\langle \bm{w}_{\infty} - \bar{\bm{w}}, \bm{w} - \bm{w}_{\infty} \rangle \geq 0, \ \text{for all} \ \bm{w} \in \mathcal{S}. \label{problemS}
\end{align}
Since determining elements of the constraint set for problem (\ref{Sprob}) requires knowing all minimizers of $\| \bm{c} - \bm{M}(\bm{w} - \bar{\bm{w}}) \|$ we consider an alternative problem. 

First, we define the sets 
\begin{align*}
\mathcal{F}_{\delta} = \left\{ 
\begin{bmatrix}
\bm{w} \\
\bm{y}
\end{bmatrix} \in \mathbb{R}^{n+m} : \bm{M}(\bm{w} - \bar{\bm{w}}) + \bm{y} = \bm{c}, \bm{w} \geq \bm{0}, \| \bm{y} \|^2 \leq \delta \right\}
\end{align*}
and 
\begin{align*}
\mathcal{F} = \left\{ 
\begin{bmatrix}
\bm{w} \\
\bm{y}
\end{bmatrix} \in \mathbb{R}^{n+m} : \bm{M}(\bm{w} - \bar{\bm{w}}) + \bm{y} = \bm{c}, \bm{w} \geq \bm{0} \right\}.
\end{align*}
Now, given a penalty parameter $p > 0$, we define the problem
\begin{align}
\min_{[\bm{w}, \bm{y}] \in \mathcal{F}} \ \ f_p(\bm{w},\bm{y}) := \frac{1}{2} \| \bm{w} - \bar{\bm{w}} \|^2 + \frac{p}{2} \| \bm{y} \|^2. \label{prob:Pp}
\end{align}
Since problem (\ref{prob:Pp}) involves minimizing a strongly convex objective function over a convex set, it has a unique solution which we will denote by $[ \bm{w}_p, \bm{y}_p]^{\intercal}$. Note that the first order optimality conditions for $[ \bm{w}_p, \bm{y}_p ]^{\intercal}$ can be expressed as
\begin{align}
\langle \bm{w}_p - \bar{\bm{w}}, \bm{w} - \bm{w}_p \rangle + p \langle \bm{y}_p, \bm{y} - \bm{y}_p \rangle \geq 0, \ \text{for all} \ [\bm{w}, \bm{y}]^{\intercal} \in \mathcal{F}. \label{POptCond}
\end{align}
We should note here that while the number of primal variables in (\ref{prob:Pp}) is greater than that of problem (\ref{Sprob}), the dimension of the dual variables is the same for problems (\ref{Sprob}) and (\ref{prob:Pp}). So we can use PPROJ \cite{Hager2016} to solve for problem (\ref{prob:Pp}) without the cost of solving for additional dual variables.
%%%That is, the complexity is the same for solving (P) and (\ref{prob:Pp}) using PPROJ \cite{Hager2016}. 
The following result provides valuable insight on the relationship between $\bm{w}_p$ and $\bm{w}_{\infty}$. 

\begin{theorem} \label{thm:feasibility-detection}
Let $[\bm{w}_p, \bm{y}_p]^{\intercal}$ be the unique solution to problem \emph{(\ref{prob:Pp})}. Then 
\begin{align*}
\| \bm{w}_p - \bm{x}_{\infty} \| = O \left( \frac{1}{p} \right),
\end{align*}
for all $p > 0$ sufficiently large.
%%%where $x_{\infty} \in \mathcal{S}$ is the closest solution to $\bar{x}$.	
\end{theorem}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ----------------------- CONSTRAINT STEP ANALYSIS ---------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Analysis for Constraint Step} \label{subsec:constraint-step-analysis}
In this section, we establish a local quadratic convergence rate of the multiplier error estimator $E_c$. Recall the iterative scheme for determining $\bm{w} \in \Omega$ such that $\bm{h} (\bm{w}) = \bm{0}$ used in the constraint step of the CMS algorithm:
\begin{align}
(\bm{w}_{i+1}, \bm{y}_{i+1}) &= \arg\min \left\{\| \bm{w} - \bm{w}_i \|^2 + \| \bm{y} \|^2 : \nabla \bm{h} (\bm{w}_i) (\bm{w} - \bm{w}_i) + \frac{1}{\sqrt{p_i}} \bm{y} = - \bm{h} (\bm{w}_i), \bm{w} \in \Omega \right\} \label{NewtonYScheme} \\
\bm{w}_{i+1} &\gets \bm{w}_i + s_i ( \bm{w}_{i+1} - \bm{w}_i) \nonumber 
\end{align}
where $p_i \geq 1$ is a penalty parameter and where $s_i \leq 1$ is chosen such that
\begin{align}
\| \bm{h} (\bm{w}_i + s_i (\bm{w}_{i+1} - \bm{w}_{i})) \| \leq (1 - \tau \alpha_i s_i) \| \bm{h} (\bm{w}_i) \|. \label{NewtonArmijo}
\end{align} 
Here, $\alpha_i$ is defined by $\alpha_i := 1 - \| \bm{y}_i \|$ and to continue performing the scheme we require that $\alpha_i \in [\alpha, 1]$ for some fixed parameter $\alpha > 0$. Note that this is the iterative scheme in the constraint step of the CMS algorithm, Algorithm~\ref{alg:cms}, where we have made the change of variables $\bm{y} \gets \frac{1}{\sqrt{p_i}} \bm{y}$ to simplify the analysis in Theorem~\ref{NewtonYSchemeThm}. By introducing the slack variable, $\bm{y}$, into our update scheme, it is no longer necessary to consider the solvability of this problem as the constraint set is always nonempty. However, Theorem~\ref{NewtonYSchemeThm} serves to update the convergence analysis performed in Theorem 2.1 of \cite{Hager1993} to account for the presence of the slack variable $\bm{y}$ and penalty parameter $p_i$ in (\ref{NewtonYScheme}). 

\begin{theorem} \label{NewtonYSchemeThm}
Suppose $\bm{x}^*$ satisfies $\bm{h} (\bm{x}^*) = \bm{0}$, $\bm{g} (\bm{x}^*) = \bm{0}$, $\bm{g}, \bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and that assumption (\textbf{LI}) holds at $\bm{x}^*$. Then there exists a neighborhood $\mathcal{N}$ about $\bm{x}^*$ and a constant $c \in \mathbb{R}$ such that for any $\bm{w}_0 \in \mathcal{N} \cap \Omega$ and sequence of penalty parameters $\{ p_i \}_{i = 0}^{\infty}$ satisfying $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, with $\beta \geq 1$, the iterative scheme (\ref{NewtonYScheme}) converges to a point $\bm{w}^*$ with the following properties: 
\iffalse
\begin{itemize}
\item[(\ref{NewtonYSchemeThm}.0)] $\bm{h}(\bm{w}^*) = \bm{g}(\bm{w}^*) = \bm{0}$ and $s_i = 1$ satisfies the Armijo line search given by (\ref{NewtonArmijo}) for each $i$.
\end{itemize}
\fi
\begin{align}
\bm{h}(\bm{w}^*) = \bm{g}(\bm{w}^*) = \bm{0} \ \text{and} \ s_i = 1 \ \text{satisfies Armijo line search given by (\ref{NewtonArmijo}) for each $i$}. \label{NewtonYSchemeThm.0}
\end{align}
Moreover, for all $i \geq 0$:
\iffalse
\begin{itemize}
\item[(\ref{NewtonYSchemeThm}.1)] $\| \bm{w}_i - \bm{w}_0 \| \leq c \| \bm{h}(\bm{w}_0) \|$
\item[(\ref{NewtonYSchemeThm}.2)] $\| \bm{w}_i - \bm{w}^* \| \leq c \| \bm{h}(\bm{w}_0) \| 2^{-2^i}$
\item[(\ref{NewtonYSchemeThm}.3)] $\| \bm{h}(\bm{w}_{i+1}) \| \leq c \| \bm{h}(\bm{w}_i) \|^2$.
\end{itemize}
\fi
\begin{align}
\| \bm{w}_i - \bm{w}_0 \| &\leq c \| \bm{h}(\bm{w}_0) \|, \label{NewtonYSchemeThm.1} \\
\| \bm{w}_i - \bm{w}^* \| &\leq c \| \bm{h}(\bm{w}_0) \| 2^{-2^i}, \label{NewtonYSchemeThm.2} \\
\| \bm{h}(\bm{w}_{i+1}) \| &\leq c \| \bm{h}(\bm{w}_i) \|^2. \label{NewtonYSchemeThm.3}
\end{align}
\end{theorem} 

\begin{proof}
Define $\bm{F}_p: \mathbb{R}^{m + 2 \ell} \times \mathbb{R}^{n} \to \mathbb{R}^{m + 2 \ell}$ by
\begin{align}
\bm{F}_p (\bm{u}, \bm{y}, \bm{x}) = \begin{bmatrix}
\nabla \bm{h} (\bm{x}) \bm{M}(\bm{x}) \bm{u} + \frac{1}{\sqrt{p}} \bm{y} + \bm{h} (\bm{x}) \\
\bm{g} \left( \bm{x} + \bm{M}(\bm{x}) \bm{u} \right) \\
\bm{y}
\end{bmatrix}
\end{align}
where $\bm{u} \in \mathbb{R}^{\ell + m}$, $\bm{y} \in \mathbb{R}^{\ell}$, $\bm{M}(\bm{x}) = \left[ \nabla \bm{h} (\bm{x})^{\intercal} \ \vert \ \nabla \bm{g} (\bm{x})^{\intercal} \right] \in \mathbb{R}^{n \times (\ell + m)}$, and $p \geq 1$ is a scalar. Evaluating the Jacobian of $\bm{F}_p$ with respect to $[\bm{u}, \bm{y}]$ at $\bm{u} = \bm{0}$, $\bm{y} = \bm{0}$, and $\bm{x} = \bm{x}^*$ yields
\begin{align}
\nabla_{[u, y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) 
&= \begin{bmatrix}
\nabla_{u} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) \ \vert \ \nabla_{y} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*)
\end{bmatrix}
= \left[
\begin{array}{c|c}
\multirow{2}{*}{$\bm{M}(\bm{x}^*)^{\intercal} \bm{M}(\bm{x}^*)$} & \frac{1}{\sqrt{p}} \bm{I}_{\ell} \\
 & \bm{0} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right]
\end{align}
which is nonsingular by our hypothesis and choice of $\bm{M}(\bm{x})$. Note that $\bm{I}_{\ell}$ denotes the identity matrix of dimension $\ell \times \ell$. Hence, by the Implicit Function Theorem, there exist neighborhoods $\mathcal{N}_1$ of $[\bm{0}, \bm{0}]$ and $\mathcal{N}_2$ of $\bm{x}^*$ such that the equation 
\begin{align}
\bm{F}_p (\bm{u}, \bm{y}, \bm{x}) = \bm{0}
\end{align}
has a unique solution $[\bm{u}, \bm{y}] = [\bm{u}_p (\bm{x}), \bm{y}_p (\bm{x})]$ in $\mathcal{N}_1$ for every $\bm{x} \in \mathcal{N}_2$. In particular, by our definition of $\bm{F}_p$ it follows that $\bm{y}_p(\bm{x}) = \bm{0}$ for every $\bm{x} \in \mathcal{N}_2$. In order to use Theorem 2.1 of \cite{Robinson1980}, we need prove that the Lipschitz constant of $\nabla_{[u, y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*)^{-1}$ is uniformly bounded for sufficiently large values of $p$. For simplicity, define $\bm{B}_p := \nabla_{[u, y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*)^{-1}$, $\bm{C} := \left( \bm{M}(\bm{x}^*)^{\intercal} \bm{M}(\bm{x}^*)\right)^{-1}$, and 
\begin{align}
\bm{D} := \bm{C} \begin{bmatrix}
\bm{I}_{\ell} \\
\bm{0}
\end{bmatrix}
\end{align} 
and observe that 
\begin{align}
\bm{B}_p = \left[
\begin{array}{c|c}
\bm{C} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right].
\end{align}
As the desired Lipschitz constant is given by $\| \bm{B}_p \|$, it suffices to determine the singular values of $\bm{B}_p$. Since 
\begin{align}
\bm{B}_p \bm{B}_p^{\intercal} &= \left[
\begin{array}{c|c}
\bm{C} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right] \left[
\begin{array}{c|c}
\bm{C}^{\intercal} & \bm{0} \\
\hline 
\frac{1}{\sqrt{p}} \bm{D}^{\intercal} & \bm{I}_{\ell}
\end{array}
\right]
= \left[
\begin{array}{c|c}
\bm{C} \bm{C}^{\intercal} + \frac{1}{p} \bm{D} \bm{D}^{\intercal} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline 
\frac{1}{\sqrt{p}} \bm{D}^{\intercal} & \bm{I}_{\ell}
\end{array}
\right]
\end{align}
we have that
\begin{align}
\lim_{p \to \infty} \bm{B}_p \bm{B}_p^{\intercal} = \left[
\begin{array}{c|c}
\bm{C} \bm{C}^{\intercal} & \bm{0} \\
\hline 
\bm{0} & \bm{I}_{\ell}
\end{array}
\right]. \label{NewtonYThm.3}
\end{align}
As the matrix in (\ref{NewtonYThm.3}) is a block diagonal matrix, its eigenvalues are the eigenvalues of $\bm{C} \bm{C}^{\intercal}$ and $\bm{I}_{\ell}$. As the nonzero singular values of $\bm{B}_p$ are the square roots of the nonzero eigenvalues of $\bm{B}_p \bm{B}_p^{\intercal}$, we conclude that the singular values of $\bm{B}_p$ are uniformly bounded for sufficiently large $p$. Thus, by Theorem 2.1 of \cite{Robinson1980} and the fact that $\bm{y}_p (\bm{x}) = \bm{0}$ for all $\bm{x} \in \mathcal{N}_2$, the solution $\bm{u}_p (\bm{x})$ satisfies the inequality
\begin{align}
\| \bm{u}_p (\bm{x}) \| &= \| [ \bm{u}_p (\bm{x}), \ \bm{y}_p (\bm{x}) ] \| \leq \sigma \| \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) - \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) \|
\end{align}
for all $\bm{x} \in \mathcal{N}_2$ and sufficiently large $p$, where $\sigma$ is independent of $\bm{x}$ and $p$. Observing that
\begin{align}
\bm{F}_p (\bm{0}, \bm{0}, \bm{x}) &= \begin{bmatrix}
\nabla \bm{h} (\bm{x}) \bm{M}(\bm{x}) \bm{0} + \frac{1}{\sqrt{p}} \bm{0} + \bm{h} (\bm{x}) \\
\bm{g} \left( \bm{x} + \bm{M}(\bm{x}) \bm{0} \right) \\
\bm{0}
\end{bmatrix} = \begin{bmatrix}
\bm{h} \left( \bm{x} \right) \\
\bm{g} \left( \bm{x} \right) \\
\bm{0}
\end{bmatrix}
\end{align}
and
\begin{align}
\bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) &= \begin{bmatrix}
\bm{h} \left( \bm{x}^* \right) \\
\bm{g} \left( \bm{x}^* \right) \\
\bm{0}
\end{bmatrix} = \begin{bmatrix}
\bm{0} \\
\bm{0} \\
\bm{0}
\end{bmatrix}
\end{align}
we now have that
\begin{align}
\| \bm{u}_p (\bm{x}) \| &\leq \sigma \left\| \begin{bmatrix}
\bm{h} \left( \bm{x} \right) \\
\bm{g} \left( \bm{x} \right)
\end{bmatrix} \right\| \label{NewtonYThm.4}
\end{align}
for all $\bm{x} \in \mathcal{N}_2$.

Now let $\eta >0$ be given such that $\bm{h}, \bm{g} \in \mathcal{C}^2 (\mathcal{B} (\bm{x}^*, \eta))$ and $\mathcal{B} (\bm{x}^*, \eta) \subset \mathcal{N}_2$. Define $\mathcal{B} := \mathcal{B} (\bm{x}^*, \eta)$. Let
\begin{align}
\eta &= \max \left\{ \max_{\bm{x} \in \mathcal{B}} \| \bm{M}(\bm{x}) \|, 1 \right\}, \\
\delta &= \left[ \sum_{j = 1}^{\ell} \max_{\bm{x}_j \in \mathcal{B}} \| \nabla^2 \bm{h}_j ( \bm{x}_j ) \|^2 \right]^{1/2},
\end{align} 
and let $\bm{w}_0 \in \mathcal{B} \cap \Omega$ be any point such that both
\begin{align}
\eta \sigma \gamma \| \bm{h}(\bm{w}_0) \| \leq \min \left\{ 1/2, 1 - \tau, \gamma (1 - \alpha) \right\} \label{NewtonYThm.4.1}
\end{align}
and $\mathcal{B} ( \bm{w}_0, 2 \eta \sigma \gamma \| \bm{h}(\bm{w}_0) \|) \subseteq \mathcal{B} \cap \Omega$, where $\displaystyle \gamma = \left( 1 + \frac{\delta \eta \sigma}{2} \right)$.

Suppose that $\bm{w}_i \in \mathcal{B} \cap \Omega$ and that $\bm{w}_{i+1}$ is generated using the scheme in (\ref{NewtonYScheme}) with $p_i$ chosen such that $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, for some $\beta > 1$, and with $s_i = 1$. By our definition of $\bm{F}_p (\bm{u}, \bm{y}, \bm{x})$ and the fact that $\bm{F}_{p_i} (u_{p_i} (\bm{w}_i), \bm{0}, \bm{w}_i) = \bm{0}$, we have that 
\begin{align}
\nabla \bm{h} (\bm{w}_i) \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) = - \bm{h} (\bm{w}_i)
\end{align}
and
\begin{align}
\bm{g} \left(\bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \right) = \bm{0} 
\ \ \ \ \Longleftrightarrow \ \ \ \ 
\bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \in \Omega.
\end{align}
So we have that the vector %$\left[ M(\bm{w}_i) u_{p_i} (\bm{w}_i), v_{p_i} (\bm{w}_i) \right]$ 
$\begin{bmatrix} \bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i), \ \bm{0} \end{bmatrix}^{\intercal}$ satisfies the constraints of the minimization problem in (\ref{NewtonYScheme}). Hence, the objective value of problem (\ref{NewtonYScheme}) at a solution is bounded above by the objective evaluated at $\begin{bmatrix} \bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i), \ \bm{0} \end{bmatrix}^{\intercal}$. Using this fact with the definition of $\eta$ and inequality (\ref{NewtonYThm.4}) we have that
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \|^2 + \| \bm{y}_{i+1} \|^2 
&\leq \| \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \|^2
\leq \eta^2 \| \bm{u}_{p_i} (\bm{w}_i) \|^2
\leq \eta^2 \sigma^2 \left\| \bm{h}(\bm{w}_i) \right\|^2. \label{NewtonYThm.4.1.1}
\end{align}
In particular, recalling that $\alpha_i := 1 - \| \bm{y}_i \|$, it follows from (\ref{NewtonYThm.4.1.1}) that
\begin{align}
1 - \eta \sigma \| \bm{h} (\bm{w}_i) \| \leq \alpha_{i+1}. \label{NewtonYThm.4.1.2}
\end{align}

Now suppose that $\bm{w}_i, \bm{w}_{i+1} \in \mathcal{B}$ where $\bm{w}_{i+1}$ is generated using the scheme in (\ref{NewtonYScheme}) with $p_i$ chosen such that $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, for some $\beta > 1$, and with $s_i = 1$. In particular, since $\bm{w}_i$ is known at the time of choosing $p_i$ we can take
\begin{align}
p_i = \max \left\{ \beta^2, \frac{1}{\| \bm{h}(\bm{w}_i) \|^2} \right\} \label{NewtonYThm.4.2}
\end{align}
for some $\beta \geq 1$ to satisfy this requirement. By Taylor's Theorem and the problem constraint, we have that 
\begin{align}
\bm{h}(\bm{w}_{i+1}) &= \bm{h} (\bm{w}_i) + \nabla \bm{h} (\bm{w}_i) (\bm{w}_{i+1} - \bm{w}_i) + \frac{1}{2} \sum_{j = 1}^{\ell} ( \bm{w}_{i+1} - \bm{w}_i )^{\intercal} \nabla^2 \bm{h}_j (\bm{\xi}_j) ( \bm{w}_{i+1} - \bm{w}_i ) \bm{e}_j, \\
&= - \frac{1}{\sqrt{p_i}} \bm{y}_{i+1} + \frac{1}{2} \sum_{j = 1}^{\ell} ( \bm{w}_{i+1} - \bm{w}_i )^{\intercal} \nabla^2 \bm{h}_j (\bm{\xi}_j) ( \bm{w}_{i+1} - \bm{w}_i ) \bm{e}_j,
\end{align}
for some vectors $\bm{\xi}_j$ between $\bm{w}_i$ and $\bm{w}_{i+1}$, for $1 \leq j \leq \ell$. This yields the inequality
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \frac{1}{\sqrt{p_i}} \| \bm{y}_{i+1} \| + \frac{\delta}{2} \| \bm{w}_{i+1} - \bm{w}_i \|^2. \label{NewtonYThm.5}
\end{align}
Combining (\ref{NewtonYThm.5}) with inequality (\ref{NewtonYThm.4.1.1}) yields
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \frac{ \eta \sigma}{\sqrt{p_i}} \left\| \bm{h}(\bm{w}_i) \right\| + \frac{ \delta \eta^2 \sigma^2}{2} \left\| \bm{h}(\bm{w}_i) \right\|^2. \label{NewtonYThm.6}
\end{align}
By our choice of $p_i$ in (\ref{NewtonYThm.4.2}), we have that $\frac{1}{\sqrt{p_i}} \leq \| \bm{h} (\bm{w}_i) \|$. Combining this with (\ref{NewtonYThm.6}) yields
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \eta \sigma \left( 1 + \frac{\delta \eta \sigma}{2} \right) \left\| \bm{h}(\bm{w}_i) \right\|^2 = \eta \sigma \gamma \left\| \bm{h}(\bm{w}_i) \right\|^2, \label{NewtonYThm.7}
\end{align}
which concludes the proof of (\ref{NewtonYSchemeThm.3}).

It remains to show that the sequence of iterates $\{ \bm{w}_i \}_{i = 0}^{\infty}$ generated by (\ref{NewtonYScheme}) is contained in the ball $\mathcal{B}$ and that $\alpha_i \geq \alpha$, for all $i \geq 1$. We proceed by way of induction. First, $\bm{w}_0 \in \mathcal{B}$ by definition. Additionally, using (\ref{NewtonYThm.4.1.2}) and (\ref{NewtonYThm.4.1}) we have that
\begin{align}
\alpha_1
\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_0) \|
\geq \alpha.
\end{align} 
Hence, the base case of induction holds. Suppose now that $\bm{w}_0, \bm{w}_1, \ldots, \bm{w}_i$ are contained in $\mathcal{B}$, that $\| \bm{w}_{i} - \bm{w}_{i-1} \| \leq \eta \sigma \| \bm{h}( \bm{w}_0 ) \| 2^{-2^{i-1} + 1}$, and that $s_j = 1$ and $\alpha_{j+1} \geq 0$, for $0 \leq j < i$. As the inequality in (\ref{NewtonYThm.7}) holds for $\bm{w}_0, \bm{w}_1, \ldots, \bm{w}_i$ by the inductive hypothesis, repeated applications of (\ref{NewtonYThm.7}) yield
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \| &\leq \eta \sigma \left\| \bm{h}(\bm{w}_i) \right\| \leq \frac{1}{\gamma} \left( \eta \sigma \gamma \| \bm{h}( \bm{w}_0 ) \| \right)^{2^i} = \eta \sigma \| \bm{h}( \bm{w}_0 ) \| \left( \eta \sigma \gamma \| \bm{h}( \bm{w}_0 ) \| \right)^{2^i - 1}. \label{NewtonYThm.8}
\end{align}
By our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}), it follows from (\ref{NewtonYThm.8}) that
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \| &\leq \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\| 2^{-2^i + 1}, \label{NewtonYThm.8.1}
\end{align}
as desired. Next, observe that (\ref{NewtonYSchemeThm.1}) follows from applying (\ref{NewtonYThm.8.1}), the inductive hypothesis, and the triangle inequality
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_0 \| = \| \bm{w}_{i+1} - \bm{w}_i + \bm{w}_i - \bm{w}_0 \| &\leq \| \bm{w}_{i+1} - \bm{w}_i \| + \| \bm{w}_{i} - \bm{w}_0 \| \\
&\leq \sum_{j = 0}^{i} \| \bm{w}_{j+1} - \bm{w}_j \| \\
&\leq \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\| \sum_{j = 0}^{i} 2^{-2^j + 1} \\
&< 2 \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\|.
\end{align}
Additionally, observe that
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| &\leq \eta \sigma \| \bm{h}(\bm{w}_i) \|^2 \leq \left( \eta \sigma \| \bm{h}(\bm{w}_0) \| \right)^{2^i} \| \bm{h}(\bm{w}_i) \| \leq \left( 1 - \tau \right) \| \bm{h}(\bm{w}_i) \|, \label{NewtonYThm.9}
\end{align}
where the final inequality holds from our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}). By our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}), we have that
\begin{align}
\eta \sigma \| \bm{h} (\bm{w}_0) \| 2^{-2^i + 1} \leq 1 - \alpha, \label{NewtonYThm.9.1}
\end{align}
for all $i \geq 0$. Hence,
\begin{align}
\alpha_{i+1} 
&\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_i) \| \tag{Using (\ref{NewtonYThm.4.1.2})} \\
&\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_0) \| 2^{-2^i + 1} \tag{Using (\ref{NewtonYThm.8})} \\
&\geq \alpha, \tag{Using (\ref{NewtonYThm.9.1})}
\end{align}
as desired. As $\alpha_{i+1} \leq 1$ by definition, we have $\alpha_{i+1} \in [\alpha, 1]$. Hence, $1 - \tau \leq 1 - \tau \alpha_i \leq 1 - \tau \alpha$. Combining this with (\ref{NewtonYThm.9}) yields that the Armijo line search update in (\ref{NewtonArmijo}) is satisfied for $s_i = 1$. This concludes the inductive phase of the proof.

Lastly, as $1 - \tau \leq 1 - \tau \alpha$ we have that
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| 
&\leq \left( 1 - \tau \alpha \right) \| \bm{h}(\bm{w}_i) \|, \label{NewtonYThm.10}
\end{align}
holds for all $i \geq 0$. Hence the sequence $\{ \bm{w}_i \}_{i = 0}^{\infty}$ is Cauchy so there exists a vector $\bm{w}^* \in \mathcal{B}$ such that $\bm{w}_i \to \bm{w}^*$ as $i \to \infty$ which, combined with (\ref{NewtonYThm.9}), yields the inequality in (\ref{NewtonYSchemeThm.2}). Lastly, as $\tau \in (0,1)$, it follows from (\ref{NewtonYThm.10}) that $\| \bm{h} (\bm{w}^*) \| = 0$. As $\bm{g} (\bm{w}_i) = \bm{0}$ for all $i \geq 0$, we conclude that (\ref{NewtonYSchemeThm.0}) holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We now provide two remarks on the proof of Theorem~\ref{NewtonYSchemeThm}. First, note that we can use the abstract convergence theorem (by Hager [\textcolor{red}{SOURCE}]) to prove the inequality in (\ref{NewtonYThm.4}). For convenience, this result is stated in the appendix as Theorem~\ref{AbstractConvThm}. Here, we take the following values for parameters and functions in the Theorem~\ref{AbstractConvThm}:
\begin{align*}
&\bm{\theta} = [ \bm{u}_p (\bm{x}), \bm{y}_p (\bm{x})], \\
&\bm{\theta}^* = [ \bm{u}_p (\bm{x}^*), \bm{y}_p (\bm{x}^*)] = [\bm{0}, \bm{0}], \\
&\bm{\delta} = \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}) - \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}^*), \\
&\mathcal{T} (\bm{\theta}) = \bm{F}_p (\bm{\theta}, \bm{x}^*), \\
&\mathcal{L} = \nabla_{\theta} \mathcal{T} (\bm{\theta}^*) = \nabla_{[u,y]} \bm{F}_p ([\bm{u}_p (\bm{x}^*), \bm{y}_p (\bm{x}^*)], \bm{x}^*) = \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*), \\
&\mathcal{F} (\bm{\theta}) = \bm{0}. \\
\end{align*}
With these choices, we have that
\begin{align*}
\mathcal{T} (\bm{\theta}^*) + \bm{\delta} = \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) + \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) - \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) = \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) = \begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix}
\end{align*}
Hence, condition (C1) in Theorem~\ref{AbstractConvThm}, given by $\mathcal{T} (\bm{\theta}^*) + \bm{\delta} \in \mathcal{F} (\bm{\theta}^*)$, is equivalent to 
\begin{align*}
\begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix} = \bm{0}.
\end{align*}
This statement enforces the requirement that $\bm{x}$ is a feasible point for problem (\ref{NewtonYScheme}). Next, observe that 
\begin{align*}
\nabla \mathcal{T}(\bm{\theta}) - \mathcal{L} &= \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) - \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) \\
&= \left[
\begin{array}{c|c}
\multirow{2}{*}{$M(\bm{x})^{\intercal} M(\bm{x})$} & \frac{1}{\sqrt{p}} I_m \\
 & \bm{0} \\
\hline
\bm{0} & I_m
\end{array}
\right] - \left[
\begin{array}{c|c}
\multirow{2}{*}{$M(\bm{x}^*)^{\intercal} M(\bm{x}^*)$} & \frac{1}{\sqrt{p}} I_m \\
 & \bm{0} \\
\hline
\bm{0} & I_m
\end{array}
\right] \\
&= \left[
\begin{array}{c|c}
M(\bm{x})^{\intercal} M(\bm{x}) - M(\bm{x}^*)^{\intercal} M(\bm{x}^*) & \bm{0} \\
\hline
\bm{0} & \bm{0}
\end{array}
\right].
\end{align*}
Hence, condition (C2) in Theorem~\ref{AbstractConvThm}, given by $\| \nabla \mathcal{T}(\bm{\theta}) - \mathcal{L} \| \leq \varepsilon$ for all $\bm{\theta} \in B(\bm{\theta}^*,r)$, is equivalent to
\begin{align*}
\| M(\bm{x})^{\intercal} M(\bm{x}) - M(\bm{x}^*)^{\intercal} M(\bm{x}^*) \| \leq \varepsilon,
\end{align*}
for all $\bm{x} \in B(\bm{x}^*,r)$. As $\bm{h}, \bm{g} \in \mathcal{C}^2$, we have that $M(\bm{x})^{\intercal} M(\bm{x})$ is a continuous function. Hence, there exists a $r > 0$ such that (C2) is satisfied. Finally, observe that
\begin{align*}
(\mathcal{F} - \mathcal{L})^{-1} = (\bm{0} - \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*))^{-1} = - (\nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*))^{-1}.
\end{align*}
Based on our analysis in the proof of Theorem~\ref{NewtonYSchemeThm}, we have that $(\mathcal{F} - \mathcal{L})^{-1}$ is Lipschitz continuous with a uniformly bounded Lipschitz constant for sufficiently large values of $p$. Hence, condition (C3) from Theorem~\ref{AbstractConvThm} holds. Lastly, it requires to choose $\varepsilon > 0$ small enough and $p$ sufficiently large such that $\gamma \varepsilon < 1$. Once this choice has been made all hypotheses are satisfied for Theorem~\ref{AbstractConvThm} and we obtain the result that
\begin{align*}
\| \bm{\theta} - \bm{\theta}^* \| \leq \frac{\gamma}{1 - \gamma \varepsilon} \| \bm{\delta} \|,
\end{align*}
which in our case is equivalent to
\begin{align*}
\| \bm{u}_p (\bm{x}) \| \leq \frac{\gamma}{1 - \gamma \varepsilon} \| \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}) - \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}^*) \| = \frac{\gamma}{1 - \gamma \varepsilon} \left\| \begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix} \right\|,
\end{align*}
for all $\bm{x} \in B(\bm{x}^*,r)$. This is the desired result that is used in the proof of Theorem~\ref{NewtonYSchemeThm}.

As an additional remark, note that the constant appearing in (\ref{NewtonYThm.7}) can be made slightly different provided that $\bm{y}_{i, \infty} = \bm{0}$ for all $i \geq 1$. This follows from first observing that
\begin{align}
\bm{y}_{i+1} - \bm{y}_{i+1, \infty} &= - \bm{h}(\bm{w}_i) - \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1} - \bm{w}_i) + \bm{h}(\bm{w}_i) + \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1, \infty} - \bm{w}_i) \nonumber \\
&= \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1, \infty} - \bm{w}_{i+1} ). \nonumber 
\end{align}
As $\| \bm{w}_{i+1, \infty} - \bm{w}_{i+1} \| = O (1/p_i)$ from Theorem~\ref{thm:feasibility-detection}, we have that $\| \bm{y}_{i+1} - \bm{y}_{i+1, \infty} \| = O (1/p_i)$. By our hypothesis that $\bm{y}_{i+1, \infty} = 0$ it follows that $\| \bm{y}_{i+1} \| = O (1/p_i)$ which, by our choice of $p_i$, yields 
\begin{align}
\| \bm{y}_{i+1} \| = O \left( \left\| \bm{h}( \bm{w}_i) \right\|^2 \right). \label{NewtonYRemark.1}
\end{align}
Combining (\ref{NewtonYThm.6}) and (\ref{NewtonYRemark.1}) yields a slightly different constant.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ----------------------- MULTIPLIER STEP ANALYSIS ---------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Analysis for Multiplier Step} \label{subsec:multiplier-step-analysis} 
We now work towards establishing local convergence for the multiplier step in the CMS algorithm. Before stating and proving the local convergence result for the multiplier step, we require seceral results that willbe used in the proof. First, we restate Theorem 3.1 from \cite{Hager1993} in terms of our current analysis. Note that there are no changes to the details of the result and the same proof from \cite{Hager1993} holds. As such, the proof is omitted here.

\begin{theorem} \label{Theorem3.1}
Suppose $\bm{x}^*$ satisfies $\bm{h}(\bm{x}^*) = \bm{0}$ and $\bm{g}(\bm{x}^*) = \bm{0}$, $\bm{g}, \bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and %$\nabla h_j (\bm{z}^*)$ and $\nabla g_j (\bm{z}^*)$ are linearly independent. 
assumptions (\textbf{LI}) and (\textbf{SOSC}) hold.
Then there exists a neighborhood $\mathcal{N}$ about $(\bm{x}^*, \bm{\lambda}^*)$ for which the problem 
\begin{align}
\min \left\{ \mathcal{L}_{p_i}(\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{u}_i) (\bm{z} - \bm{u}_i) = \bm{0}, \bm{z} \in \Omega \right\}
\end{align}
has a local minimizer $\bm{z} = \bm{z}_{i+1}$, whenever $(\bm{u}_i, \bm{\nu}_i) \in \mathcal{N}$. Moreover, there exists a constant $c \in \mathbb{R}$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{\nu}_i - \bm{\lambda}^* \|^2 + c \| \bm{u}_i - \bm{x}^* \|^2 + c \| \bm{h}(\bm{u}_i) \|,
\end{align} 
for every $(\bm{u}_i, \bm{\nu}_i) \in \mathcal{N}$ with $\bm{u}_i \in \Omega$.
\end{theorem}

Next, we restate Corollary 3.1 from \cite{Hager1993} in terms of our current analysis (note that there are no changes to the details of the result and the same proof from \cite{Hager1993} holds).

\begin{corollary} \label{Corollary3.1}
Suppose $\bm{x}^*$ satisfies $\bm{h} (\bm{x}^*) = \bm{0}$ and $\bm{g} (\bm{x}^*) = \bm{0}$, $\bm{g}, \bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and 
%the rows of the matrix $[\nabla h (\bm{z}^*)^{\intercal} \ A^{\intercal}]^{\intercal}$ are linearly independent. 
assumptions (\textbf{LI}) and (\textbf{SOSC}) hold.
Then there exists a neighborhood $\mathcal{N}$ about $(\bm{x}^*, \bm{\lambda}^*)$ for which the problem 
\begin{align}
\min \left\{ \mathcal{L}_{p_i}(\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{u}_i) (\bm{z} - \bm{u}_i) = \bm{0}, \bm{z} \in \Omega \right\}
\end{align}
has a local minimizer $\bm{z} = \bm{z}_{i+1}$, whenever $(\bm{x}_k, \bm{\nu}_i) \in \mathcal{N}$, $\bm{x}_k \in \Omega$, and any $\bm{u}_i = \bm{w}_j$ for any $j \geq 1$, where $\bm{w}_j$ are generated by the scheme in (\ref{NewtonYScheme}) starting from $\bm{w}_0 = \bm{x}_k$. Moreover, there exists a constant $c \in \mathbb{R}$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{\nu}_i - \bm{\lambda}^* \|^2 + c \| \bm{x}_k - \bm{x}^* \|^2,
\end{align} 
where $c$ is independent of $(\bm{x}_k, \bm{\nu}_i) \in \mathcal{N} \cap \left( \Omega \times \mathbb{R}^m \right)$.
\end{corollary}
\iffalse
\begin{proof}
As $\bm{h} (\bm{x}^*) = \bm{0}$ we have that
\begin{align}
\| \bm{h}(\bm{x}_k)  \| = \| \bm{h}(\bm{x}_k) - \bm{h}(\bm{x}^*) \| = \| \nabla \bm{h}(\bm{\xi}) (\bm{x}_k - \bm{x}^*) \| \leq c \| \bm{x}_k - \bm{x}^* \|, \label{Corollary.1}
\end{align}
where $\bm{\xi}$ is some vector between $\bm{x}_k$ and $\bm{x}^*$. Using (\ref{NewtonYSchemeThm.1}) from Theorem~\ref{NewtonYSchemeThm} with $\bm{w}_0 = \bm{x}_k$, we have that $\| \bm{w}_j - \bm{x}_k \| \leq c \| \bm{h}(\bm{x}_k) \|$, for all $j \geq 1$. As $\bm{u}_i = \bm{w}_j$ for some $1 \leq j \leq i_C$, it follows that $\| \bm{u}_i - \bm{x}_k \| \leq c \| \bm{h}(\bm{x}_k) \|$. Combining this with (\ref{Corollary.1}) and the triangle inequality yields
\begin{align*}
\| \bm{u}_i - \bm{x}^* \| 
&\leq \| \bm{u}_i - \bm{x}_k \| + \| \bm{x}_k - \bm{x}^* \| 
\leq c \| \bm{x}_k - \bm{x}^* \|.
\end{align*}
Lastly, (\ref{NewtonYSchemeThm.3}) from Theorem~\ref{NewtonYSchemeThm} with $\bm{w}_0 = \bm{x}_k$ yields that $\| \bm{h}(\bm{u}_i) \| \leq c \| \bm{h}(\bm{x}_k) \|^2$ which combined with (\ref{Corollary.1}) yields that $\| \bm{h}(\bm{u}_i) \| \leq c \| \bm{x}_k - \bm{x}^* \|^2$. Making these substitutions into Theorem~\ref{Theorem3.1} concludes the proof.
\end{proof}
\fi

In order to prove the local convergence result for the multiplier step, we make use of the following problem:
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x} \in \mathbb{R}^{n}} & f(\bm{x}) \\
\text{s.t.} & \bm{h}(\bm{x}) = \bm{u}, \ \ \bm{r} (\bm{x}) \leq \bm{0},
\end{array} \label{prob:Ru}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x}} & f(\bm{x}) \\
\text{s.t.} & \bm{h} (\bm{x}) = \bm{u}, \ \ \bm{g} (\bm{x}) = \bm{0},
\end{array} \label{prob:Gu}
\end{align}
and
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\bm{u}$ is a fixed vector in $\mathbb{R}^m$. Note that (\ref{prob:Ru}) is very similar to problem (\ref{prob:main-nlp}) with the only difference being the perturbation applied to the nonlinear portion of the constraint set, namely changing $\bm{h} (\bm{x}) = \bm{0}$ to $\bm{h} (\bm{x}) = \bm{u}$. Lemma~\ref{lem:Lem13.1} will provide insight into how close a solution of problem (\ref{prob:Ru}) is to a solution of (\ref{prob:main-nlp}) for different values of $\bm{u}$ by performing stability analysis of problem (\ref{prob:Ru}) for values of $\bm{u}$ in a neighborhood of $\bm{u} = \bm{0}$. We note that Lemma~\ref{lem:Lem13.1} has the same conclusions as Lemma 13.1 from \cite{Hager1993}, however, the difference here being that the hypotheses are more general. This is accomplished by making use of strong regularity as discussed by Robinson in \cite{Robinson1980}. This difference will allow us to clearly justify alternate sets of assumptions when establishing convergence results for the multiplier step of NPASA. 

\begin{lemma} \label{lem:Lem13.1}
Suppose that $f, \bm{h}$ from problem (\ref{prob:main-nlp}) are twice continuously differentiable and that %the KKT system for problem (\ref{prob:Ru}) is strongly regular at a KKT point $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. 
either assumptions (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LI}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Then there exists a neighborhood $\mathcal{N}$ of $\bm{0}$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Ru}) has a local minimizer $\bm{x}(\bm{u})$ and associated multipliers $\bm{\lambda} (\bm{u})$ and $\bm{\mu} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.1}.1)] $\begin{pmatrix} \bm{x}(\bm{0}), \ \bm{\lambda} (\bm{0}), \ \bm{\mu} (\bm{0}) \end{pmatrix} = \left( \bm{x}^*, \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:Lem13.1}.2)] $\begin{pmatrix} \bm{x}(\bm{u}), \ \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Ru}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{x}(\bm{0}), \ \bm{\lambda} (\bm{0}), \ \bm{\mu} (\bm{0}) \end{pmatrix} = \left( \bm{x}^*, \bm{\lambda}^*, \bm{\mu}^* \right),\label{lem:Lem13.1.1} \\
&\begin{pmatrix} \bm{x}(\bm{u}), \ \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}) \end{pmatrix} \ \text{satisfies the KKT system for problem (\ref{prob:Ru})}. \label{lem:Lem13.1.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.1}.3)] $\displaystyle \left\| \left(
\bm{x} (\bm{u}_1), \bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1) 
\right) - \left(
\bm{x} (\bm{u}_2), \bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{x} (\bm{u}_1), \bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1) 
\right) - \left(
\bm{x} (\bm{u}_2), \bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|. \label{lem:Lem13.1.3}
\end{align}
\end{lemma}
\begin{proof}
We first establish that the KKT system for problem (\ref{prob:main-nlp}) is strongly regular at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. In Section 4 of \cite{Robinson1980}, Robinson outlines conditions under which the KKT system for a nonlinear program is strongly regular. One set of assumptions that guarantees a strongly regular KKT system for problem (\ref{prob:main-nlp}) at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is that (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}) hold at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Additionally, Theorem 4.1 of \cite{Robinson1980} proves that if assumptions (\textbf{LI}) and (\textbf{SSOSC}) hold at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ then this guarantees strong regularity for the KKT system in (\ref{prob:main-nlp}). Under either set of hypotheses for our lemma, we have that the KKT system for problem (\ref{prob:main-nlp}) is strongly regular at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. We now prove the lemma using some results from \cite{Robinson1980}.

Now denote the Lagrangian of problem (\ref{prob:Ru}) by
\begin{align}
\mathcal{L} (\bm{u}; \bm{x}, \bm{\lambda}, \bm{\mu}) = f (\bm{x}) + \bm{\lambda}^{\intercal} \left( \bm{h} (\bm{x}) - \bm{u} \right) + \bm{\mu}^{\intercal} \bm{r} (\bm{x}). \label{eq:KKTStability.0}
\end{align}
Using $\bm{f}(\cdot)$ in this proof in the context of \cite{Robinson1980}, we define 
\begin{align}
\bm{f} (\bm{u}, \bm{x}, \bm{\lambda}, \bm{\mu}) 
:= \begin{bmatrix}
\nabla_x \mathcal{L} (\bm{x}, \bm{\lambda}, \bm{\mu}) \\
- \bm{r} (\bm{x}) \\
- \bm{h} (\bm{x}) + \bm{u}
\end{bmatrix}. \label{eq:KKTStability.1}
\end{align}
By the hypotheses of our lemma, we have that the hypotheses of Theorem 2.1 of \cite{Robinson1980} are satisfied. To apply Corollary 2.2 from \cite{Robinson1980}, it remains to show that there exists a constant $\nu$ such that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{x}, \bm{\lambda}, \bm{\mu}) - \bm{f} (\bm{u}_2, \bm{x}, \bm{\lambda}, \bm{\mu}) \| \leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:KKTStability.2}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{x}, \bm{\lambda}, \bm{\mu}) \in V$, where $V$ is a closed neighborhood of $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Noting that
\begin{align}
\nabla_x \mathcal{L} (\bm{u}; \bm{x}, \bm{\lambda}, \bm{\mu})^{\intercal} = \nabla_x f (\bm{x})^{\intercal} + \nabla_x \bm{h} (\bm{x})^{\intercal} \bm{\lambda} + \nabla_x \bm{r} (\bm{x})^{\intercal} \bm{\mu} \label{eq:KKTStability.3}
\end{align}
it follows that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{x}, \bm{\lambda}, \bm{\mu}) - \bm{f} (\bm{u}_2, \bm{x}, \bm{\lambda}, \bm{\mu}) \| 
= \left\| \begin{bmatrix}
\bm{0} \\
\bm{0} \\
\bm{u}_1 - \bm{u}_2 
\end{bmatrix} \right\|
= \left\| \bm{u}_1 - \bm{u}_2 \right\|, \label{eq:KKTStability.4}
\end{align}
which concludes the proof.
\end{proof}

%In Section 4 of \cite{Robinson1980}, Robinson outlines sufficient conditions under which the KKT system for a nonlinear program is strongly regular. One set of assumptions that guarantees a strongly regular KKT system is (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}). Additionally, Theorem 4.1 of \cite{Robinson1980} proves that assumptions (\textbf{LI}) and (\textbf{SSOSC}) guarantee strong regularity for the KKT system in a nonlinear program.

Next, we consider the problem where we %choose $j \in \{0,1\}$ and 
fix a vector $\bm{u}$ then solve
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{\lambda}, \bm{\mu}} & E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) \\
\text{s.t.} & \bm{\mu} \geq \bm{0}.
\end{array} \label{prob:Mu}
\end{align}
For this problem, we have a stability result that follows from an application of Corollary 2.2 in \cite{Robinson1980}.
\begin{lemma} \label{lem:Lem13.2}
%Let $j \in \{0,1\}$. 
Suppose that $f, \bm{h}$ from problem (\ref{prob:main-nlp}) are continuously differentiable, $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}), and that (\textbf{LI}) holds at $\bm{x}^*$. %, and that $E_{m,j} (\bm{u}, \bm{\lambda}, \bm{\mu})$ is twice continuously differentiable with respect to $\bm{\lambda}$ and $\bm{\mu}$ in a neighborhood of $(\bm{\lambda}^*, \bm{\mu}^*)$. 
Then there exists a neighborhood $\mathcal{N}$ of $\bm{x}^*$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Mu}) has a local minimizer $(\bm{\lambda} (\bm{u}), \bm{\mu} (\bm{u}))$ and associated multiplier $\bm{\alpha} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.2}.1)] $\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:Lem13.2}.2)] $\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Mu}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right), \label{lem:Lem13.2.1} \\
&\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}  \ \text{satisfies the KKT system for problem (\ref{prob:Mu})}. \label{lem:Lem13.2.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.2}.3)] $\displaystyle \left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|. \label{lem:Lem13.2.3}
\end{align}
\end{lemma}
\begin{proof}
Denote the Lagrangian for problem (\ref{prob:Mu}) by
\begin{align}
\mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) = E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) - \bm{\mu}^{\intercal} \bm{\alpha}. \label{eq:EMStability.0.0}
\end{align}
As in the proof of Lemma~\ref{lem:Lem13.1}, we first establish that the KKT system for problem (\ref{prob:Mu}) is strongly regular at $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$ under the given hypotheses. Using (\ref{eq:EMStability.0.0}) we have that the hessian of the Lagrangian for problem (\ref{prob:Mu}) is given by $\nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) = B (\bm{u})^{\intercal} B (\bm{u})$, where $B (\bm{u})$ is the matrix defined by
\begin{align}
B (\bm{u})
&:= \begin{bmatrix}
\ \nabla_x \bm{h} (\bm{u})^{\intercal} &\vert& \nabla_x \bm{r} (\bm{u})^{\intercal} \
\end{bmatrix}. \label{eq:EmDiscussion.1}
\end{align}
Hence, for every vector $\bm{v} = [\bm{\lambda}, \bm{\mu}]^{\intercal}$ with $\bm{v} \neq \bm{0}$ we have
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{u}) \bm{v} \right\|^2
\geq 0. \label{eq:EmDiscussion.2}
\end{align}
So we have that the hessian of the Lagrangian for problem (\ref{prob:Mu}) is positive semidefinite. Under our hypothesis that (\textbf{LI}) holds at $\bm{x}^*$, we have that $B (\bm{x}^*)$ is of full column rank yielding that $B (\bm{x}^*)^{\intercal} B (\bm{x}^*)$ is nonsingular. As such, there exists a constant $\sigma > 0$ such that
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{x}^*; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{x}^*) \bm{v} \right\|^2
> \sigma. \label{eq:EmDiscussion.3}
\end{align}
So we have positive definiteness of the hessian under assumption (\textbf{LI}). As (\ref{prob:Mu}) only has bound constraints, the gradients of the active constraints are linearly independent. Thus, under the assumption that (\textbf{LI}) holds at $\bm{x}^*$ the KKT system in problem (\ref{prob:Mu}) satisfies the strong regularity condition from \cite{Robinson1980}.

Now define $\bm{f} (\bm{u}, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) := \begin{bmatrix}
\nabla_{[\lambda, \mu]} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \\
\bm{\mu}
\end{bmatrix}$, where $\bm{f}(\cdot)$ is used in this proof in the context of \cite{Robinson1980}. By our hypotheses, we have that the hypotheses of Theorem 2.1 of \cite{Robinson1980} are satisfied. To apply Corollary 2.2 from \cite{Robinson1980}, it remains to show that there exists a constant $\nu$ such that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) - \bm{f} (\bm{u}_2, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \| \leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.0}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$, where $V$ is a closed neighborhood of $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$. To this end, observe that
\begin{align}
\nabla_{\lambda} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal}
&= \nabla \bm{h} (\bm{u}) \nabla f (\bm{u})^{\intercal} + \nabla \bm{h} (\bm{u}) \nabla \bm{h} (\bm{u})^{\intercal} \bm{\lambda} + \nabla \bm{h} (\bm{u}) \nabla \bm{r} (\bm{u})^{\intercal} \bm{\mu}. \label{eq:EMStability.1}
\end{align}
Hence,
\begin{align}
\| \nabla_{\lambda} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\lambda} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \| \nabla \bm{h} (\bm{u}_1) \nabla f (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla f (\bm{u}_2)^{\intercal} \| \nonumber \\
&\quad + \| \nabla \bm{h} (\bm{u}_1) \nabla \bm{h} (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla \bm{h} (\bm{u}_2)^{\intercal} \| \| \bm{\lambda} \| \nonumber \\
&\quad + \| \nabla \bm{h} (\bm{u}_1) \nabla \bm{r} (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla \bm{r} (\bm{u}_2)^{\intercal} \| \| \bm{\mu} \|. \label{eq:EMStability.2}
\end{align}
As $(\bm{\lambda}, \bm{\mu}, \bm{\alpha})$ is in a closed neighborhood $V$ of $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$, there exist constants $c_1$ and $c_2$ such that $\| \bm{\lambda} \| \leq c_1$ and $\| \bm{\mu} \| \leq c_2$ for all $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. As $f, \bm{h}, \bm{r} \in \mathcal{C}^1$, the functions $\nabla \bm{h} (\cdot) \nabla f (\cdot)^{\intercal}$, $\nabla \bm{h} (\cdot) \nabla \bm{h} (\cdot)^{\intercal}$, and $\nabla \bm{h} (\cdot) \nabla \bm{r} (\cdot)^{\intercal}$ are Lipschitz continuous on $\mathcal{N}$. Combining these facts with (\ref{eq:EMStability.2}) yields that there exists a constant $\nu$ such that
\begin{align}
\| \nabla_{\lambda} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\lambda} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.3}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. Next, observe that
\begin{align}
\nabla_{\mu} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal}
&= \nabla \bm{r} (\bm{u}) \nabla f (\bm{u})^{\intercal} + \nabla \bm{r} (\bm{u}) \nabla \bm{h} (\bm{u})^{\intercal} \bm{\lambda} + \nabla \bm{r} (\bm{u}) \nabla \bm{r} (\bm{u})^{\intercal} \bm{\mu} - \bm{r} (\bm{u}) - \bm{\alpha}. \label{eq:EMStability.4}
\end{align}
Hence,
\begin{align}
\| \nabla_{\mu} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\mu} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \| \nabla \bm{r} (\bm{u}_1) \nabla f (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla f (\bm{u}_2)^{\intercal} \| \nonumber \\
&\quad + \| \nabla \bm{r} (\bm{u}_1) \nabla \bm{h} (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla \bm{h} (\bm{u}_2)^{\intercal} \| \| \bm{\lambda} \| \nonumber \\
&\quad + \| \nabla \bm{r} (\bm{u}_1) \nabla \bm{r} (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla \bm{r} (\bm{u}_2)^{\intercal} \| \| \bm{\mu} \| \nonumber \\
&\quad + \| \bm{r} (\bm{u}_1) - \bm{r} (\bm{u}_2) \|. \label{eq:EMStability.5}
\end{align}
By an argument similar to the one establishing (\ref{eq:EMStability.3}), there exists a constant $\nu$ such that
\begin{align}
\| \nabla_{\mu} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\mu} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.6}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. Now combining (\ref{eq:EMStability.3}) and (\ref{eq:EMStability.6}) yields (\ref{eq:EMStability.0}). Corollary 2.2 from \cite{Robinson1980} can now be applied to conclude the proof.
\end{proof}

We now make a comment on what can be said on the stability of problem (\ref{prob:Mu}) if $E_{m,0}$ is replaced with $E_{m,1}$. To this end, we note that $E_{m,1} (\bm{u}, \bm{\lambda}, \bm{\mu})$ must be twice continuously differentiable with respect to $\bm{\lambda}$ and $\bm{\mu}$ in a neighborhood of a solution $(\bm{\lambda}^*, \bm{\mu}^*)$ to establish a satibility result similar to Lemma~\ref{lem:Lem13.2}. We can guarantee this holds provided that the hypotheses of Lemma~\ref{lem:E1diff} are satisfied, that is, in addition to the hypotheses of Lemma~\ref{lem:Lem13.2} we require that assumption (\textbf{SCS}) holds at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. This result is much more restrictive as it would limit future analysis to only nondegenerate stationary points of problem (\ref{prob:main-nlp}). As such, this provides some motivation behind the choice of minimizing $E_{m,0}$ with respect to $\bm{\lambda}$ and $\bm{\mu}$ instead of $E_{m,1}$ in the Multiplier Step of NPASA. We note that the additional minization of $E_{m,1}$ with respect to $\bm{\mu}$ in the Multiplier Step is required in order to ensure fast local convergence of the Multiplier Step in the CMS algorithm as will be illustrated in the proof of Theorem~\ref{ConvergenceResult}.

It should be noted that we can slightly modify problem (\ref{prob:Mu}) to ensure positive definiteness even in the case where (\textbf{LI}) fails to hold. This can be done by fixing a constant $\gamma > 0$ and slightly augmenting the objective function to obtain
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{\lambda}, \bm{\mu}} & E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) + \gamma \left\| [\bm{\lambda}, \bm{\mu}] \right\|^2 \\
\text{s.t.} & \bm{\mu} \geq \bm{0}.
\end{array} \label{prob:Mu-gamma}
\end{align}
Under this modification, for every vector $\bm{v} = [\bm{\lambda}, \bm{\mu}]^{\intercal}$ with $\bm{v} \neq \bm{0}$ we have
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{u}) \bm{v} \right\|^2 + \gamma \| \bm{v} \|^2
> 0. \label{eq:PostEmDiscussion.1}
\end{align} 
Hence, the hessian of the Lagrangian for (\ref{prob:Mu-gamma}) is positive definite. As (\ref{prob:Mu-gamma}) has the same constraints as (\ref{prob:Mu}), the gradients of the active constraints are linearly independent. Thus, the KKT system in problem (\ref{prob:Mu-gamma}) always satisfies the strong regularity condition from \cite{Robinson1980}. With this established, we now state the following result that follows from the same argument in Lemma~\ref{lem:Lem13.2} but is applied to problem (\ref{prob:Mu-gamma}).

\begin{lemma} \label{lem:AltLem13.2}
Suppose that $f, \bm{h} \in \mathcal{C}^1$ and that $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}). Then there exists a neighborhood $\mathcal{N}$ of $\bm{x}^*$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Mu-gamma}) has a local minimizer $(\bm{\lambda} (\bm{u}), \bm{\mu} (\bm{u}))$ and associated multiplier $\bm{\alpha} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:AltLem13.2}.1)] $\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:AltLem13.2}.2)] $\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Mu-gamma}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right), \label{lem:AltLem13.2.1} \\
&\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix} \ \text{satisfies the KKT system for problem (\ref{prob:Mu-gamma})}. \label{lem:AltLem13.2.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:AltLem13.2}.3)] $\displaystyle \left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \| \label{lem:AltLem13.2.3}
\end{align}
\end{lemma}

%%%%%%%% (Following result is not true since it is missing constraint)
\iffalse
We now provide one final result that will be useful in establishing local convergence of the multiplier step of NPASA.

\begin{lemma} \label{lem:DualStep}
Suppose $f, \bm{h}, \bm{r} \in \mathcal{C}^1$ and let $\{ \bm{z}_i \}_{i = 1}^{\infty}$ be the sequence of primal variables generated by the miltiplier step of NPASA in Algorithm~\ref{alg:npasa}. Then
\begin{align}
\min_{\bm{\mu} \geq \bm{0}, \bm{\lambda}} E_m (\bm{z}_{i+1}, \bm{\lambda}, \bm{\mu}) 
= 0
%\leq \| \bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i) \|^2
, \label{result:DualStep}
\end{align}
for all $i \geq 1$.
\end{lemma}
\begin{proof}
By the KKT conditions for the primal step, there exists a vector $\bm{\alpha}_{i+1} \geq \bm{0}$ such that
\begin{align*}
\nabla f (\bm{z}_{i+1}) + \left( \bm{\lambda}_i + 2 q_i (\bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i)) \right)^{\intercal} \nabla \bm{h} (\bm{z}_{i+1}) + \bm{\alpha}_{i+1}^{\intercal} A = \bm{0}
\end{align*}
and $\bm{\alpha}_{i+1}^{\intercal} \bm{r} (\bm{z}_{i+1}) = 0$. Hence,
\begin{align}
\min_{\bm{\mu} \geq \bm{0}, \bm{\lambda}} E_m (\bm{z}_{i+1}, \bm{\lambda}, \bm{\mu})
&\leq E_m (\bm{z}_{i+1}, \bm{\lambda}_i + 2 q_i (\bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i)), \bm{\alpha}_{i+1}) = 0, \label{eq:DualStep.1}
\end{align}
which concludes the proof.
%As $\| \bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i) \|^2 \geq 0$, the result (\ref{result:DualStep}) now follows from (\ref{eq:DualStep.1}).
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With these lemmas in place, we are now ready to state and prove a convergence result for the multiplier step of NPASA, found in Algorithm~\ref{alg:cms}. This result is a modified version of Theorem 4.1 in \cite{Hager1993} accounting for the updates made to the algorithm. While there are many required updates to the proof, we note that some details of the proof are essentially the same as in the proof of Theorem 4.1 in \cite{Hager1993} but are included here for completeness. %Additionally, note that the iterative scheme in (\ref{scheme:MS1}) -- (\ref{scheme:MS3}) is the same update provided in the CMS pseudocode, Algorithm~\ref{alg:cms}, so the following result applies to the Algorithm~\ref{alg:cms}.

\begin{theorem} \label{ConvergenceResult}
Suppose that $f, \bm{h} \in \mathcal{C}^2$ and that either assumptions (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LI}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. %If $p_k$ is chosen such that $p_k \geq 1$ and $\frac{1}{p_k} \leq \| h (\bm{x}_k) \|^2$ for all $k \geq 0$ then 
Then there exists a neighborhood $\mathcal{N}_1$ and $\mathcal{N}_2$ of $\bm{x}^*$ and a constant $c$ such that, for every $\bm{z}_0 \in \mathcal{N}_1 \cap \Omega$, the primal variables and equality multipliers, $(\bm{z}, \bm{\nu})$, generated using the scheme
\begin{align}
(\bm{\nu}_i, \bm{\eta}_i) &\in \arg\min \left\{ E_{m,0} ( \bm{z}_i, \bm{\nu}, \bm{\eta}) : \bm{\eta} \geq \bm{0} \right\} \label{scheme:MS1} \\
\bm{\eta}_i' &\in \arg\min \left\{ E_{m,1} ( \bm{z}_i, \bm{\nu}_i, \bm{\eta}) : \bm{\eta} \geq \bm{0} \right\} \label{scheme:MS2} \\
\bm{z}_{i+1} &= \arg \min \left\{ \mathcal{L}_{p_i}^i (\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{z}_i) (\bm{z} - \bm{z}_i) = 0, \bm{z} \in \mathcal{N}_2 \cap \Omega \right\} \label{scheme:MS3}
\end{align}
%in the multiplier step of NPASA 
converge to a point $( \bm{z}^*, \bm{\nu}^* )$ and
\iffalse
\begin{itemize}
\item[(\ref{ConvergenceResult}.0)] $\displaystyle \min_{\bm{\eta} \geq \bm{0}} E_{m,1} ( \bm{z}^*, \bm{\nu}^*, \bm{\eta} ) = 0$.
\end{itemize}
\fi
\begin{align}
\min_{\bm{\eta} \geq \bm{0}} E_{m,1} ( \bm{z}^*, \bm{\nu}^*, \bm{\eta} ) = 0. \label{ConvergenceResult.0}
\end{align}
Furthermore, the following properties hold for $i \geq 0$:
\iffalse
\begin{itemize}
\item[(\ref{ConvergenceResult}.1)] $\| \bm{z}_i - \bm{z}^* \| \leq c 2^{-2^i}$.
\item[(\ref{ConvergenceResult}.2)] $\| \bm{z}_{i+1} - \bm{z}_1 \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2$.
\item[(\ref{ConvergenceResult}.3)] $\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| h (\bm{z}_0) \|$.
\item[(\ref{ConvergenceResult}.4)] $E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2$.
\item[(\ref{ConvergenceResult}.5)] $E_1 \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \leq \| \bm{z}_i - \bm{x}^* \|$.
%\item[(\ref{ConvergenceResult}.6)] $\displaystyle \lim_{i \to \infty} E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) = 0$.
\end{itemize}
\fi
\begin{align}
&\| \bm{z}_i - \bm{z}^* \| \leq c 2^{-2^i}, \label{ConvergenceResult.1} \\
&\| \bm{z}_{i+1} - \bm{z}_1 \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2, \label{ConvergenceResult.2} \\
&\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| h (\bm{z}_0) \|, \label{ConvergenceResult.3} \\
&E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2, \label{ConvergenceResult.4} \\
&E_1 \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \leq \| \bm{z}_i - \bm{x}^* \|. \label{ConvergenceResult.5}
%\lim_{i \to \infty} E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) &= 0. \label{ConvergenceResult.6}
\end{align}
\end{theorem}

Before providing the proof for this theorem, we note that the iterative scheme in (\ref{scheme:MS1}) -- (\ref{scheme:MS3}) is the same update provided in the CMS pseudocode, Algorithm~\ref{alg:cms}, without checking for a sufficient decrease in the error estimator at each iteration. %that would result in reusing the same multipliers at the next iteration. 
As a result, it follows from (\ref{ConvergenceResult.4}) that the criterion $E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq \delta E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)$ in the Multiplier Step of the CMS algorithm will always be satisfied under the hypotheses of Theorem~\ref{ConvergenceResult} for $i$ sufficiently large. Hence, this local convergence result can be applied to the Multiplier step of the CMS algorithm without modification. We now provide a proof for Theorem~\ref{ConvergenceResult}.
\fi

\begin{proof}[Proof of Theorem~\ref{ConvergenceResult}]
We will perform our analysis of this method by considering the perturbed problem (\ref{prob:Ru}). As problem (\ref{prob:main-nlp}) is equivalent to problem (\ref{prob:Ru}) with $\bm{u} = \bm{0}$, we have that $\bm{x}^*$ is a solution of problem (\ref{prob:Ru}) with $\bm{u} = \bm{0}$. Additionally, we will let $\bm{z}_i^*$ denote the local minimizer of (\ref{prob:Ru}) with $\bm{u} = \bm{h}(\bm{z}_i)$ and $( \bm{\nu}_i^*, \bm{\eta}_i^* )$ be corresponding multipliers for which $E_{m,1} \left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right) = 0$. To justify the existence of $( \bm{\nu}_i^*, \bm{\eta}_i^* )$, observe that the Lagrangian for problem (\ref{prob:Ru}) with $\bm{u} = \bm{h}(\bm{z}_i)$ is 
\begin{align}
f(\bm{x}) + \bm{\lambda}^{\intercal} \left( \bm{h}(\bm{x}) - \bm{h}(\bm{z}_i) \right) + \bm{\mu}^{\intercal} \bm{r} (\bm{x})
\end{align} 
which has gradient 
\begin{align}
\nabla f(\bm{x}) + \bm{\lambda}^{\intercal} \nabla \bm{h}(\bm{x}) + \bm{\mu}^{\intercal} \nabla \bm{r} (\bm{x}).
\end{align}
As this gradient is the same as the gradient of the Lagrangian for problem (\ref{prob:main-nlp}), we have that a KKT point $\left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right)$ for problem (\ref{prob:Ru}) satisfies $E_{m,1} \left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right) = 0$, as desired.

\iffalse % No longer necessary for analysis (keeping for now in case it comes up later)
Finally, we define 
\begin{align*}
\bm{y}_k^* = - \bm{h}(\bm{x}_k) - \nabla \bm{h}(\bm{x}_k) (\bm{x}_k^* - \bm{x}_k).
\end{align*}
\fi

Suppose that $\bm{z}_i$ is near $\bm{x}^*$. %By Lemma 13.1 in \cite{Hager1993} with $\bm{u} = \bm{h} (\bm{x}_k)$, we have that
By (\ref{lem:Lem13.1.1}) in Lemma~\ref{lem:Lem13.1}, we have $\bm{x} (\bm{h} (\bm{z}_i)) = \bm{z}_i^*$ and $\bm{x} (\bm{h} (\bm{x}^*)) = \bm{x}^*$. Hence, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_i)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*) = \bm{0}$, it follows that
\begin{align}
\| \bm{z}_i^* - \bm{x}^* \| \leq c \| \bm{h}( \bm{z}_i ) - \bm{h}(\bm{x}^*) \| = c \| \bm{h}( \bm{z}_i ) \|.
\end{align} 
Since $\| \bm{h}(\bm{z}_i) \| \to 0$ as $\bm{z}_i \to \bm{x}^*$, we have that $\bm{z}_i^*$ is near $\bm{x}^*$ when $\bm{z}_i$ is near $\bm{x}^*$. As $\bm{x} = \bm{z}_i$ satisfies the constraint $\bm{h} (\bm{x}) = \bm{u}$ when $\bm{u} = \bm{h} (\bm{z}_i)$, it follows from Theorem~\ref{Theorem3.1} that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| &\leq c \| \bm{\nu}_i - \bm{\nu}_i^* \|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2 + c \| \bm{h} (\bm{z}_i) - \bm{h} (\bm{z}_i) \| \\
&= c \| \bm{\nu}_i - \bm{\nu}_i^* \|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2 \\
&\leq c \left\| \begin{bmatrix} \bm{\nu}_i, \ \bm{\eta}_i \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2, \label{NPASA8.1}
\end{align}
for some constant $c$. As a note of interest to the reader, observe that the penalized Lagrangian function for problem (\ref{prob:Ru}) is given by
\begin{align}
\mathcal{L}_{p} (\bm{\nu}, \bm{z}) = f(\bm{z}) + \bm{\nu}^{\intercal} \bm{h} (\bm{z}) + p \| \bm{h} (\bm{z}) - \bm{u} \|^2.
\end{align}
Hence, when we take $\bm{u} = \bm{h} (\bm{z}_i)$ we have that the penalized Lagrangian function for problem (\ref{prob:Ru}) is equal to $\mathcal{L}_{p}^i (\bm{\nu}, \bm{z})$.
%
\iffalse % No longer needed since corollary covers this part
Next, observe that
\begin{align}
\| \bm{z}_k - \bm{x}_k^* \|^2 &= \| \bm{z}_k - \bm{x}_k + \bm{x}_k - \bm{x}_k^* \|^2 \nonumber \\
&\leq \| \bm{z}_k - \bm{x}_k \|^2 + 2 \left| \langle \bm{z}_k - \bm{x}_k, \bm{x}_k - \bm{x}_k^* \rangle \right| + \| \bm{x}_k - \bm{x}_k^* \|^2 \nonumber \\
&\leq 2 \| \bm{z}_k - \bm{x}_k \|^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2 \label{NPASA8.1.1} \\
&\leq 2 \left( c_1 \| h (\bm{x}_k) \| \right)^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2 \label{NPASA8.1.2} \\
&= 2 c_1^2 \| h (\bm{x}_k) \|^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2, \label{NPASA8.2}
\end{align}
where (\ref{NPASA8.1.1}) follows from Cauchy and (\ref{NPASA8.1.2}) follows from Theorem~\ref{NewtonYSchemeThm} with $\bm{z}_0 = \bm{x}_k$. Combining (\ref{NPASA8.1}) and (\ref{NPASA8.2}) yields
\begin{align}
\| \bm{x}_{k+1} - \bm{x}_k^* \| \leq c \| [\bm{\lambda}_k \ \bm{\mu}_k] - [\bm{\lambda}_k^* \ \bm{\mu}_k^*] \|^2 + c \| \bm{x}_k - \bm{x}_k^* \|^2 + c \| h (\bm{x}_k) \|^2. \label{NPASA8.2.1}
\end{align}
\fi
%
Next, by either assumptions (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}) or assumptions (\textbf{LI}) and (\textbf{SSOSC}) we have that the hypotheses of Lemma~\ref{lem:Lem13.2} are satisfied. Hence, it follows from (\ref{lem:Lem13.2.3}) in Lemma~\ref{lem:Lem13.2} with $\bm{u}_1 = \bm{z}_i$ and $\bm{u}_2 = \bm{z}_i^*$ that 
\begin{align}
\left\| \begin{bmatrix} \bm{\nu}_i, \ \bm{\eta}_i \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| = O \left( \| \bm{z}_i - \bm{z}_i^* \| \right). \label{NPASA8.3}
\end{align}
Similarly, $\left\| \begin{bmatrix} \bm{\nu}_{i+1}, \ \bm{\eta}_{i+1} \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| = O \left( \| \bm{z}_{i+1} - \bm{z}_i^* \| \right)$ follows from an additional application of (\ref{lem:Lem13.2.3}) in Lemma~\ref{lem:Lem13.2}. Now (\ref{NPASA8.1}) and (\ref{NPASA8.3}) together imply that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| + \left\| \begin{bmatrix} \bm{\nu}_{i+1}, \ \bm{\eta}_{i+1} \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2. \label{NPASA8.3.1}
\end{align}

By our choice of Problem (\ref{prob:Ru}), for $\bm{u} = \bm{h}(\bm{z}_i)$ we have that $\bm{h}(\bm{z}_i^*) = \bm{h}(\bm{z}_i)$. Hence,
\begin{align}
\| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \| &= \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i^*) \| \leq c \| \bm{z}_{i+1} - \bm{z}_i^* \| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2, \label{NPASA8.10}
\end{align}
where (\ref{NPASA8.10}) follows from performing a first order Taylor expansion of $\bm{h}$ and using (\ref{NPASA8.3.1}). Next, from (\ref{lem:Lem13.1.1}) in Lemma~\ref{lem:Lem13.1} we have that $\bm{x} (\bm{h} (\bm{z}_{i+1})) = \bm{z}_{i+1}^*$ and $\bm{x} (\bm{h} (\bm{z}_i)) = \bm{z}_i^*$. Hence, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_{i+1})$ and $\bm{u}_2 = \bm{h} (\bm{z}_i)$ together with (\ref{NPASA8.10}) yields
\begin{align}
\| \bm{z}_{i+1}^* - \bm{z}_i^* \| &\leq c \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2. \label{NPASA8.11}
\end{align}
Now define
\begin{align}
r_{i+1} := \| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{z}_{i+1}^* - \bm{z}_i^* \|. \label{NPASA8.12}
\end{align}
We claim that $r_{i+1} = O (r_i^2)$. To prove this claim, first note that combining (\ref{NPASA8.3.1}), (\ref{NPASA8.11}), and (\ref{NPASA8.12}) yields
\begin{align}
r_{i+1} \leq c \| \bm{z}_i - \bm{z}_i^* \|. \label{NPASA8.12.1}
\end{align}
By Cauchy, we have
\begin{align}
\| \bm{z}_i - \bm{z}_i^* \| \leq 2 \| \bm{z}_i - \bm{z}_{i-1}^* \|^2 + 2 \| \bm{z}_i^* - \bm{z}_{i-1}^* \|^2 \label{NPASA8.13}
\end{align}
which combined with (\ref{NPASA8.12.1}) yields $r_{i+1} = O (r_i^2)$, as claimed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% No longer needed since this term doesn't show up in bound but might be useful later
\iffalse 
Additionally, performing a second order Taylor expansion and applying $\nabla \bm{h} (\bm{z}_k) (\bm{x}_{k+1} - \bm{z}_k) = 0$ from the constraint in (A2) yields that
\begin{align}
\| h (\bm{x}_{k+1}) \| &\leq \| h (\bm{z}_k) \| + c \| \bm{x}_{k+1} - \bm{z}_k \|^2 \leq \| h (\bm{z}_k) \| + c \| \bm{x}_{k+1} - \bm{x}_k^* \|^2 + c \| \bm{z}_k - \bm{x}_k^* \|^2 \label{NPASA8.14}
\end{align}
As $\| h (\bm{z}_k) \| \leq c \| h (\bm{x}_k) \|^2$ from (\ref{NewtonYSchemeThm.3}) in Theorem~\ref{NewtonYSchemeThm}, substituting the bounds established in (\ref{NPASA8.2}) and (\ref{NPASA8.3.1}) into (\ref{NPASA8.14}) yields
\begin{align}
\| h (\bm{x}_{k+1}) \| &\leq c \| h (\bm{x}_k) \|^2 + c \| \bm{x}_k - \bm{x}_k^* \|^2 + c \| h (\bm{x}_k) \|^4 + c \| \bm{x}_k - \bm{x}_k^* \|^4. \nonumber
\end{align}
Hence, 
\begin{align}
\| h (\bm{x}_{k+1}) \| = O (\| h (\bm{x}_k) \|^2) + O (\| \bm{x}_k^* - \bm{x}_k \|^2). \label{NPASA8.15}
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
So there exists a constant $\gamma$ such that $r_{i+1} \leq \gamma r_i^2$. Then we have
\begin{align}
r_{i+1} 
&\leq \frac{1}{\gamma} \left( \gamma r_i \right)^2 \leq \ldots \leq \frac{1}{\gamma} \left( \gamma r_1 \right)^{2^i} = r_1 \left( \gamma r_1 \right)^{2^i - 1}.
\end{align}
Now observe that
\begin{align}
r_1
&= \| \bm{z}_1 - \bm{z}_0^* \| + \| \bm{z}_1^* - \bm{z}_0^* \| \nonumber \\
&\leq c \| \bm{z}_0 - \bm{z}_0^* \|^2 \tag{Applying \ref{NPASA8.3.1} and \ref{NPASA8.11}} \\
&\leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| \bm{z}_0^* - \bm{x}^* \|^2. \tag{Applying triangle inequality and Cauchy}
\end{align}
Using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_0)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*)$ it follows that
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \|
&\leq c \| \bm{h} (\bm{z}_0) - \bm{h} (\bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|
\end{align}
which combined with the bound on $r_1$ yields
\begin{align}
r_1 &\leq c \| \bm{z}_0 - \bm{x}^* \|^2. \label{NPASA8.14.4}
\end{align}
It now follows that $r_1 \to 0$ as $\bm{z}_0 \to \bm{x}^*$. Thus, there exists a constant $c$ such that $r_i \leq c r_1 2^{-2^i - 1}$, for all $\bm{z}_0$ sufficiently close to $\bm{x}^*$. It now follows that the sequence $\{ \bm{z}_i \}_{i = 0}^{\infty}$ is Cauchy since
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i \| 
&\leq \| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{z}_i^* - \bm{z}_{i-1}^* \| + \| \bm{z}_i - \bm{z}_{i-1}^* \| \\
&\leq r_{i+1} + r_i \\
&\leq c r_1 2^{-2^i}, \label{NPASA8.15}
\end{align}
for all $i \geq 1$. Thus, $\{ \bm{z}_i \}_{i = 0}^{\infty}$ has a limit, say $\bm{z}^*$, and it follows from (\ref{NPASA8.15}) that $\bm{z}^*$ satisfies
\begin{align}
\| \bm{z}_{i} - \bm{z}^* \| &\leq c 2^{-2^i},
\end{align}
for all $i \geq 0$, hence, establishing (\ref{ConvergenceResult.1}). In particular, note that (\ref{NPASA8.15}) also implies that $\{ \bm{z}_i^* \}_{i = 0}^{\infty}$ converges to $\bm{z}^*$.

Now we claim that $\{ \left[ \bm{\nu}_i, \bm{\eta}_i \right] \}_{i = 0}^{\infty}$ converges to a limit. Let $\varepsilon > 0$ be given. As $\bm{z}_i \to \bm{z}^*$ and $\bm{z}_i^* \to \bm{z}^*$, there exists a $M \geq 0$ such that $\| \bm{z}_i - \bm{z}_i^* \| + \| \bm{z}_i - \bm{z}_i^* \|^2 < \varepsilon$, for all $i \geq M$. Hence, 
\begin{align}
\| [\bm{\nu}_{i+1} \ \bm{\eta}_{i+1}] - [\bm{\nu}_i \ \bm{\eta}_i] \| 
&\leq \| [\bm{\nu}_{i+1} \ \bm{\eta}_{i+1}] - [\bm{\nu}_i^* \ \bm{\eta}_i^*] \| + \| [\bm{\nu}_i \ \bm{\eta}_i] - [\bm{\nu}_i^* \ \bm{\eta}_i^*] \| \\
&\leq c \| \bm{z}_i - \bm{z}_i^* \| + c \| \bm{z}_i - \bm{z}_i^* \|^2 \\
&\leq c \varepsilon,
\end{align}
for all $i \geq M$. So $\{ \left[ \bm{\nu}_i, \bm{\eta}_i \right] \}_{i = 0}^{\infty}$ is Cauchy and therefore has a limit, say $\left[ \bm{\nu}^*, \bm{\eta}^* \right]$. Similarly, it follows that $\{ \left[ \bm{\nu}_i^*, \bm{\eta}_i^* \right] \}_{i = 0}^{\infty}$ converges to $\left[ \bm{\nu}^*, \bm{\eta}^* \right]$. As $E_{m,1}$ is continuous, we now have that
\begin{align}
\min_{\bm{\eta} \geq \bm{0}} E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}) 
&\leq E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}^*) 
= \lim_{i \to \infty} E_{m,1} (\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*). \label{NPASA8.15.1}
\end{align}
Since $E_{m,1} (\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*) = 0$ for all $i \geq 0$, it follows that %$E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}^*) = 0$ 
from (\ref{NPASA8.15.1}) that (\ref{ConvergenceResult.0}) holds.

Recalling (\ref{NPASA8.3.1}) and (\ref{NPASA8.11}) it follows that
\begin{align}
r_1 &= \| \bm{z}_{1} - \bm{z}_0^* \| + \| \bm{z}_{1}^* - \bm{z}_0^* \| \leq c \| \bm{z}_{0} - \bm{z}_0^* \|^2 + c \| h (\bm{z}_0) \|^2. \label{NPASA8.16}
\end{align}
Using $\bm{h}(\bm{x}^*) = \bm{0}$ we have that
\begin{align}
\| \bm{h} (\bm{z}_0) \| 
= \| \bm{h}(\bm{z}_0) - \bm{h}(\bm{x}^*) \| 
= \| \nabla \bm{h}(\xi_0) (\bm{z}_0 - \bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|, \label{NPASA8.17}
\end{align}
for some $\bm{\xi}_0$ between $\bm{z}_0$ and $\bm{x}^*$. Also, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_0)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*) = \bm{0}$ together with the fact that $\bm{h} (\bm{z}_0^*) = \bm{h} (\bm{z}_0)$ we have that
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{h}(\bm{z}_0^*) - \bm{h}(\bm{x}^*) \| 
= c \| \bm{h}(\bm{z}_0) - \bm{h}(\bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|. \label{NPASA8.17.1}
\end{align}
Hence,
\begin{align}
\| \bm{z}_0 - \bm{z}_0^* \| 
\leq \| \bm{z}_0 - \bm{x}^* \| + \| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{z}_0 - \bm{x}^* \| \label{NPASA8.17.2}
\end{align}
which, when substituted into (\ref{NPASA8.16}) with (\ref{NPASA8.17}), yields
\begin{align}
r_1 &\leq c \| \bm{z}_{0} - \bm{x}^* \|^2. \label{NPASA8.18}
\end{align}
Next, applying the triangle inequality and using (\ref{NPASA8.15}) and (\ref{NPASA8.17}) we find that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_1 \| 
&\leq \sum_{j = 1}^{i} \| \bm{z}_{j+1} - \bm{z}_{j} \| 
\leq c r_1 \sum_{j = 1}^{i} 2^{-2^i} 
\leq c r_1 
\leq c \| \bm{z}_{0} - \bm{x}^* \|^2,
\end{align}
which proves (\ref{ConvergenceResult.2}).

Next, from (\ref{NPASA8.17.1}) we have that 
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{h}(\bm{z}_0^*) - \bm{h}(\bm{x}^*) \| 
= c \| \bm{h}(\bm{z}_0) \|
\end{align}
and from (\ref{NPASA8.3.1}) and (\ref{NPASA8.17.2}) we have $\| \bm{z}_1 - \bm{z}_0^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2$. Using these together with the triangle inequality and (\ref{ConvergenceResult.3}) we have
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| 
&\leq \| \bm{z}_{i+1} - \bm{z}_1 \| + \| \bm{z}_1 - \bm{z}_0^* \| + \| \bm{z}_0^* - \bm{x}^* \|
\leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| \bm{h} (\bm{z}_0) \|,
\end{align}
concluding the proof of (\ref{ConvergenceResult.3}).

To prove the remaining parts of the theorem, we proceed by defining
\begin{align}
E_u \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) 
= \sqrt{ \| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{h}(\bm{z}) - \bm{u} \|^2 } \label{def:Eu}
\end{align}
where $\bm{u}$ is a fixed vector and we note that $E_u \in \mathcal{C}^2$ in a neighborhood of $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ by our hypotheses. First, we show that (\ref{ConvergenceResult.4}) holds. As $(\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*)$ is sufficiently close to $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$, by fixing $\bm{\eta} = \bm{\eta}_i^*$ we can apply Lemma 13.2 in \cite{Hager1993} to $E_u \left( \bm{z}, \bm{\nu}, \bm{\eta}_i^* \right)$ with $\bm{u} = \bm{h} (\bm{z}_i)$ to yield that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{\nu}_{i+1} - \bm{\nu}_i^* \| 
&\geq c_1 E_u \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \\
&= c_1 \sqrt{ \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|^2 + \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \|^2 } \\
&\geq c_1 \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|, \label{NPASA8.7}
\end{align}
for some constant $c_1$. From (\ref{lem:Lem13.2.3}) in Lemma~\ref{lem:Lem13.2} with $\bm{u}_1 = \bm{z}_{i+1}$ and $\bm{u}_2 = \bm{z}_i^*$ we have that
\begin{align}
\left\| \bm{\nu}_{i+1} - \bm{\nu}_i^* \right\| = O \left( \| \bm{z}_{i+1} - \bm{z}_i^* \| \right) \label{NPASA8.7.1}
\end{align}
which combined with (\ref{NPASA8.7}) yields
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| ^2
&\geq c_1 \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|^2. \label{NPASA8.7.2}
\end{align}
Now recall the function $\bm{\Phi} : \mathbb{R}^m \times \mathbb{R}^m \to \mathbb{R}^m$ where the $j$th component of $\bm{\Phi}$ is defined to be $\Phi_j (\bm{a}, \bm{b}) = \min \{ a_j, b_j \}$. As $(\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*)$ is a KKT point for problem (\ref{prob:Ru}), we have that $\eta_{ij}^* r_j (\bm{z}_i^*) = 0$, for $1 \leq j \leq m$. Now fix $j \in \{ 1, 2, \ldots, m \}$. Suppose $\eta_{ij}^* = 0$. As $\bm{r} (\bm{z}_{i+1}) \leq \bm{0}$, we have
\begin{align}
\Phi_j (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \eta_{ij}^*, -r_j (\bm{z}_{i+1}) \}^2
= \min \{ 0, -r_j (\bm{z}_{i+1}) \}^2
= 0. \label{NPASA8.7.3}
\end{align}
On the other hand, suppose $r_j (\bm{z}_i^*) = 0$. As $\bm{r} (\bm{z}) = \bm{A} \bm{z} - \bm{b}$, we have that
\begin{align}
\Phi_j (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \eta_{ij}^*, -r_j (\bm{z}_{i+1}) \}^2 \\
&\leq \left( r_j (\bm{z}_{i+1}) \right)^2 \\
&= \left( r_j (\bm{z}_{i+1}) - r_j (\bm{z}_i^*) \right)^2 \\
&\leq \| \bm{A} \|^2 \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.4}
\end{align}
Combining (\ref{NPASA8.7.3}) and (\ref{NPASA8.7.4}) we have that
\begin{align}
c_1 \| \bm{\Phi} (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.5}
\end{align}
Recalling that $E_{m,1} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) = \| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{\Phi} (\bm{\eta}, -\bm{r} (\bm{z})) \|^2$ it follows from (\ref{NPASA8.7.2}) and (\ref{NPASA8.7.5}) that 
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) 
\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.6}
\end{align}
Recalling (\ref{scheme:MS2}) we have that $\bm{\eta}_{i+1}' \in \arg\min \left\{ E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta} \right) : \bm{\eta} \geq \bm{0} \right\}$. As $\bm{\eta}_{i+1}^* \geq \bm{0}$, it follows from (\ref{NPASA8.7.6}) and (\ref{scheme:MS2}) that
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) 
&\leq c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right)
\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.8}
\end{align}
Next, applying Theorem~\ref{thm:E1-error-bound} to problem (\ref{prob:Ru}) with $\bm{u} = \bm{h} (\bm{z}_i)$ yields that
\begin{align}
\| \bm{z}_i - \bm{z}_i^* \|^2 
%&\leq c_2 \left( \| \nabla \mathcal{L} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \|^2 + \| \bm{h}(\bm{z}_i) - \bm{h}(\bm{z}_i) \|^2 + \| \bm{\Phi} (\bm{\eta}_i', -\bm{r} (\bm{z}_i)) \|^2 \right) \nonumber \\
&\leq c_2 \left( \| \nabla \mathcal{L} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \|^2 + \| \bm{\Phi} (\bm{\eta}_i', -\bm{r} (\bm{z}_i)) \|^2 \right) %\nonumber \\
= c_2 E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right). \label{NPASA8.7.9}
\end{align}
Now combining (\ref{NPASA8.3.1}), (\ref{NPASA8.7.8}), and (\ref{NPASA8.7.9}) yields
\begin{align}
E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right)
&\leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2, \label{NPASA8.7.10}
\end{align}
which proves (\ref{ConvergenceResult.4}).

Now we show that (\ref{ConvergenceResult.5}) holds. By definition of (\ref{def:Eu}) and the fact that $\bm{h} (\bm{x}^*) = \bm{0}$, note that $E_u \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) = \sqrt{\| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{h} (\bm{z}) \|^2}$ when $\bm{u} = \bm{h}(\bm{x}^*)$. So by fixing $\bm{\eta} = \bm{\mu}^*$ then appliyng Lemma 13.2 in \cite{Hager1993} to $E_u \left( \bm{z}, \bm{\nu}, \bm{\mu}^* \right)$ with $\bm{u} = \bm{h}(\bm{x}^*)$ we have that there exists a constant $c_1$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| + \| \bm{\nu}_{i+1} - \bm{\lambda}^* \|
&\geq c_1 E_u \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \\
&= c_1 \sqrt{\| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \|^2 + \| \bm{h} (\bm{z}_{i+1}) \|^2}. \label{NPASA8.8}
\end{align}
From (\ref{lem:Lem13.2.3}) in Lemma~\ref{lem:Lem13.2} with $\bm{u}_1 = \bm{z}_{i+1}$ and $\bm{u}_2 = \bm{x}^*$ we have
\begin{align}
\left\| \bm{\nu}_{i+1} - \bm{\lambda}^* \right\| = O \left( \| \bm{z}_{i+1} - \bm{x}^* \| \right) \label{NPASA8.8.1}
\end{align}
which combined with (\ref{NPASA8.8}) yields
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| ^2
&\geq c_1 \left( \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \|^2 + \| \bm{h} (\bm{z}_{i+1}) \|^2 \right). \label{NPASA8.8.2}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Now recall the function $\bm{\Phi} : \mathbb{R}^m \times \mathbb{R}^m \to \mathbb{R}^m$ where the $j$th component of $\bm{\Phi}$ is defined to be $\Phi_j (\bm{a}, \bm{b}) = \min \{ a_j, b_j \}$. As $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}), we have that $\mu_j^* r_j (\bm{x}^*) = 0$, for $1 \leq j \leq m$. Now fix $j \in \{ 1, 2, \ldots, m \}$. Suppose $\mu_j^* = 0$. As $\bm{r} (\bm{z}_{i+1}) \leq \bm{0}$, we have
\begin{align}
\Phi_j (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \mu_j^*, -r_j (\bm{z}_{i+1}) \}^2
= \min \{ 0, -r_j (\bm{z}_{i+1}) \}^2
= 0. \label{NPASA8.8.3}
\end{align}
On the other hand, suppose $r_j (\bm{x}^*) = 0$. Then
\begin{align}
\Phi_j (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \mu_j^*, -r_j (\bm{z}_{i+1}) \}^2 \nonumber \\
&\leq \left( r_j (\bm{z}_{i+1}) \right)^2 \nonumber \\
&= \left( r_j (\bm{z}_{i+1}) - r_j (\bm{x}^*) \right)^2 \nonumber \\
&\leq c \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.4}
\end{align}
Combining (\ref{NPASA8.8.3}) and (\ref{NPASA8.8.4}) we have that there exists a constant $c$ such that
\begin{align}
\| \bm{\Phi} (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq c \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.5}
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By an argument similar to the one establishing (\ref{NPASA8.7.5}), we can show that
\begin{align}
c_1 \| \bm{\Phi} (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.5}
\end{align}
%Recalling that $E_{m,1} \left( \bm{x}, \bm{\lambda}, \bm{\mu} \right) = \| \nabla \mathcal{L} \left( \bm{x}, \bm{\lambda}, \bm{\mu} \right) \|^2 + \| \bm{\Phi} (\bm{\mu}, -\bm{r} (\bm{x})) \|^2$ 
It now follows from (\ref{NPASA8.8.2}) and (\ref{NPASA8.8.5}) that 
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) 
\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.6}
\end{align}
As $\bm{\mu}^* \geq \bm{0}$, using the definition of $\bm{\eta}_{i+1}'$ in (\ref{scheme:MS2}) with (\ref{NPASA8.8.6}) we now have
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) 
&\leq c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right)
\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.8}
\end{align}
Finally, recalling that $E_1 \left( \bm{z}, \bm{\nu}, \bm{\eta} \right)^2 = E_{m,1} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) + \| \bm{h} (\bm{z}) \|^2$ it follows from (\ref{NPASA8.8.2}) and (\ref{NPASA8.8.8}) that
\begin{align}
E_1 \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c \| \bm{z}_{i+1} - \bm{x}^* \|, \label{NPASA8.8.9}
\end{align}
which concludes the proof of (\ref{ConvergenceResult.5}).
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Note that we can obtain the same convergence guarantees without assuming (\textbf{SCS}) provided that we substitute assumption (\textbf{SOSC}) with the slightly stronger assumption (\textbf{SSOSC}).

\begin{theorem} \label{ConvergenceResultAlt}
Suppose that $f, \bm{h} \in \mathcal{C}^2$ and that assumptions (\textbf{LI}) and (\textbf{SSOSC}) are satisfied for problem (\ref{prob:main-nlp}) at a point $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. %If $p_k$ is chosen such that $p_k \geq 1$ and $\frac{1}{p_k} \leq \| h (\bm{x}_k) \|^2$ for all $k \geq 0$ then 
Then the conclusions of Theorem~\ref{ConvergenceResult} hold.
\end{theorem}

The proof of Theorem~\ref{ConvergenceResultAlt} is essentially identical to the proof of Theorem~\ref{ConvergenceResult}. The only difference between the proofs are the assumptions guaranteeing strong regularity of the KKT system for problem (\ref{prob:main-nlp}) so that Lemma~\ref{lem:Lem13.1} can be applied. %In Section 4 of his paper \cite{Robinson1980}, Robinson outlines necessary conditions for strong regularity which are required to obtain the bound in (\ref{NPASA8.3}). 
With the alternative set of hypotheses in Theorem~\ref{ConvergenceResultAlt}, it follows from Section 4 of \cite{Robinson1980} that the strong regulatiry assumption is satisfied without requiring (\textbf{SCS}). 
%However, the absence of the strict complementary slackness assumption causes the hypotheses of Lemma~\ref{lem:E1diff} to no longer be satisfied. As a result, the proof of Theorem~\ref{ConvergenceResultAlt} only holds for $E_{m,0}$. 
%It should also be noted that argument estabilishing (\ref{NPASA8.7}) and (\ref{NPASA8.8}) fails to hold for $E_{m,1}$ as it requires that $E_{m,1} \in \mathcal{C}^2$ in a neighborhood of $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ which is not necessarily true in the absence of strict complementary slackness.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ------------------------ CMS: LOCAL CONVERGENCE ----------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Local Convergence of Phase Two of NPASA} \label{subsec:npasa-phase-two-local-conv}
Now that we have established local convergence results for the constraint and multiplier step problems, we are ready to provide a local convergence result for phase two of NPASA. Phase two of NPASA is comprised of the CMS algorithm, Algorithm~\ref{alg:cms}, and branching criterion. We note that (\ref{cor:PhaseTwoConvergence.0}) and its proof are similar to Corollary 5.1 and its proof from \cite{Hager1993}.

\begin{corollary} \label{cor:PhaseTwoConvergence}
Suppose that $f, \bm{h} \in \mathcal{C}^2$ and that either assumptions (\textbf{LI}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LI}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Then there exists a neighborhood $\mathcal{N}_1$ of $\bm{x}^*$ and a constant $c$ such that, for every $\bm{x}_0 \in \mathcal{N}_1 \cap \Omega$ and every $k \geq 0$, the iterates of phase two of NPASA satisfy
\iffalse
\begin{itemize}
\item[(\ref{cor:PhaseTwoConvergence}.0)] $\| \bm{x}_{k+1} - \bm{x}^* \| \leq c \| \bm{x}_{k} - \bm{x}^* \|^2$,
\item[(\ref{cor:PhaseTwoConvergence}.1)] $E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) \leq c E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2$.
\end{itemize}
\fi
\begin{align}
    &\| \bm{x}_{k+1} - \bm{x}^* \| \leq c \| \bm{x}_{k} - \bm{x}^* \|^2, \label{cor:PhaseTwoConvergence.0} \\
    &E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) \leq c E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2. \label{cor:PhaseTwoConvergence.1}
\end{align}
\end{corollary}

\begin{proof}
The proof of (\ref{cor:PhaseTwoConvergence.0}) follows from applying Theorems~\ref{NewtonYSchemeThm} and~\ref{ConvergenceResult}. Observe that
\begin{align}
\| \bm{x}_{k+1} - \bm{x}^* \| 
&\leq c \| \bm{w}_{i_C} - \bm{x}^* \|^2 + c \| \bm{h} (\bm{w}_{i_C}) \| \tag{Applying \ref{ConvergenceResult.5}} \\
&\leq c \| \bm{w}_{i_C} - \bm{x}^* \|^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Applying \ref{NewtonYSchemeThm.3}} \\
&\leq c \left( \| \bm{w}_{i_C} - \bm{x}_k \| + \| \bm{x}_k - \bm{x}^* \| \right)^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Using triangle inequality} \\
&\leq c \left( \| \bm{h} (\bm{x}_k) \| + \| \bm{x}_k - \bm{x}^* \| \right)^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Applying \ref{NewtonYSchemeThm.1}} \\
&\leq \frac{5c}{2} \| \bm{h} (\bm{x}_k) \|^2 + \frac{3c}{2} \| \bm{x}_k - \bm{x}^* \|^2. \tag{Using Cauchy inequality}
\end{align}
By performing a first-order Taylor expansion of $\bm{h} (\bm{x})$ and using the fact that $\bm{h} (\bm{x}^*) = \bm{0}$, there exists some $\bm{\xi}_k$ between $\bm{x}_k$ and $\bm{x}^*$ such that $\bm{h} (\bm{x}_k) = \nabla \bm{h} (\bm{\xi}_k) (\bm{x}_k - \bm{x}^*)$. Hence, $\| \bm{h} (\bm{x}_k) \| \leq c \| \bm{x}_k - \bm{x}^* \|$. Making this substitution into our previous inequality yields
\begin{align}
\| \bm{x}_{k+1} - \bm{x}^* \| 
&\leq \frac{5c^2}{2} \| \bm{x}_k - \bm{x}^* \|^2 + \frac{3c}{2} \| \bm{x}_k - \bm{x}^* \|^2 
= C \| \bm{x}_k - \bm{x}^* \|^2,
\end{align}
which proves (\ref{cor:PhaseTwoConvergence.0}).

To prove (\ref{cor:PhaseTwoConvergence.1}), we use (\ref{ConvergenceResult.5}), (\ref{cor:PhaseTwoConvergence.0}), and Theorem~\ref{thm:E1-error-bound}. Observe that
\begin{align}
E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) 
&\leq C \| \bm{x}_{k+1} - \bm{x}^* \| \tag{Applying \ref{ConvergenceResult.5}} \\
&\leq C \| \bm{x}_k - \bm{x}^* \|^2 \tag{Applying \ref{cor:PhaseTwoConvergence.0}} \\
&\leq C E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2, \tag{Applying Theorem~\ref{thm:E1-error-bound}}
\end{align}
which concludes the proof.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We can obtain a similar result with an alternate set of assumptions.
%, however, this alternative result only holds when the error estimator $E_0$ is used in NPASA. 
The proof is nearly identical to the proof of Corollary~\ref{cor:PhaseTwoConvergence} with the only difference being the application of Theorem~\ref{ConvergenceResultAlt} instead of Theorem~\ref{ConvergenceResult}.

\begin{corollary} \label{cor:PhaseTwoConvergenceAlt}
Suppose that $f, \bm{h} \in \mathcal{C}^2$ and that assumptions (\textbf{LI}) and (\textbf{SSOSC}) are satisfied for problem (\ref{prob:main-nlp}) at a point $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Then the conclusions of Theorem~\ref{cor:PhaseTwoConvergence} hold.
\end{corollary}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> local-phase-two-no-g.tex <==
\section{Convergence Analysis for Phase Two of NPASA} \label{section:npasa-phase-two}
In this section, we provide conditions under which phase two of NPASA satisfies desirable local convergences properties. From the pseodocode of Algorithm~\ref{alg:npasa}, recall that phase two of NPASA consists of the constraint and multiplier steps. First, we prove fast local convergence properties of the constraint step in Section~\ref{subsec:constraint-step-analysis}. Then we provide a local convergence analysis of the multiplier step of NPASA in Section~\ref{subsec:multiplier-step-analysis}. Lastly, we use our analysis of both steps to provide a local convergence result for the CMS algorithm in Section~\ref{subsec:npasa-phase-two-local-conv}. 
%To establish our convergence result we make use of some sensitivity analysis from \cite{Robinson} which require the following assumptions:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

For several results in this section we will require some subset of the assumptions (\textbf{LICQ}), (\textbf{SCS}), (\textbf{SOSC}), and (\textbf{SSOSC}) provided in Section~\ref{section:introduction}. We will clearly specify which assumptions are used in the statement of each convergence result. Additionally, note that for the purposes of simplifying the analysis for several results in Sections~\ref{subsec:constraint-step-analysis} and \ref{subsec:multiplier-step-analysis}, we will express the polyhedral constraint set for problem (\ref{prob:main-nlp}), originally defined by $\Omega = \{ \bm{x} : \bm{r}(\bm{x}) \leq \bm{0} \}$, in an equivalent form $\Omega = \{ \bm{x} : \bm{g} (\bm{x}) = \bm{0} \}$, for some function $\bm{g} (\bm{x})$. Note that this equivalent formulation of $\Omega$ can be constructed by adding a slack variable to the inequality constraints in problem (\ref{prob:main-nlp}) and performing a change of variables to define $\bm{g} (\cdot)$, as illustrated in Section 3.3.2 of \cite{bertsekas1995nonlinear}. Further, using this approach we have that $\nabla \bm{g}(\bm{x})$ is of full row rank provided that $\bm{A}$ is of full row rank. It should be noted that in the actual implementation of this method we will still use the definition of the set $\Omega$ as originally defined in Section~\ref{section:introduction}.% so that problem %(\ref{NewtonYScheme}) 
%in line 5 of Algorithm~\ref{alg:cms}, the CMS algorithm, can be solved using PPROJ \cite{Hager2016}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ------------- INFEASIBILITY DETECTION FOR CONSTRAINT STEP ------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Algorithm with Infeasibility Detection for Solving Constraint Step} \label{subsec:infeas}
\iffalse
In order to simplify the notation in our discussion of this problem, we express the linearized constraint set as
\begin{align*}
\left\{ \bm{w} \in \mathbb{R}^n : \bm{M} (\bm{w} - \bar{\bm{w}}) = \bm{c}, \bm{w} \geq \bm{0} \right\}
\end{align*}
supposing that we are given $\bm{M} \in \mathbb{R}^{m \times n}$, $\bm{c} \in \mathbb{R}^m$, and $\bar{\bm{w}} \in \mathbb{R}^n$. Ideally, we would like to determine the solution to the problem 
\begin{align}
&\min_{\bm{w} \in \mathcal{S}} \ \frac{1}{2} \| \bm{w} - \bar{\bm{w}} \|^2, \label{Sprob}
\end{align}
%\begin{align}
%&\min_{x \geq 0} \ \frac{1}{2} \| b - A(x - \bar{x}) \|^2, \label{FeasibilityProb}
%\end{align}
%%%given $A$, $b$, and $\bar{x}$. 
%Ideally, if we knew a solution to problem (\ref{FeasibilityProb}) then we would know whether or not $\mathcal{F}_0 = \emptyset$ since $\mathcal{F}_0 = \emptyset$ if and only if $\| b - A(x - \bar{x}) \| > 0$ for all $x \geq 0$. 
where $\mathcal{S} = \arg\min_{\bm{w} \geq \bm{0}} \left\{ \| \bm{c} - \bm{M} (\bm{w} - \bar{\bm{w}}) \|^2 \right\}$. Since problem (\ref{Sprob}) involves minimizing a strongly convex objective function over a convex set, there exists a unique solution which we will denote by $\bm{w}_{\infty}$. As such, every search direction from $\bm{w}_{\infty}$ leading to a point in $\mathcal{S}$ must be an ascent direction. Hence, the first order optimality conditions for $\bm{w}_{\infty}$ can be expressed as 
\begin{align}
\langle \bm{w}_{\infty} - \bar{\bm{w}}, \bm{w} - \bm{w}_{\infty} \rangle \geq 0, \ \text{for all} \ \bm{w} \in \mathcal{S}. \label{problemS}
\end{align}
Since determining elements of the constraint set for problem (\ref{Sprob}) requires knowing all minimizers of $\| \bm{c} - \bm{M}(\bm{w} - \bar{\bm{w}}) \|$ we consider an alternative problem. 

First, we define the sets 
\begin{align*}
\mathcal{F}_{\delta} = \left\{ 
\begin{bmatrix}
\bm{w} \\
\bm{y}
\end{bmatrix} \in \mathbb{R}^{n+m} : \bm{M}(\bm{w} - \bar{\bm{w}}) + \bm{y} = \bm{c}, \bm{w} \geq \bm{0}, \| \bm{y} \|^2 \leq \delta \right\}
\end{align*}
and 
\begin{align*}
\mathcal{F} = \left\{ 
\begin{bmatrix}
\bm{w} \\
\bm{y}
\end{bmatrix} \in \mathbb{R}^{n+m} : \bm{M}(\bm{w} - \bar{\bm{w}}) + \bm{y} = \bm{c}, \bm{w} \geq \bm{0} \right\}.
\end{align*}
Now, given a penalty parameter $p > 0$, we define the problem
\begin{align}
\min_{[\bm{w}, \bm{y}] \in \mathcal{F}} \ \ f_p(\bm{w},\bm{y}) := \frac{1}{2} \| \bm{w} - \bar{\bm{w}} \|^2 + \frac{p}{2} \| \bm{y} \|^2. \label{prob:Pp}
\end{align}
Since problem (\ref{prob:Pp}) involves minimizing a strongly convex objective function over a convex set, it has a unique solution which we will denote by $[ \bm{w}_p, \bm{y}_p]^{\intercal}$. Note that the first order optimality conditions for $[ \bm{w}_p, \bm{y}_p ]^{\intercal}$ can be expressed as
\begin{align}
\langle \bm{w}_p - \bar{\bm{w}}, \bm{w} - \bm{w}_p \rangle + p \langle \bm{y}_p, \bm{y} - \bm{y}_p \rangle \geq 0, \ \text{for all} \ [\bm{w}, \bm{y}]^{\intercal} \in \mathcal{F}. \label{POptCond}
\end{align}
We should note here that while the number of primal variables in (\ref{prob:Pp}) is greater than that of problem (\ref{Sprob}), the dimension of the dual variables is the same for problems (\ref{Sprob}) and (\ref{prob:Pp}). So we can use PPROJ \cite{Hager2016} to solve for problem (\ref{prob:Pp}) without the cost of solving for additional dual variables.
%%%That is, the complexity is the same for solving (P) and (\ref{prob:Pp}) using PPROJ \cite{Hager2016}. 
The following result provides valuable insight on the relationship between $\bm{w}_p$ and $\bm{w}_{\infty}$. 

\begin{theorem} \label{thm:feasibility-detection}
Let $[\bm{w}_p, \bm{y}_p]^{\intercal}$ be the unique solution to problem \emph{(\ref{prob:Pp})}. Then 
\begin{align*}
\| \bm{w}_p - \bm{x}_{\infty} \| = O \left( \frac{1}{p} \right),
\end{align*}
for all $p > 0$ sufficiently large.
%%%where $x_{\infty} \in \mathcal{S}$ is the closest solution to $\bar{x}$.	
\end{theorem}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ----------------------- CONSTRAINT STEP ANALYSIS ---------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Analysis for Constraint Step} \label{subsec:constraint-step-analysis}
In this section, we establish a local quadratic convergence rate of the multiplier error estimator $E_c$. Recall the iterative scheme for determining $\bm{w} \in \Omega$ such that $\bm{h} (\bm{w}) = \bm{0}$ used in the constraint step of the CMS algorithm for a given initial point $\bm{w}_0$:
\begin{align}
(\bm{w}_{i+1}, \bm{y}_{i+1}) &= \arg\min \left\{\| \bm{w} - \bm{w}_i \|^2 + \| \bm{y} \|^2 : \nabla \bm{h} (\bm{w}_i) (\bm{w} - \bm{w}_i) + \frac{1}{\sqrt{p_i}} \bm{y} = - \bm{h} (\bm{w}_i), \bm{w} \in \Omega \right\} \label{NewtonYScheme} \\
\bm{w}_{i+1} &\gets \bm{w}_i + s_i ( \bm{w}_{i+1} - \bm{w}_i) 
\end{align}
where $p_i \geq 1$ is a penalty parameter and where $s_i \leq 1$ is chosen such that
\begin{align}
\| \bm{h} (\bm{w}_i + s_i (\bm{w}_{i+1} - \bm{w}_{i})) \| \leq (1 - \tau \alpha_i s_i) \| \bm{h} (\bm{w}_i) \|. \label{NewtonArmijo}
\end{align} 
Here, $\alpha_i$ is defined by $\alpha_i := 1 - \| \bm{y}_i \|$ and to continue performing the scheme we require that $\alpha_i \in [\alpha, 1]$ for some fixed parameter $\alpha > 0$. Note that this is the iterative scheme in the constraint step of the CMS algorithm, Algorithm~\ref{alg:cms}, where we have made the change of variables $\bm{y} \gets \frac{1}{\sqrt{p_i}} \bm{y}$ to simplify the analysis in Theorem~\ref{NewtonYSchemeThm}. By introducing the slack variable, $\bm{y}$, into our update scheme, it is no longer necessary to consider the solvability of this problem as the constraint set is always nonempty. However, Theorem~\ref{NewtonYSchemeThm} serves to update the convergence analysis performed in Theorem 2.1 of \cite{Hager1993} to account for the presence of the slack variable $\bm{y}$ and penalty parameter $p_i$ in (\ref{NewtonYScheme}). 

\begin{theorem} \label{NewtonYSchemeThm}
Suppose $\bm{x}^*$ satisfies $\bm{h} (\bm{x}^*) = \bm{0}$, $\bm{x}^* \in \Omega$, $\bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and that assumption (\textbf{LICQ}) holds at $\bm{x}^*$. Then there exists a neighborhood $\mathcal{N}$ about $\bm{x}^*$ and a constant $c \in \mathbb{R}$ such that for any $\bm{w}_0 \in \mathcal{N} \cap \Omega$ and sequence of penalty parameters $\{ p_i \}_{i = 0}^{\infty}$ satisfying $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, with $\beta \geq 1$, the iterative scheme (\ref{NewtonYScheme}) converges to a point $\bm{w}^*$ with the following properties: 
\iffalse
\begin{itemize}
\item[(\ref{NewtonYSchemeThm}.0)] $\bm{h}(\bm{w}^*) = \bm{g}(\bm{w}^*) = \bm{0}$ and $s_i = 1$ satisfies the Armijo line search given by (\ref{NewtonArmijo}) for each $i$.
\end{itemize}
\fi
\begin{align}
\bm{h}(\bm{w}^*) = \bm{0}, \bm{w}^* \in \Omega, \ \text{and} \ s_i = 1 \ \text{satisfies Armijo line search given by (\ref{NewtonArmijo}) for each $i$}. \label{NewtonYSchemeThm.0}
\end{align}
Moreover, for all $i \geq 0$:
\iffalse
\begin{itemize}
\item[(\ref{NewtonYSchemeThm}.1)] $\| \bm{w}_i - \bm{w}_0 \| \leq c \| \bm{h}(\bm{w}_0) \|$
\item[(\ref{NewtonYSchemeThm}.2)] $\| \bm{w}_i - \bm{w}^* \| \leq c \| \bm{h}(\bm{w}_0) \| 2^{-2^i}$
\item[(\ref{NewtonYSchemeThm}.3)] $\| \bm{h}(\bm{w}_{i+1}) \| \leq c \| \bm{h}(\bm{w}_i) \|^2$.
\end{itemize}
\fi
\begin{align}
\| \bm{w}_i - \bm{w}_0 \| &\leq c \| \bm{h}(\bm{w}_0) \|, \label{NewtonYSchemeThm.1} \\
\| \bm{w}_i - \bm{w}^* \| &\leq c \| \bm{h}(\bm{w}_0) \| 2^{-2^i}, \label{NewtonYSchemeThm.2} \\
\| \bm{h}(\bm{w}_{i+1}) \| &\leq c \| \bm{h}(\bm{w}_i) \|^2. \label{NewtonYSchemeThm.3}
\end{align}
\end{theorem} 

\begin{proof}
Let $\mathcal{S} \subseteq [m] := \{ 1, 2, \ldots, m \}$ and let $\mathcal{A} := \mathcal{A} (\bm{x}^*)$, for simplicity. Define $\bm{F}_{p, \mathcal{S}}: \mathbb{R}^{|\mathcal{S}| + 2 \ell} \times \mathbb{R}^{n} \to \mathbb{R}^{|\mathcal{S}| + 2 \ell}$ by
\begin{align}
\bm{F}_{p,\mathcal{S}} (\bm{u}, \bm{y}, \bm{x}) 
&= \begin{bmatrix}
\nabla \bm{h} (\bm{x}) \bm{M}_{\mathcal{S}}(\bm{x}) \bm{u} + \frac{1}{\sqrt{p}} \bm{y} + \bm{h} (\bm{x}) \\
\bm{r}_{\mathcal{S}} \left( \bm{x} + \bm{M}_{\mathcal{S}}(\bm{x}) \bm{u} \right) \\
\bm{y}
\end{bmatrix}
\end{align}
where $\bm{u} \in \mathbb{R}^{\ell + |\mathcal{S}|}$, $\bm{y} \in \mathbb{R}^{\ell}$, $\bm{M}_{\mathcal{S}}(\bm{x}) = \left[ \nabla \bm{h} (\bm{x})^{\intercal} \ \vert \ \bm{A}_{\mathcal{S}}^{\intercal} \right] \in \mathbb{R}^{n \times (\ell + |\mathcal{S}|)}$, and $p \geq 1$ is a scalar. Additionally, let $\psi_{\mathcal{C}} (\bm{x})$ be the normal cone operator \textcolor{red}{(give definition)}. Taking $\mathcal{S} = [m]$, we claim that there exists neighborhoods $\mathcal{N}_1$ of $[\bm{0}, \bm{0}] \in \mathbb{R}^{\ell + m} \times \mathbb{R}^{\ell}$ and $\mathcal{N}_2$ of $\bm{x}^* \in \mathbb{R}^n$ such that the generalized equation 
\begin{align}
\bm{0} \in \bm{F}_{p,[m]} (\bm{u}, \bm{y}, \bm{x}) + \psi_{\mathbb{R}^{\ell + |\mathcal{S}|} \times \mathbb{R}^{\ell}} (\bm{u}, \bm{y}) \label{reg-gen-eq.1}
\end{align}
has a unique solution $[\bm{u}, \bm{y}] = [\bm{u}_p (\bm{x}), \bm{y}_p (\bm{x})]$ in $\mathcal{N}_1$ for every $\bm{x} \in \mathcal{N}_2$. To prove this claim, we will make use of Theorem~2.1 in \cite{Robinson1980}. It follows from Corollary~3.2 in \cite{Robinson1980} that if $\nabla_{[u, y]} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*)$ is nonsingular and the Lipschitz constant of $\nabla_{[u, y]} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*)^{-1}$ is uniformly bounded for sufficiently large values of $p$ then the hypothesis of Theorem~2.1 in \cite{Robinson1980} is satisfied for equation (\ref{reg-gen-eq.1}). Evaluating the Jacobian of $\bm{F}_{p,\mathcal{A}}$ with respect to $[\bm{u}, \bm{y}]$ at $\bm{u} = \bm{0}$, $\bm{y} = \bm{0}$, and $\bm{x} = \bm{x}^*$ yields
\begin{align}
\nabla_{[u, y]} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*) 
&= \begin{bmatrix}
\nabla_{u} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*) \ \vert \ \nabla_{y} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*)
\end{bmatrix}
= \left[
\begin{array}{c|c}
\multirow{2}{*}{$\bm{M}_{\mathcal{A}}(\bm{x}^*)^{\intercal} \bm{M}_{\mathcal{A}}(\bm{x}^*)$} & \frac{1}{\sqrt{p}} \bm{I}_{\ell} \\
 & \bm{0} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right]
\end{align}
which is nonsingular by the (\textbf{LICQ}) hypothesis and choice of $\bm{M}_{\mathcal{A}}(\bm{x})$. Note that $\bm{I}_{\ell}$ denotes the identity matrix of dimension $\ell \times \ell$. It remains to shows that the Lipschitz constant of $\nabla_{[u, y]} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*)^{-1}$ is uniformly bounded for sufficiently large values of $p$. For simplicity, define $\bm{B}_p := \nabla_{[u, y]} \bm{F}_{p,\mathcal{A}} (\bm{0}, \bm{0}, \bm{x}^*)^{-1}$, $\bm{C} := \left( \bm{M}_{\mathcal{A}}(\bm{x}^*)^{\intercal} \bm{M}_{\mathcal{A}}(\bm{x}^*)\right)^{-1}$, and 
\begin{align}
\bm{D} := \bm{C} \begin{bmatrix}
\bm{I}_{\ell} \\
\bm{0}
\end{bmatrix}
\end{align} 
and observe that 
\begin{align}
\bm{B}_p = \left[
\begin{array}{c|c}
\bm{C} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right].
\end{align}
As the desired Lipschitz constant is given by $\| \bm{B}_p \|$, it suffices to determine the singular values of $\bm{B}_p$. Since 
\begin{align}
\bm{B}_p \bm{B}_p^{\intercal} &= \left[
\begin{array}{c|c}
\bm{C} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline
\bm{0} & \bm{I}_{\ell}
\end{array}
\right] \left[
\begin{array}{c|c}
\bm{C}^{\intercal} & \bm{0} \\
\hline 
\frac{1}{\sqrt{p}} \bm{D}^{\intercal} & \bm{I}_{\ell}
\end{array}
\right]
= \left[
\begin{array}{c|c}
\bm{C} \bm{C}^{\intercal} + \frac{1}{p} \bm{D} \bm{D}^{\intercal} & \frac{1}{\sqrt{p}} \bm{D} \\
\hline 
\frac{1}{\sqrt{p}} \bm{D}^{\intercal} & \bm{I}_{\ell}
\end{array}
\right]
\end{align}
we have that
\begin{align}
\lim_{p \to \infty} \bm{B}_p \bm{B}_p^{\intercal} = \left[
\begin{array}{c|c}
\bm{C} \bm{C}^{\intercal} & \bm{0} \\
\hline 
\bm{0} & \bm{I}_{\ell}
\end{array}
\right]. \label{NewtonYThm.3}
\end{align}
As the matrix in (\ref{NewtonYThm.3}) is a block diagonal matrix, its eigenvalues are the eigenvalues of $\bm{C} \bm{C}^{\intercal}$ and $\bm{I}_{\ell}$. As the nonzero singular values of $\bm{B}_p$ are the square roots of the nonzero eigenvalues of $\bm{B}_p \bm{B}_p^{\intercal}$, we conclude that the singular values of $\bm{B}_p$ are uniformly bounded for sufficiently large $p$. Hence, the hypothesis of Theorem~2.1 in \cite{Robinson1980} holds for equation (\ref{reg-gen-eq.1}). Thus, there exist neighborhoods $\mathcal{N}_1$ of $[\bm{0}, \bm{0}]$ and $\mathcal{N}_2$ of $\bm{x}^*$ such that equation (\ref{reg-gen-eq.1}) has a unique solution $[\bm{u}, \bm{y}] = [\bm{u}_p (\bm{x}), \bm{y}_p (\bm{x})]$ in $\mathcal{N}_1$ for every $\bm{x} \in \mathcal{N}_2$. Further, Theorem 2.1 of \cite{Robinson1980} yields that %this solution satisfies 
$\| [ \bm{u}_p (\bm{x}), \ \bm{y}_p (\bm{x}) ] \| 
&\leq \sigma \| \bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}) - \bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}^*) \|$, for all $\bm{x} \in \mathcal{N}_2$ and sufficiently large $p$, where $\sigma$ is independent of $\bm{x}$ and $p$. 
It follows from the definition of $\bm{F}_{p,[m]}(\bm{u}, \bm{y}, \bm{x})$ and equation (\ref{reg-gen-eq.1}) that $\bm{y}_p(\bm{x}) = \bm{0}$ for every $\bm{x} \in \mathcal{N}_2$ which, in turn, yields
\begin{align}
\| \bm{u}_p (\bm{x}) \| 
&\leq \sigma \| \bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}) - \bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}^*) \|.
\end{align}
Observing that
\begin{align}
\bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}) &= \begin{bmatrix}
\nabla \bm{h} (\bm{x}) \bm{M}(\bm{x}) \bm{0} + \frac{1}{\sqrt{p}} \bm{0} + \bm{h} (\bm{x}) \\
\bm{g} \left( \bm{x} + \bm{M}(\bm{x}) \bm{0} \right) \\
\bm{0}
\end{bmatrix} = \begin{bmatrix}
\bm{h} \left( \bm{x} \right) \\
\bm{g} \left( \bm{x} \right) \\
\bm{0}
\end{bmatrix}
\end{align}
and
\begin{align}
\bm{F}_{p,[m]} (\bm{0}, \bm{0}, \bm{x}^*) &= \begin{bmatrix}
\bm{h} \left( \bm{x}^* \right) \\
\bm{g} \left( \bm{x}^* \right) \\
\bm{0}
\end{bmatrix} = \begin{bmatrix}
\bm{0} \\
\bm{0} \\
\bm{0}
\end{bmatrix}
\end{align}
we now have that
\begin{align}
\| \bm{u}_p (\bm{x}) \| &\leq \sigma \left\| \begin{bmatrix}
\bm{h} \left( \bm{x} \right) \\
\bm{g} \left( \bm{x} \right)
\end{bmatrix} \right\|, \label{NewtonYThm.4}
\end{align}
for all $\bm{x} \in \mathcal{N}_2$.

Now let $\eta >0$ be given such that $\bm{h}, \bm{g} \in \mathcal{C}^2 (\mathcal{B} (\bm{x}^*, \eta))$ and $\mathcal{B} (\bm{x}^*, \eta) \subset \mathcal{N}_2$. Define $\mathcal{B} := \mathcal{B} (\bm{x}^*, \eta)$. Let
\begin{align}
\eta &= \max \left\{ \max_{\bm{x} \in \mathcal{B}} \| \bm{M}(\bm{x}) \|, 1 \right\}, \\
\delta &= \left[ \sum_{j = 1}^{\ell} \max_{\bm{x}_j \in \mathcal{B}} \| \nabla^2 \bm{h}_j ( \bm{x}_j ) \|^2 \right]^{1/2},
\end{align} 
and let $\bm{w}_0 \in \mathcal{B} \cap \Omega$ be any point such that both
\begin{align}
\eta \sigma \gamma \| \bm{h}(\bm{w}_0) \| \leq \min \left\{ 1/2, 1 - \tau, \gamma (1 - \alpha) \right\} \label{NewtonYThm.4.1}
\end{align}
and $\mathcal{B} ( \bm{w}_0, 2 \eta \sigma \gamma \| \bm{h}(\bm{w}_0) \|) \subseteq \mathcal{B} \cap \Omega$, where $\displaystyle \gamma = \left( 1 + \frac{\delta \eta \sigma}{2} \right)$.

Suppose that $\bm{w}_i \in \mathcal{B} \cap \Omega$ and that $\bm{w}_{i+1}$ is generated using the scheme in (\ref{NewtonYScheme}) with $p_i$ chosen such that $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, for some $\beta > 1$, and with $s_i = 1$. By our definition of $\bm{F}_{p,[m]} (\bm{u}, \bm{y}, \bm{x})$ and the fact that $\bm{F}_{p_i,[m]} (u_{p_i} (\bm{w}_i), \bm{0}, \bm{w}_i) = \bm{0}$, we have that 
\begin{align}
\nabla \bm{h} (\bm{w}_i) \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) = - \bm{h} (\bm{w}_i)
\end{align}
and
\begin{align}
\bm{g} \left(\bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \right) = \bm{0}
\ \ \ \ \Longleftrightarrow \ \ \ \ 
\bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \in \Omega.
\label{NewtonYThm.4.1.0}
\end{align}
Hence, the vector 
$\begin{bmatrix} \bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i), \ \bm{0} \end{bmatrix}^{\intercal}$ satisfies the constraints of the minimization problem in (\ref{NewtonYScheme}). Thus, the objective value of problem (\ref{NewtonYScheme}) at a solution, $\bm{w}_{i+1}$, is bounded above by the objective evaluated at $\begin{bmatrix} \bm{w}_i + \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i), \ \bm{0} \end{bmatrix}^{\intercal}$. Using this fact with the definition of $\eta$ and inequality (\ref{NewtonYThm.4}) we have that
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \|^2 + \| \bm{y}_{i+1} \|^2 
&\leq \| \bm{M}(\bm{w}_i) \bm{u}_{p_i} (\bm{w}_i) \|^2
\leq \eta^2 \| \bm{u}_{p_i} (\bm{w}_i) \|^2
%\leq \eta^2 \sigma^2 \left\| \begin{bmatrix}
%\bm{h} \left( \bm{w}_i \right) \\
%\bm{g} \left( \bm{w}_i \right)
%\end{bmatrix} \right\|
\leq \eta^2 \sigma^2 \left\| \bm{h}(\bm{w}_i) \right\|^2. \label{NewtonYThm.4.1.1}
\end{align}
In particular, recalling that $\alpha_i := 1 - \| \bm{y}_i \|$, it follows from (\ref{NewtonYThm.4.1.1}) that
\begin{align}
1 - \eta \sigma \| \bm{h} (\bm{w}_i) \| \leq \alpha_{i+1}. \label{NewtonYThm.4.1.2}
\end{align}

Now suppose that $\bm{w}_i, \bm{w}_{i+1} \in \mathcal{B}$ where $\bm{w}_{i+1}$ is generated using the scheme in (\ref{NewtonYScheme}) with $p_i$ chosen such that $p_i \geq \max \left\{ \beta^2, \| \bm{h} (\bm{w}_i) \|^{-2} \right\}$, for some $\beta > 1$, and with $s_i = 1$. In particular, since $\bm{w}_i$ is known at the time of choosing $p_i$ we can take
\begin{align}
p_i = \max \left\{ \beta^2, \frac{1}{\| \bm{h}(\bm{w}_i) \|^2} \right\} \label{NewtonYThm.4.2}
\end{align}
for some $\beta \geq 1$ to satisfy this requirement. By Taylor's Theorem and the problem constraint, we have that 
\begin{align}
\bm{h}(\bm{w}_{i+1}) &= \bm{h} (\bm{w}_i) + \nabla \bm{h} (\bm{w}_i) (\bm{w}_{i+1} - \bm{w}_i) + \frac{1}{2} \sum_{j = 1}^{\ell} ( \bm{w}_{i+1} - \bm{w}_i )^{\intercal} \nabla^2 \bm{h}_j (\bm{\xi}_j) ( \bm{w}_{i+1} - \bm{w}_i ) \bm{e}_j, \\
&= - \frac{1}{\sqrt{p_i}} \bm{y}_{i+1} + \frac{1}{2} \sum_{j = 1}^{\ell} ( \bm{w}_{i+1} - \bm{w}_i )^{\intercal} \nabla^2 \bm{h}_j (\bm{\xi}_j) ( \bm{w}_{i+1} - \bm{w}_i ) \bm{e}_j,
\end{align}
for some vectors $\bm{\xi}_j$ between $\bm{w}_i$ and $\bm{w}_{i+1}$, for $1 \leq j \leq \ell$. This yields the inequality
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \frac{1}{\sqrt{p_i}} \| \bm{y}_{i+1} \| + \frac{\delta}{2} \| \bm{w}_{i+1} - \bm{w}_i \|^2. \label{NewtonYThm.5}
\end{align}
Combining (\ref{NewtonYThm.5}) with inequality (\ref{NewtonYThm.4.1.1}) yields
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \frac{ \eta \sigma}{\sqrt{p_i}} \left\| \bm{h}(\bm{w}_i) \right\| + \frac{ \delta \eta^2 \sigma^2}{2} \left\| \bm{h}(\bm{w}_i) \right\|^2. \label{NewtonYThm.6}
\end{align}
By our choice of $p_i$ in (\ref{NewtonYThm.4.2}), we have that $\frac{1}{\sqrt{p_i}} \leq \| \bm{h} (\bm{w}_i) \|$. Combining this with (\ref{NewtonYThm.6}) yields
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| \leq \eta \sigma \left( 1 + \frac{\delta \eta \sigma}{2} \right) \left\| \bm{h}(\bm{w}_i) \right\|^2 = \eta \sigma \gamma \left\| \bm{h}(\bm{w}_i) \right\|^2, \label{NewtonYThm.7}
\end{align}
which concludes the proof of (\ref{NewtonYSchemeThm.3}).

It remains to show that the sequence of iterates $\{ \bm{w}_i \}_{i = 0}^{\infty}$ generated by (\ref{NewtonYScheme}) is contained in the ball $\mathcal{B}$ and that $\alpha_i \geq \alpha$, for all $i \geq 1$. We proceed by way of induction. First, $\bm{w}_0 \in \mathcal{B}$ by definition. Additionally, using (\ref{NewtonYThm.4.1.2}) and (\ref{NewtonYThm.4.1}) we have that
\begin{align}
\alpha_1
\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_0) \|
\geq \alpha.
\end{align} 
Hence, the base case of induction holds. Suppose now that $\bm{w}_0, \bm{w}_1, \ldots, \bm{w}_i$ are contained in $\mathcal{B}$, that $\| \bm{w}_{i} - \bm{w}_{i-1} \| \leq \eta \sigma \| \bm{h}( \bm{w}_0 ) \| 2^{-2^{i-1} + 1}$, and that $s_j = 1$ and $\alpha_{j+1} \geq 0$, for $0 \leq j < i$. As the inequality in (\ref{NewtonYThm.7}) holds for $\bm{w}_0, \bm{w}_1, \ldots, \bm{w}_i$ by the inductive hypothesis, repeated applications of (\ref{NewtonYThm.7}) yield
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \| &\leq \eta \sigma \left\| \bm{h}(\bm{w}_i) \right\| \leq \frac{1}{\gamma} \left( \eta \sigma \gamma \| \bm{h}( \bm{w}_0 ) \| \right)^{2^i} = \eta \sigma \| \bm{h}( \bm{w}_0 ) \| \left( \eta \sigma \gamma \| \bm{h}( \bm{w}_0 ) \| \right)^{2^i - 1}. \label{NewtonYThm.8}
\end{align}
By our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}), it follows from (\ref{NewtonYThm.8}) that
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_i \| &\leq \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\| 2^{-2^i + 1}, \label{NewtonYThm.8.1}
\end{align}
as desired. Next, observe that (\ref{NewtonYSchemeThm.1}) follows from applying (\ref{NewtonYThm.8.1}), the inductive hypothesis, and the triangle inequality
\begin{align}
\| \bm{w}_{i+1} - \bm{w}_0 \| = \| \bm{w}_{i+1} - \bm{w}_i + \bm{w}_i - \bm{w}_0 \| &\leq \| \bm{w}_{i+1} - \bm{w}_i \| + \| \bm{w}_{i} - \bm{w}_0 \| \\
&\leq \sum_{j = 0}^{i} \| \bm{w}_{j+1} - \bm{w}_j \| \\
&\leq \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\| \sum_{j = 0}^{i} 2^{-2^j + 1} \\
&< 2 \eta \sigma \left\| \bm{h}(\bm{w}_0) \right\|.
\end{align}
Additionally, observe that
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| &\leq \eta \sigma \| \bm{h}(\bm{w}_i) \|^2 \leq \left( \eta \sigma \| \bm{h}(\bm{w}_0) \| \right)^{2^i} \| \bm{h}(\bm{w}_i) \| \leq \left( 1 - \tau \right) \| \bm{h}(\bm{w}_i) \|, \label{NewtonYThm.9}
\end{align}
where the final inequality holds from our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}). By our choice of $\bm{w}_0$ in (\ref{NewtonYThm.4.1}), we have that
\begin{align}
\eta \sigma \| \bm{h} (\bm{w}_0) \| 2^{-2^i + 1} \leq 1 - \alpha, \label{NewtonYThm.9.1}
\end{align}
for all $i \geq 0$. Hence,
\begin{align}
\alpha_{i+1} 
&\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_i) \| \tag{Using (\ref{NewtonYThm.4.1.2})} \\
&\geq 1 - \eta \sigma \| \bm{h} (\bm{w}_0) \| 2^{-2^i + 1} \tag{Using (\ref{NewtonYThm.8})} \\
&\geq \alpha, \tag{Using (\ref{NewtonYThm.9.1})}
\end{align}
as desired. As $\alpha_{i+1} \leq 1$ by definition, we have $\alpha_{i+1} \in [\alpha, 1]$. Hence, $1 - \tau \leq 1 - \tau \alpha_i \leq 1 - \tau \alpha$. Combining this with (\ref{NewtonYThm.9}) yields that the Armijo line search update in (\ref{NewtonArmijo}) is satisfied for $s_i = 1$. This concludes the inductive phase of the proof.

Lastly, as $1 - \tau \leq 1 - \tau \alpha$ we have that
\begin{align}
\| \bm{h}(\bm{w}_{i+1}) \| 
&\leq \left( 1 - \tau \alpha \right) \| \bm{h}(\bm{w}_i) \|, \label{NewtonYThm.10}
\end{align}
holds for all $i \geq 0$. Hence the sequence $\{ \bm{w}_i \}_{i = 0}^{\infty}$ is Cauchy so there exists a vector $\bm{w}^* \in \mathcal{B}$ such that $\bm{w}_i \to \bm{w}^*$ as $i \to \infty$ which, combined with (\ref{NewtonYThm.9}), yields the inequality in (\ref{NewtonYSchemeThm.2}). Lastly, as $\tau \in (0,1)$, it follows from (\ref{NewtonYThm.10}) that $\| \bm{h} (\bm{w}^*) \| = 0$. As $\bm{g}(\bm{w}_i) = \bm{0}$ for all $i \geq 0$, we conclude that (\ref{NewtonYSchemeThm.0}) holds.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
We now provide two remarks on the proof of Theorem~\ref{NewtonYSchemeThm}. First, note that we can use the abstract convergence theorem (by Hager [\textcolor{red}{SOURCE}]) to prove the inequality in (\ref{NewtonYThm.4}). For convenience, this result is stated in the appendix as Theorem~\ref{AbstractConvThm}. Here, we take the following values for parameters and functions in the Theorem~\ref{AbstractConvThm}:
\begin{align*}
&\bm{\theta} = [ \bm{u}_p (\bm{x}), \bm{y}_p (\bm{x})], \\
&\bm{\theta}^* = [ \bm{u}_p (\bm{x}^*), \bm{y}_p (\bm{x}^*)] = [\bm{0}, \bm{0}], \\
&\bm{\delta} = \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}) - \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}^*), \\
&\mathcal{T} (\bm{\theta}) = \bm{F}_p (\bm{\theta}, \bm{x}^*), \\
&\mathcal{L} = \nabla_{\theta} \mathcal{T} (\bm{\theta}^*) = \nabla_{[u,y]} \bm{F}_p ([\bm{u}_p (\bm{x}^*), \bm{y}_p (\bm{x}^*)], \bm{x}^*) = \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*), \\
&\mathcal{F} (\bm{\theta}) = \bm{0}. \\
\end{align*}
With these choices, we have that
\begin{align*}
\mathcal{T} (\bm{\theta}^*) + \bm{\delta} = \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) + \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) - \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) = \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) = \begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix}
\end{align*}
Hence, condition (C1) in Theorem~\ref{AbstractConvThm}, given by $\mathcal{T} (\bm{\theta}^*) + \bm{\delta} \in \mathcal{F} (\bm{\theta}^*)$, is equivalent to 
\begin{align*}
\begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix} = \bm{0}.
\end{align*}
This statement enforces the requirement that $\bm{x}$ is a feasible point for problem (\ref{NewtonYScheme}). Next, observe that 
\begin{align*}
\nabla \mathcal{T}(\bm{\theta}) - \mathcal{L} &= \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}) - \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*) \\
&= \left[
\begin{array}{c|c}
\multirow{2}{*}{$M(\bm{x})^{\intercal} M(\bm{x})$} & \frac{1}{\sqrt{p}} I_m \\
 & \bm{0} \\
\hline
\bm{0} & I_m
\end{array}
\right] - \left[
\begin{array}{c|c}
\multirow{2}{*}{$M(\bm{x}^*)^{\intercal} M(\bm{x}^*)$} & \frac{1}{\sqrt{p}} I_m \\
 & \bm{0} \\
\hline
\bm{0} & I_m
\end{array}
\right] \\
&= \left[
\begin{array}{c|c}
M(\bm{x})^{\intercal} M(\bm{x}) - M(\bm{x}^*)^{\intercal} M(\bm{x}^*) & \bm{0} \\
\hline
\bm{0} & \bm{0}
\end{array}
\right].
\end{align*}
Hence, condition (C2) in Theorem~\ref{AbstractConvThm}, given by $\| \nabla \mathcal{T}(\bm{\theta}) - \mathcal{L} \| \leq \varepsilon$ for all $\bm{\theta} \in B(\bm{\theta}^*,r)$, is equivalent to
\begin{align*}
\| M(\bm{x})^{\intercal} M(\bm{x}) - M(\bm{x}^*)^{\intercal} M(\bm{x}^*) \| \leq \varepsilon,
\end{align*}
for all $\bm{x} \in B(\bm{x}^*,r)$. As $\bm{h}, \bm{g} \in \mathcal{C}^2$, we have that $M(\bm{x})^{\intercal} M(\bm{x})$ is a continuous function. Hence, there exists a $r > 0$ such that (C2) is satisfied. Finally, observe that
\begin{align*}
(\mathcal{F} - \mathcal{L})^{-1} = (\bm{0} - \nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*))^{-1} = - (\nabla_{[u,y]} \bm{F}_p (\bm{0}, \bm{0}, \bm{x}^*))^{-1}.
\end{align*}
Based on our analysis in the proof of Theorem~\ref{NewtonYSchemeThm}, we have that $(\mathcal{F} - \mathcal{L})^{-1}$ is Lipschitz continuous with a uniformly bounded Lipschitz constant for sufficiently large values of $p$. Hence, condition (C3) from Theorem~\ref{AbstractConvThm} holds. Lastly, it requires to choose $\varepsilon > 0$ small enough and $p$ sufficiently large such that $\gamma \varepsilon < 1$. Once this choice has been made all hypotheses are satisfied for Theorem~\ref{AbstractConvThm} and we obtain the result that
\begin{align*}
\| \bm{\theta} - \bm{\theta}^* \| \leq \frac{\gamma}{1 - \gamma \varepsilon} \| \bm{\delta} \|,
\end{align*}
which in our case is equivalent to
\begin{align*}
\| \bm{u}_p (\bm{x}) \| \leq \frac{\gamma}{1 - \gamma \varepsilon} \| \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}) - \bm{F}_p ([\bm{0}, \bm{0}], \bm{x}^*) \| = \frac{\gamma}{1 - \gamma \varepsilon} \left\| \begin{bmatrix}
\bm{h} (\bm{x}) \\
\bm{g} (\bm{x})
\end{bmatrix} \right\|,
\end{align*}
for all $\bm{x} \in B(\bm{x}^*,r)$. This is the desired result that is used in the proof of Theorem~\ref{NewtonYSchemeThm}.

As an additional remark, note that the constant appearing in (\ref{NewtonYThm.7}) can be made slightly different provided that $\bm{y}_{i, \infty} = \bm{0}$ for all $i \geq 1$. This follows from first observing that
\begin{align}
\bm{y}_{i+1} - \bm{y}_{i+1, \infty} &= - \bm{h}(\bm{w}_i) - \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1} - \bm{w}_i) + \bm{h}(\bm{w}_i) + \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1, \infty} - \bm{w}_i) \nonumber \\
&= \nabla \bm{h}(\bm{w}_i) ( \bm{w}_{i+1, \infty} - \bm{w}_{i+1} ). \nonumber 
\end{align}
As $\| \bm{w}_{i+1, \infty} - \bm{w}_{i+1} \| = O (1/p_i)$ from Theorem~\ref{thm:feasibility-detection}, we have that $\| \bm{y}_{i+1} - \bm{y}_{i+1, \infty} \| = O (1/p_i)$. By our hypothesis that $\bm{y}_{i+1, \infty} = 0$ it follows that $\| \bm{y}_{i+1} \| = O (1/p_i)$ which, by our choice of $p_i$, yields 
\begin{align}
\| \bm{y}_{i+1} \| = O \left( \left\| \bm{h}( \bm{w}_i) \right\|^2 \right). \label{NewtonYRemark.1}
\end{align}
Combining (\ref{NewtonYThm.6}) and (\ref{NewtonYRemark.1}) yields a slightly different constant.
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ----------------------- MULTIPLIER STEP ANALYSIS ---------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Convergence Analysis for Multiplier Step} \label{subsec:multiplier-step-analysis} 
We now work towards establishing local convergence for the multiplier step in the CMS algorithm. Before stating and proving the local convergence result for the multiplier step, we require seceral results that willbe used in the proof. First, we restate Theorem 3.1 from \cite{Hager1993} in terms of our current analysis. Note that there are no changes to the details of the result and the same proof from \cite{Hager1993} holds. As such, the proof is omitted here. %% NOTE: This result actually uses LICQ instead of LI like the old result. However, based on our analysis for Theorem 4.1 the idea used there can be carried over to the original proof of THeorem 4.2. 

\begin{theorem} \label{Theorem3.1}
Suppose $\bm{x}^*$ satisfies $\bm{h}(\bm{x}^*) = \bm{0}$ and $\bm{g}(\bm{x}^*) = \bm{0}$, $\bm{g}, \bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and %$\nabla h_j (\bm{z}^*)$ and $\nabla g_j (\bm{z}^*)$ are linearly independent. 
assumptions (\textbf{LICQ}) and (\textbf{SOSC}) hold.
Then there exists a neighborhood $\mathcal{N}$ about $(\bm{x}^*, \bm{\lambda}^*)$ for which the problem 
\begin{align}
\min \left\{ \mathcal{L}_{p_i}(\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{u}_i) (\bm{z} - \bm{u}_i) = \bm{0}, \bm{z} \in \Omega \right\}
\end{align}
has a local minimizer $\bm{z} = \bm{z}_{i+1}$, whenever $(\bm{u}_i, \bm{\nu}_i) \in \mathcal{N}$. Moreover, there exists a constant $c \in \mathbb{R}$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{\nu}_i - \bm{\lambda}^* \|^2 + c \| \bm{u}_i - \bm{x}^* \|^2 + c \| \bm{h}(\bm{u}_i) \|,
\end{align} 
for every $(\bm{u}_i, \bm{\nu}_i) \in \mathcal{N}$ with $\bm{u}_i \in \Omega$.
\end{theorem}

Next, we restate Corollary 3.1 from \cite{Hager1993} in terms of our current analysis (note that there are no changes to the details of the result and the same proof from \cite{Hager1993} holds).

\begin{corollary} \label{Corollary3.1}
Suppose $\bm{x}^*$ satisfies $\bm{h} (\bm{x}^*) = \bm{0}$ and $\bm{g} (\bm{x}^*) = \bm{0}$, $\bm{g}, \bm{h} \in \mathcal{C}^2$ near $\bm{x}^*$, and 
%the rows of the matrix $[\nabla h (\bm{z}^*)^{\intercal} \ A^{\intercal}]^{\intercal}$ are linearly independent. 
assumptions (\textbf{LICQ}) and (\textbf{SOSC}) hold.
Then there exists a neighborhood $\mathcal{N}$ about $(\bm{x}^*, \bm{\lambda}^*)$ for which the problem 
\begin{align}
\min \left\{ \mathcal{L}_{p_i}(\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{u}_i) (\bm{z} - \bm{u}_i) = \bm{0}, \bm{z} \in \Omega \right\}
\end{align}
has a local minimizer $\bm{z} = \bm{z}_{i+1}$, whenever $(\bm{x}_k, \bm{\nu}_i) \in \mathcal{N}$, $\bm{x}_k \in \Omega$, and any $\bm{u}_i = \bm{w}_j$ for any $j \geq 1$, where $\bm{w}_j$ are generated by the scheme in (\ref{NewtonYScheme}) starting from $\bm{w}_0 = \bm{x}_k$. Moreover, there exists a constant $c \in \mathbb{R}$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{\nu}_i - \bm{\lambda}^* \|^2 + c \| \bm{x}_k - \bm{x}^* \|^2,
\end{align} 
where $c$ is independent of $(\bm{x}_k, \bm{\nu}_i) \in \mathcal{N} \cap \left( \Omega \times \mathbb{R}^m \right)$.
\end{corollary}
\iffalse
\begin{proof}
As $\bm{h} (\bm{x}^*) = \bm{0}$ we have that
\begin{align}
\| \bm{h}(\bm{x}_k)  \| = \| \bm{h}(\bm{x}_k) - \bm{h}(\bm{x}^*) \| = \| \nabla \bm{h}(\bm{\xi}) (\bm{x}_k - \bm{x}^*) \| \leq c \| \bm{x}_k - \bm{x}^* \|, \label{Corollary.1}
\end{align}
where $\bm{\xi}$ is some vector between $\bm{x}_k$ and $\bm{x}^*$. Using (\ref{NewtonYSchemeThm.1}) from Theorem~\ref{NewtonYSchemeThm} with $\bm{w}_0 = \bm{x}_k$, we have that $\| \bm{w}_j - \bm{x}_k \| \leq c \| \bm{h}(\bm{x}_k) \|$, for all $j \geq 1$. As $\bm{u}_i = \bm{w}_j$ for some $1 \leq j \leq i_C$, it follows that $\| \bm{u}_i - \bm{x}_k \| \leq c \| \bm{h}(\bm{x}_k) \|$. Combining this with (\ref{Corollary.1}) and the triangle inequality yields
\begin{align*}
\| \bm{u}_i - \bm{x}^* \| 
&\leq \| \bm{u}_i - \bm{x}_k \| + \| \bm{x}_k - \bm{x}^* \| 
\leq c \| \bm{x}_k - \bm{x}^* \|.
\end{align*}
Lastly, (\ref{NewtonYSchemeThm.3}) from Theorem~\ref{NewtonYSchemeThm} with $\bm{w}_0 = \bm{x}_k$ yields that $\| \bm{h}(\bm{u}_i) \| \leq c \| \bm{h}(\bm{x}_k) \|^2$ which combined with (\ref{Corollary.1}) yields that $\| \bm{h}(\bm{u}_i) \| \leq c \| \bm{x}_k - \bm{x}^* \|^2$. Making these substitutions into Theorem~\ref{Theorem3.1} concludes the proof.
\end{proof}
\fi

In order to prove the local convergence result for the multiplier step, we make use of the following problem:
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x} \in \mathbb{R}^{n}} & f(\bm{x}) \\
\text{s.t.} & \bm{h}(\bm{x}) = \bm{u}, \ \ \bm{r} (\bm{x}) \leq \bm{0},
\end{array} \label{prob:Ru}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{x}} & f(\bm{x}) \\
\text{s.t.} & \bm{h} (\bm{x}) = \bm{u}, \ \ \bm{g} (\bm{x}) = \bm{0},
\end{array} \label{prob:Gu}
\end{align}
and
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
where $\bm{u}$ is a fixed vector in $\mathbb{R}^m$. Note that (\ref{prob:Ru}) is very similar to problem (\ref{prob:main-nlp}) with the only difference being the perturbation applied to the nonlinear portion of the constraint set, namely changing $\bm{h} (\bm{x}) = \bm{0}$ to $\bm{h} (\bm{x}) = \bm{u}$. Lemma~\ref{lem:Lem13.1} will provide insight into how close a solution of problem (\ref{prob:Ru}) is to a solution of (\ref{prob:main-nlp}) for different values of $\bm{u}$ by performing stability analysis of problem (\ref{prob:Ru}) for values of $\bm{u}$ in a neighborhood of $\bm{u} = \bm{0}$. We note that Lemma~\ref{lem:Lem13.1} has the same conclusions as Lemma 13.1 from \cite{Hager1993}, however, the difference here being that the hypotheses are more general. This is accomplished by making use of strong regularity as discussed by Robinson in \cite{Robinson1980}. This difference will allow us to clearly justify alternate sets of assumptions when establishing convergence results for the multiplier step of NPASA. 

\begin{lemma} \label{lem:Lem13.1}
Suppose that $f, \bm{h}$ from problem (\ref{prob:main-nlp}) are twice continuously differentiable and that %the KKT system for problem (\ref{prob:Ru}) is strongly regular at a KKT point $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. 
either assumptions (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Then there exists a neighborhood $\mathcal{N}$ of $\bm{0}$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Ru}) has a local minimizer $\bm{x}(\bm{u})$ and associated multipliers $\bm{\lambda} (\bm{u})$ and $\bm{\mu} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.1}.1)] $\begin{pmatrix} \bm{x}(\bm{0}), \ \bm{\lambda} (\bm{0}), \ \bm{\mu} (\bm{0}) \end{pmatrix} = \left( \bm{x}^*, \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:Lem13.1}.2)] $\begin{pmatrix} \bm{x}(\bm{u}), \ \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Ru}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{x}(\bm{0}), \ \bm{\lambda} (\bm{0}), \ \bm{\mu} (\bm{0}) \end{pmatrix} = \left( \bm{x}^*, \bm{\lambda}^*, \bm{\mu}^* \right),\label{lem:Lem13.1.1} \\
&\begin{pmatrix} \bm{x}(\bm{u}), \ \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}) \end{pmatrix} \ \text{satisfies the KKT system for problem (\ref{prob:Ru})}. \label{lem:Lem13.1.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.1}.3)] $\displaystyle \left\| \left(
\bm{x} (\bm{u}_1), \bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1) 
\right) - \left(
\bm{x} (\bm{u}_2), \bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{x} (\bm{u}_1), \bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1) 
\right) - \left(
\bm{x} (\bm{u}_2), \bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|. \label{lem:Lem13.1.3}
\end{align}
\end{lemma}
\begin{proof}
We first establish that the KKT system for problem (\ref{prob:main-nlp}) is strongly regular at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. In Section 4 of \cite{Robinson1980}, Robinson outlines conditions under which the KKT system for a nonlinear program is strongly regular. One set of assumptions that guarantees a strongly regular KKT system for problem (\ref{prob:main-nlp}) at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is that (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}) hold at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Additionally, Theorem 4.1 of \cite{Robinson1980} proves that if assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) hold at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ then this guarantees strong regularity for the KKT system in (\ref{prob:main-nlp}). Under either set of hypotheses for our lemma, we have that the KKT system for problem (\ref{prob:main-nlp}) is strongly regular at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. We now prove the lemma using some results from \cite{Robinson1980}.

Now denote the Lagrangian of problem (\ref{prob:Ru}) by
\begin{align}
\mathcal{L} (\bm{u}; \bm{x}, \bm{\lambda}, \bm{\mu}) = f (\bm{x}) + \bm{\lambda}^{\intercal} \left( \bm{h} (\bm{x}) - \bm{u} \right) + \bm{\mu}^{\intercal} \bm{r} (\bm{x}). \label{eq:KKTStability.0}
\end{align}
Using $\bm{f}(\cdot)$ in this proof in the context of \cite{Robinson1980}, we define 
\begin{align}
\bm{f} (\bm{u}, \bm{x}, \bm{\lambda}, \bm{\mu}) 
:= \begin{bmatrix}
\nabla_x \mathcal{L} (\bm{x}, \bm{\lambda}, \bm{\mu}) \\
%- \bm{r} (\bm{x}) \\
- \bm{r} (\bm{x}) \\
- \bm{h} (\bm{x}) + \bm{u}
\end{bmatrix}. \label{eq:KKTStability.1}
\end{align}
By the hypotheses of our lemma, we have that the hypotheses of Theorem 2.1 of \cite{Robinson1980} are satisfied. To apply Corollary 2.2 from \cite{Robinson1980}, it remains to show that there exists a constant $\nu$ such that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{x}, \bm{\lambda}, \bm{\mu}) - \bm{f} (\bm{u}_2, \bm{x}, \bm{\lambda}, \bm{\mu}) \| \leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:KKTStability.2}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{x}, \bm{\lambda}, \bm{\mu}) \in V$, where $V$ is a closed neighborhood of $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Noting that
\begin{align}
\nabla_x \mathcal{L} (\bm{u}; \bm{x}, \bm{\lambda}, \bm{\mu})^{\intercal} = \nabla_x f (\bm{x})^{\intercal} + \nabla_x \bm{h} (\bm{x})^{\intercal} \bm{\lambda} + \nabla_x \bm{r} (\bm{x})^{\intercal} \bm{\mu} \label{eq:KKTStability.3}
\end{align}
it follows that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{x}, \bm{\lambda}, \bm{\mu}) - \bm{f} (\bm{u}_2, \bm{x}, \bm{\lambda}, \bm{\mu}) \| 
= \left\| \begin{bmatrix}
\bm{0} \\
\bm{0} \\
\bm{u}_1 - \bm{u}_2 
\end{bmatrix} \right\|
= \left\| \bm{u}_1 - \bm{u}_2 \right\|, \label{eq:KKTStability.4}
\end{align}
which concludes the proof.
\end{proof}

%In Section 4 of \cite{Robinson1980}, Robinson outlines sufficient conditions under which the KKT system for a nonlinear program is strongly regular. One set of assumptions that guarantees a strongly regular KKT system is (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}). Additionally, Theorem 4.1 of \cite{Robinson1980} proves that assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) guarantee strong regularity for the KKT system in a nonlinear program.

Next, we consider the problem where we %choose $j \in \{0,1\}$ and 
fix a vector $\bm{u}$ then solve
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{\lambda}, \bm{\mu}} & E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) \\
\text{s.t.} & \bm{\mu} \geq \bm{0}.
\end{array} \label{prob:Mu}
\end{align}
For this problem, we have a stability result that follows from an application of Corollary 2.2 in \cite{Robinson1980}.
\begin{lemma} \label{lem:Lem13.2}
%Let $j \in \{0,1\}$. 
Suppose that $f, \bm{h}$ from problem (\ref{prob:main-nlp}) are continuously differentiable, $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}), and that (\textbf{LI}) holds at $\bm{x}^*$. %, and that $E_{m,j} (\bm{u}, \bm{\lambda}, \bm{\mu})$ is twice continuously differentiable with respect to $\bm{\lambda}$ and $\bm{\mu}$ in a neighborhood of $(\bm{\lambda}^*, \bm{\mu}^*)$. 
Then there exists a neighborhood $\mathcal{N}$ of $\bm{x}^*$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Mu}) has a local minimizer $(\bm{\lambda} (\bm{u}), \bm{\mu} (\bm{u}))$ and associated multiplier $\bm{\alpha} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.2}.1)] $\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:Lem13.2}.2)] $\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Mu}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right), \label{lem:Lem13.2.1} \\
&\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}  \ \text{satisfies the KKT system for problem (\ref{prob:Mu})}. \label{lem:Lem13.2.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:Lem13.2}.3)] $\displaystyle \left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|. \label{lem:Lem13.2.3}
\end{align}
\end{lemma}
\begin{proof}
Denote the Lagrangian for problem (\ref{prob:Mu}) by
\begin{align}
\mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) = E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) - \bm{\mu}^{\intercal} \bm{\alpha}. \label{eq:EMStability.0.0}
\end{align}
As in the proof of Lemma~\ref{lem:Lem13.1}, we first establish that the KKT system for problem (\ref{prob:Mu}) is strongly regular at $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$ under the given hypotheses. Using (\ref{eq:EMStability.0.0}) we have that the hessian of the Lagrangian for problem (\ref{prob:Mu}) is given by $\nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) = B (\bm{u})^{\intercal} B (\bm{u})$, where $B (\bm{u})$ is the matrix defined by
\begin{align}
B (\bm{u})
&:= \begin{bmatrix}
\ \nabla_x \bm{h} (\bm{u})^{\intercal} &\vert& \nabla_x \bm{r} (\bm{u})^{\intercal} \
\end{bmatrix}. \label{eq:EmDiscussion.1}
\end{align}
Hence, for every vector $\bm{v} = [\bm{\lambda}, \bm{\mu}]^{\intercal}$ with $\bm{v} \neq \bm{0}$ we have
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{u}) \bm{v} \right\|^2
\geq 0. \label{eq:EmDiscussion.2}
\end{align}
So we have that the hessian of the Lagrangian for problem (\ref{prob:Mu}) is positive semidefinite. Under our hypothesis that (\textbf{LI}) holds at $\bm{x}^*$, we have that $B (\bm{x}^*)$ is of full column rank yielding that $B (\bm{x}^*)^{\intercal} B (\bm{x}^*)$ is nonsingular. As such, there exists a constant $\sigma > 0$ such that
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{x}^*; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{x}^*) \bm{v} \right\|^2
> \sigma. \label{eq:EmDiscussion.3}
\end{align}
So we have positive definiteness of the hessian under assumption (\textbf{LI}). As (\ref{prob:Mu}) only has bound constraints, the gradients of the active constraints are linearly independent. Thus, under the assumption that (\textbf{LI}) holds at $\bm{x}^*$ the KKT system in problem (\ref{prob:Mu}) satisfies the strong regularity condition from \cite{Robinson1980}.

Now define $\bm{f} (\bm{u}, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) := \begin{bmatrix}
\nabla_{[\lambda, \mu]} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \\
\bm{\mu}
\end{bmatrix}$, where $\bm{f}(\cdot)$ is used in this proof in the context of \cite{Robinson1980}. By our hypotheses, we have that the hypotheses of Theorem 2.1 of \cite{Robinson1980} are satisfied. To apply Corollary 2.2 from \cite{Robinson1980}, it remains to show that there exists a constant $\nu$ such that
\begin{align}
\| \bm{f} (\bm{u}_1, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) - \bm{f} (\bm{u}_2, \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \| \leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.0}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$, where $V$ is a closed neighborhood of $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$. To this end, observe that
\begin{align}
\nabla_{\lambda} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal}
&= \nabla \bm{h} (\bm{u}) \nabla f (\bm{u})^{\intercal} + \nabla \bm{h} (\bm{u}) \nabla \bm{h} (\bm{u})^{\intercal} \bm{\lambda} + \nabla \bm{h} (\bm{u}) \nabla \bm{r} (\bm{u})^{\intercal} \bm{\mu}. \label{eq:EMStability.1}
\end{align}
Hence,
\begin{align}
\| \nabla_{\lambda} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\lambda} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \| \nabla \bm{h} (\bm{u}_1) \nabla f (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla f (\bm{u}_2)^{\intercal} \| \nonumber \\
&\quad + \| \nabla \bm{h} (\bm{u}_1) \nabla \bm{h} (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla \bm{h} (\bm{u}_2)^{\intercal} \| \| \bm{\lambda} \| \nonumber \\
&\quad + \| \nabla \bm{h} (\bm{u}_1) \nabla \bm{r} (\bm{u}_1)^{\intercal} - \nabla \bm{h} (\bm{u}_2) \nabla \bm{r} (\bm{u}_2)^{\intercal} \| \| \bm{\mu} \|. \label{eq:EMStability.2}
\end{align}
As $(\bm{\lambda}, \bm{\mu}, \bm{\alpha})$ is in a closed neighborhood $V$ of $(\bm{\lambda}^*, \bm{\mu}^*, \bm{\alpha}^*)$, there exist constants $c_1$ and $c_2$ such that $\| \bm{\lambda} \| \leq c_1$ and $\| \bm{\mu} \| \leq c_2$ for all $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. As $f, \bm{h}, \bm{r} \in \mathcal{C}^1$, the functions $\nabla \bm{h} (\cdot) \nabla f (\cdot)^{\intercal}$, $\nabla \bm{h} (\cdot) \nabla \bm{h} (\cdot)^{\intercal}$, and $\nabla \bm{h} (\cdot) \nabla \bm{r} (\cdot)^{\intercal}$ are Lipschitz continuous on $\mathcal{N}$. Combining these facts with (\ref{eq:EMStability.2}) yields that there exists a constant $\nu$ such that
\begin{align}
\| \nabla_{\lambda} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\lambda} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.3}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. Next, observe that
\begin{align}
\nabla_{\mu} \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal}
&= \nabla \bm{r} (\bm{u}) \nabla f (\bm{u})^{\intercal} + \nabla \bm{r} (\bm{u}) \nabla \bm{h} (\bm{u})^{\intercal} \bm{\lambda} + \nabla \bm{r} (\bm{u}) \nabla \bm{r} (\bm{u})^{\intercal} \bm{\mu} - \bm{r} (\bm{u}) - \bm{\alpha}. \label{eq:EMStability.4}
\end{align}
Hence,
\begin{align}
\| \nabla_{\mu} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\mu} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \| \nabla \bm{r} (\bm{u}_1) \nabla f (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla f (\bm{u}_2)^{\intercal} \| \nonumber \\
&\quad + \| \nabla \bm{r} (\bm{u}_1) \nabla \bm{h} (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla \bm{h} (\bm{u}_2)^{\intercal} \| \| \bm{\lambda} \| \nonumber \\
&\quad + \| \nabla \bm{r} (\bm{u}_1) \nabla \bm{r} (\bm{u}_1)^{\intercal} - \nabla \bm{r} (\bm{u}_2) \nabla \bm{r} (\bm{u}_2)^{\intercal} \| \| \bm{\mu} \| \nonumber \\
&\quad + \| \bm{r} (\bm{u}_1) - \bm{r} (\bm{u}_2) \|. \label{eq:EMStability.5}
\end{align}
By an argument similar to the one establishing (\ref{eq:EMStability.3}), there exists a constant $\nu$ such that
\begin{align}
\| \nabla_{\mu} \mathcal{L} (\bm{u}_1; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} - \nabla_{\mu} \mathcal{L} (\bm{u}_2; \bm{\lambda}, \bm{\mu}, \bm{\alpha})^{\intercal} \|
&\leq \nu \| \bm{u}_1 - \bm{u}_2 \|, \label{eq:EMStability.6}
\end{align}
for all $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$ and $(\bm{\lambda}, \bm{\mu}, \bm{\alpha}) \in V$. Now combining (\ref{eq:EMStability.3}) and (\ref{eq:EMStability.6}) yields (\ref{eq:EMStability.0}). Corollary 2.2 from \cite{Robinson1980} can now be applied to conclude the proof.
\end{proof}

We now make a comment on what can be said on the stability of problem (\ref{prob:Mu}) if $E_{m,0}$ is replaced with $E_{m,1}$. To this end, we note that $E_{m,1} (\bm{u}, \bm{\lambda}, \bm{\mu})$ must be twice continuously differentiable with respect to $\bm{\lambda}$ and $\bm{\mu}$ in a neighborhood of a solution $(\bm{\lambda}^*, \bm{\mu}^*)$ to establish a satibility result similar to Lemma~\ref{lem:Lem13.2}. We can guarantee this holds provided that the hypotheses of Lemma~\ref{lem:E1diff} are satisfied, that is, in addition to the hypotheses of Lemma~\ref{lem:Lem13.2} we require that assumption (\textbf{SCS}) holds at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. This result is much more restrictive as it would limit future analysis to only nondegenerate stationary points of problem (\ref{prob:main-nlp}). As such, this provides some motivation behind the choice of minimizing $E_{m,0}$ with respect to $\bm{\lambda}$ and $\bm{\mu}$ instead of $E_{m,1}$ in the Multiplier Step of NPASA. We note that the additional minization of $E_{m,1}$ with respect to $\bm{\mu}$ in the Multiplier Step is required in order to ensure fast local convergence of the Multiplier Step in the CMS algorithm as will be illustrated in the proof of Theorem~\ref{ConvergenceResult}.

It should be noted that we can slightly modify problem (\ref{prob:Mu}) to ensure positive definiteness and avoid the requirement that (\textbf{LI}) holds. This can be done by fixing a constant $\gamma > 0$ and slightly augmenting the objective function to obtain
\begin{align}
\begin{array}{cc}
\displaystyle \min_{\bm{\lambda}, \bm{\mu}} & E_{m,0} (\bm{u}, \bm{\lambda}, \bm{\mu}) + \gamma \left\| [\bm{\lambda}, \bm{\mu}] \right\|^2 \\
\text{s.t.} & \bm{\mu} \geq \bm{0}.
\end{array} \label{prob:Mu-gamma}
\end{align}
Under this modification, for every vector $\bm{v} = [\bm{\lambda}, \bm{\mu}]^{\intercal}$ with $\bm{v} \neq \bm{0}$ we have
\begin{align}
\bm{v}^{\intercal} \nabla^2 \mathcal{L} (\bm{u}; \bm{\lambda}, \bm{\mu}, \bm{\alpha}) \bm{v}
&= \left\| B (\bm{u}) \bm{v} \right\|^2 + \gamma \| \bm{v} \|^2
> 0. \label{eq:PostEmDiscussion.1}
\end{align} 
Hence, the hessian of the Lagrangian for (\ref{prob:Mu-gamma}) is positive definite. As (\ref{prob:Mu-gamma}) has the same constraints as (\ref{prob:Mu}), the gradients of the active constraints are linearly independent. Thus, the KKT system in problem (\ref{prob:Mu-gamma}) always satisfies the strong regularity condition from \cite{Robinson1980}. With this established, we now state the following result that follows from the same argument in Lemma~\ref{lem:Lem13.2} but is applied to problem (\ref{prob:Mu-gamma}).

\begin{lemma} \label{lem:AltLem13.2}
Suppose that $f, \bm{h} \in \mathcal{C}^1$ and that $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}). Then there exists a neighborhood $\mathcal{N}$ of $\bm{x}^*$ such that, for every $\bm{u} \in \mathcal{N}$, problem (\ref{prob:Mu-gamma}) has a local minimizer $(\bm{\lambda} (\bm{u}), \bm{\mu} (\bm{u}))$ and associated multiplier $\bm{\alpha} (\bm{u})$ satisfying
\iffalse
\begin{itemize}
\item[(\ref{lem:AltLem13.2}.1)] $\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right)$.
\item[(\ref{lem:AltLem13.2}.2)] $\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix}$ satisfies the KKT system for problem (\ref{prob:Mu-gamma}).
\end{itemize}
\fi
\begin{align}
&\begin{pmatrix} \bm{\lambda} (\bm{x}^*), \ \bm{\mu} (\bm{x}^*) \end{pmatrix} = \left( \bm{\lambda}^*, \bm{\mu}^* \right), \label{lem:AltLem13.2.1} \\
&\begin{pmatrix} \bm{\lambda} (\bm{u}), \ \bm{\mu} (\bm{u}), \ \bm{\alpha} (\bm{u}) \end{pmatrix} \ \text{satisfies the KKT system for problem (\ref{prob:Mu-gamma})}. \label{lem:AltLem13.2.2}
\end{align}
Additionally, there exists a constant $c \in \mathbb{R}$ such that, for every $\bm{u}_1, \bm{u}_2 \in \mathcal{N}$, we have
\iffalse
\begin{itemize}
\item[(\ref{lem:AltLem13.2}.3)] $\displaystyle \left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \|$.
\end{itemize}
\fi
\begin{align}
\left\| \left(
\bm{\lambda} (\bm{u}_1), \bm{\mu} (\bm{u}_1), \bm{\alpha} (\bm{u}_1)
\right) - \left(
\bm{\lambda} (\bm{u}_2), \bm{\mu} (\bm{u}_2), \bm{\alpha} (\bm{u}_2)
\right) \right\| \leq c \| \bm{u}_1 - \bm{u}_2 \| \label{lem:AltLem13.2.3}
\end{align}
\end{lemma}

%%%%%%%% (Following result is not true since it is missing constraint)
\iffalse
We now provide one final result that will be useful in establishing local convergence of the multiplier step of NPASA.

\begin{lemma} \label{lem:DualStep}
Suppose $f, \bm{h}, \bm{r} \in \mathcal{C}^1$ and let $\{ \bm{z}_i \}_{i = 1}^{\infty}$ be the sequence of primal variables generated by the miltiplier step of NPASA in Algorithm~\ref{alg:npasa}. Then
\begin{align}
\min_{\bm{\mu} \geq \bm{0}, \bm{\lambda}} E_m (\bm{z}_{i+1}, \bm{\lambda}, \bm{\mu}) 
= 0
%\leq \| \bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i) \|^2
, \label{result:DualStep}
\end{align}
for all $i \geq 1$.
\end{lemma}
\begin{proof}
By the KKT conditions for the primal step, there exists a vector $\bm{\alpha}_{i+1} \geq \bm{0}$ such that
\begin{align*}
\nabla f (\bm{z}_{i+1}) + \left( \bm{\lambda}_i + 2 q_i (\bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i)) \right)^{\intercal} \nabla \bm{h} (\bm{z}_{i+1}) + \bm{\alpha}_{i+1}^{\intercal} A = \bm{0}
\end{align*}
and $\bm{\alpha}_{i+1}^{\intercal} \bm{r} (\bm{z}_{i+1}) = 0$. Hence,
\begin{align}
\min_{\bm{\mu} \geq \bm{0}, \bm{\lambda}} E_m (\bm{z}_{i+1}, \bm{\lambda}, \bm{\mu})
&\leq E_m (\bm{z}_{i+1}, \bm{\lambda}_i + 2 q_i (\bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i)), \bm{\alpha}_{i+1}) = 0, \label{eq:DualStep.1}
\end{align}
which concludes the proof.
%As $\| \bm{h} (\bm{z}_{i+1}) - \bm{h} (\bm{z}_i) \|^2 \geq 0$, the result (\ref{result:DualStep}) now follows from (\ref{eq:DualStep.1}).
\end{proof}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

With these lemmas in place, we are now ready to state and prove a convergence result for the multiplier step of NPASA, found in Algorithm~\ref{alg:cms}. This result is a modified version of Theorem 4.1 in \cite{Hager1993} accounting for the updates made to the algorithm. While there are many required updates to the proof, we note that some details of the proof are essentially the same as in the proof of Theorem 4.1 in \cite{Hager1993} but are included here for completeness. %Additionally, note that the iterative scheme in (\ref{scheme:MS1}) -- (\ref{scheme:MS3}) is the same update provided in the CMS pseudocode, Algorithm~\ref{alg:cms}, so the following result applies to the Algorithm~\ref{alg:cms}.

\begin{theorem} \label{ConvergenceResult}
Suppose that $f, \bm{h} \in \mathcal{C}^2$ and that either assumptions (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. %If $p_k$ is chosen such that $p_k \geq 1$ and $\frac{1}{p_k} \leq \| h (\bm{x}_k) \|^2$ for all $k \geq 0$ then 
Then there exists a neighborhood $\mathcal{N}_1$ and $\mathcal{N}_2$ of $\bm{x}^*$ and a constant $c$ such that, for every $\bm{z}_0 \in \mathcal{N}_1 \cap \Omega$, the primal variables and equality multipliers, $(\bm{z}, \bm{\nu})$, generated using the scheme
\begin{align}
%(\bm{\nu}_i, \bm{\eta}_i) &\in \arg\min \left\{ E_{m,0} ( \bm{z}_i, \bm{\nu}, \bm{\eta}) : \bm{\eta} \geq \bm{0} \right\} \label{scheme:MS1} \\
(\bm{\nu}_i, \bm{\eta}_i) &\in \arg\min \left\{ E_{m,0} ( \bm{z}_i, \bm{\nu}, \bm{\eta}) + \gamma \left\| [\bm{\lambda}, \bm{\mu}] \right\|^2 : \bm{\eta} \geq \bm{0} \right\} \label{scheme:MS1} \\
\bm{\eta}_i' &\in \arg\min \left\{ E_{m,1} ( \bm{z}_i, \bm{\nu}_i, \bm{\eta}) : \bm{\eta} \geq \bm{0} \right\} \label{scheme:MS2} \\
\bm{z}_{i+1} &= \arg \min \left\{ \mathcal{L}_{p_i}^i (\bm{z}, \bm{\nu}_i) : \nabla \bm{h} (\bm{z}_i) (\bm{z} - \bm{z}_i) = 0, \bm{z} \in \mathcal{N}_2 \cap \Omega \right\} \label{scheme:MS3}
\end{align}
%in the multiplier step of NPASA 
converge to a point $( \bm{z}^*, \bm{\nu}^* )$ and
\iffalse
\begin{itemize}
\item[(\ref{ConvergenceResult}.0)] $\displaystyle \min_{\bm{\eta} \geq \bm{0}} E_{m,1} ( \bm{z}^*, \bm{\nu}^*, \bm{\eta} ) = 0$.
\end{itemize}
\fi
\begin{align}
\min_{\bm{\eta} \geq \bm{0}} E_{m,1} ( \bm{z}^*, \bm{\nu}^*, \bm{\eta} ) = 0. \label{ConvergenceResult.0}
\end{align}
Furthermore, the following properties hold for $i \geq 0$:
\iffalse
\begin{itemize}
\item[(\ref{ConvergenceResult}.1)] $\| \bm{z}_i - \bm{z}^* \| \leq c 2^{-2^i}$.
\item[(\ref{ConvergenceResult}.2)] $\| \bm{z}_{i+1} - \bm{z}_1 \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2$.
\item[(\ref{ConvergenceResult}.3)] $\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| h (\bm{z}_0) \|$.
\item[(\ref{ConvergenceResult}.4)] $E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2$.
\item[(\ref{ConvergenceResult}.5)] $E_1 \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \leq \| \bm{z}_i - \bm{x}^* \|$.
%\item[(\ref{ConvergenceResult}.6)] $\displaystyle \lim_{i \to \infty} E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) = 0$.
\end{itemize}
\fi
\begin{align}
&\| \bm{z}_i - \bm{z}^* \| \leq c 2^{-2^i}, \label{ConvergenceResult.1} \\
&\| \bm{z}_{i+1} - \bm{z}_1 \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2, \label{ConvergenceResult.2} \\
&\| \bm{z}_{i+1} - \bm{x}^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| h (\bm{z}_0) \|, \label{ConvergenceResult.3} \\
&E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2, \label{ConvergenceResult.4} \\
&E_1 \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \leq \| \bm{z}_i - \bm{x}^* \|. \label{ConvergenceResult.5}
%\lim_{i \to \infty} E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) &= 0. \label{ConvergenceResult.6}
\end{align}
\end{theorem}

Before providing the proof for this theorem, we note that the iterative scheme in (\ref{scheme:MS1}) -- (\ref{scheme:MS3}) is the same update provided in the CMS pseudocode, Algorithm~\ref{alg:cms}, without checking for a sufficient decrease in the error estimator at each iteration. %that would result in reusing the same multipliers at the next iteration. 
As a result, it follows from (\ref{ConvergenceResult.4}) that the criterion $E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq \delta E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)$ in the Multiplier Step of the CMS algorithm will always be satisfied under the hypotheses of Theorem~\ref{ConvergenceResult} for $i$ sufficiently large. Hence, this local convergence result can be applied to the Multiplier step of the CMS algorithm without modification. We now provide a proof for Theorem~\ref{ConvergenceResult}.
\fi

\begin{proof}[Proof of Theorem~\ref{ConvergenceResult}]
We will perform our analysis of this method by considering the perturbed problem (\ref{prob:Ru}). As problem (\ref{prob:main-nlp}) is equivalent to problem (\ref{prob:Ru}) with $\bm{u} = \bm{0}$, we have that $\bm{x}^*$ is a solution of problem (\ref{prob:Ru}) with $\bm{u} = \bm{0}$. Additionally, we will let $\bm{z}_i^*$ denote the local minimizer of (\ref{prob:Ru}) with $\bm{u} = \bm{h}(\bm{z}_i)$ and $( \bm{\nu}_i^*, \bm{\eta}_i^* )$ be corresponding multipliers for which $E_{m,1} \left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right) = 0$. To justify the existence of $( \bm{\nu}_i^*, \bm{\eta}_i^* )$, observe that the Lagrangian for problem (\ref{prob:Ru}) with $\bm{u} = \bm{h}(\bm{z}_i)$ is 
\begin{align}
f(\bm{x}) + \bm{\lambda}^{\intercal} \left( \bm{h}(\bm{x}) - \bm{h}(\bm{z}_i) \right) + \bm{\mu}^{\intercal} \bm{r} (\bm{x})
\end{align} 
which has gradient 
\begin{align}
\nabla f(\bm{x}) + \bm{\lambda}^{\intercal} \nabla \bm{h}(\bm{x}) + \bm{\mu}^{\intercal} \nabla \bm{r} (\bm{x}).
\end{align}
As this gradient is the same as the gradient of the Lagrangian for problem (\ref{prob:main-nlp}), we have that a KKT point $\left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right)$ for problem (\ref{prob:Ru}) satisfies $E_{m,1} \left( \bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^* \right) = 0$, as desired.

\iffalse % No longer necessary for analysis (keeping for now in case it comes up later)
Finally, we define 
\begin{align*}
\bm{y}_k^* = - \bm{h}(\bm{x}_k) - \nabla \bm{h}(\bm{x}_k) (\bm{x}_k^* - \bm{x}_k).
\end{align*}
\fi

Suppose that $\bm{z}_i$ is near $\bm{x}^*$. %By Lemma 13.1 in \cite{Hager1993} with $\bm{u} = \bm{h} (\bm{x}_k)$, we have that
By (\ref{lem:Lem13.1.1}) in Lemma~\ref{lem:Lem13.1}, we have $\bm{x} (\bm{h} (\bm{z}_i)) = \bm{z}_i^*$ and $\bm{x} (\bm{h} (\bm{x}^*)) = \bm{x}^*$. Hence, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_i)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*) = \bm{0}$, it follows that
\begin{align}
\| \bm{z}_i^* - \bm{x}^* \| \leq c \| \bm{h}( \bm{z}_i ) - \bm{h}(\bm{x}^*) \| = c \| \bm{h}( \bm{z}_i ) \|.
\end{align} 
Since $\| \bm{h}(\bm{z}_i) \| \to 0$ as $\bm{z}_i \to \bm{x}^*$, we have that $\bm{z}_i^*$ is near $\bm{x}^*$ when $\bm{z}_i$ is near $\bm{x}^*$. As $\bm{x} = \bm{z}_i$ satisfies the constraint $\bm{h} (\bm{x}) = \bm{u}$ when $\bm{u} = \bm{h} (\bm{z}_i)$, it follows from Theorem~\ref{Theorem3.1} that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| &\leq c \| \bm{\nu}_i - \bm{\nu}_i^* \|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2 + c \| \bm{h} (\bm{z}_i) - \bm{h} (\bm{z}_i) \| \\
&= c \| \bm{\nu}_i - \bm{\nu}_i^* \|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2 \\
&\leq c \left\| \begin{bmatrix} \bm{\nu}_i, \ \bm{\eta}_i \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2, \label{NPASA8.1}
\end{align}
for some constant $c$. As a note of interest to the reader, observe that the penalized Lagrangian function for problem (\ref{prob:Ru}) is given by
\begin{align}
\mathcal{L}_{p} (\bm{\nu}, \bm{z}) = f(\bm{z}) + \bm{\nu}^{\intercal} \bm{h} (\bm{z}) + p \| \bm{h} (\bm{z}) - \bm{u} \|^2.
\end{align}
Hence, when we take $\bm{u} = \bm{h} (\bm{z}_i)$ we have that the penalized Lagrangian function for problem (\ref{prob:Ru}) is equal to $\mathcal{L}_{p}^i (\bm{\nu}, \bm{z})$.
%
\iffalse % No longer needed since corollary covers this part
Next, observe that
\begin{align}
\| \bm{z}_k - \bm{x}_k^* \|^2 &= \| \bm{z}_k - \bm{x}_k + \bm{x}_k - \bm{x}_k^* \|^2 \nonumber \\
&\leq \| \bm{z}_k - \bm{x}_k \|^2 + 2 \left| \langle \bm{z}_k - \bm{x}_k, \bm{x}_k - \bm{x}_k^* \rangle \right| + \| \bm{x}_k - \bm{x}_k^* \|^2 \nonumber \\
&\leq 2 \| \bm{z}_k - \bm{x}_k \|^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2 \label{NPASA8.1.1} \\
&\leq 2 \left( c_1 \| h (\bm{x}_k) \| \right)^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2 \label{NPASA8.1.2} \\
&= 2 c_1^2 \| h (\bm{x}_k) \|^2 + 2 \| \bm{x}_k - \bm{x}_k^* \|^2, \label{NPASA8.2}
\end{align}
where (\ref{NPASA8.1.1}) follows from Cauchy and (\ref{NPASA8.1.2}) follows from Theorem~\ref{NewtonYSchemeThm} with $\bm{z}_0 = \bm{x}_k$. Combining (\ref{NPASA8.1}) and (\ref{NPASA8.2}) yields
\begin{align}
\| \bm{x}_{k+1} - \bm{x}_k^* \| \leq c \| [\bm{\lambda}_k \ \bm{\mu}_k] - [\bm{\lambda}_k^* \ \bm{\mu}_k^*] \|^2 + c \| \bm{x}_k - \bm{x}_k^* \|^2 + c \| h (\bm{x}_k) \|^2. \label{NPASA8.2.1}
\end{align}
\fi
%
%Next, by either assumptions (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}) or assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) we have that the hypotheses of Lemma~\ref{lem:Lem13.2} are satisfied. Hence, 
As the hypotheses of Lemma~\ref{lem:AltLem13.2} are satisfied,
it follows from (\ref{lem:AltLem13.2.3}) in Lemma~\ref{lem:AltLem13.2} with $\bm{u}_1 = \bm{z}_i$ and $\bm{u}_2 = \bm{z}_i^*$ that 
\begin{align}
\left\| \begin{bmatrix} \bm{\nu}_i, \ \bm{\eta}_i \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| = O \left( \| \bm{z}_i - \bm{z}_i^* \| \right). \label{NPASA8.3}
\end{align}
Similarly, $\left\| \begin{bmatrix} \bm{\nu}_{i+1}, \ \bm{\eta}_{i+1} \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| = O \left( \| \bm{z}_{i+1} - \bm{z}_i^* \| \right)$ follows from an additional application of (\ref{lem:AltLem13.2.3}) in Lemma~\ref{lem:AltLem13.2}. Now (\ref{NPASA8.1}) and (\ref{NPASA8.3}) together imply that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| + \left\| \begin{bmatrix} \bm{\nu}_{i+1}, \ \bm{\eta}_{i+1} \end{bmatrix} - \begin{bmatrix} \bm{\nu}_i^*, \ \bm{\eta}_i^* \end{bmatrix} \right\| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2. \label{NPASA8.3.1}
\end{align}

By our choice of Problem (\ref{prob:Ru}), for $\bm{u} = \bm{h}(\bm{z}_i)$ we have that $\bm{h}(\bm{z}_i^*) = \bm{h}(\bm{z}_i)$. Hence,
\begin{align}
\| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \| &= \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i^*) \| \leq c \| \bm{z}_{i+1} - \bm{z}_i^* \| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2, \label{NPASA8.10}
\end{align}
where (\ref{NPASA8.10}) follows from performing a first order Taylor expansion of $\bm{h}$ and using (\ref{NPASA8.3.1}). Next, from (\ref{lem:Lem13.1.1}) in Lemma~\ref{lem:Lem13.1} we have that $\bm{x} (\bm{h} (\bm{z}_{i+1})) = \bm{z}_{i+1}^*$ and $\bm{x} (\bm{h} (\bm{z}_i)) = \bm{z}_i^*$. Hence, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_{i+1})$ and $\bm{u}_2 = \bm{h} (\bm{z}_i)$ together with (\ref{NPASA8.10}) yields
\begin{align}
\| \bm{z}_{i+1}^* - \bm{z}_i^* \| &\leq c \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \| \leq c \| \bm{z}_i - \bm{z}_i^* \|^2. \label{NPASA8.11}
\end{align}
Now define
\begin{align}
r_{i+1} := \| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{z}_{i+1}^* - \bm{z}_i^* \|. \label{NPASA8.12}
\end{align}
We claim that $r_{i+1} = O (r_i^2)$. To prove this claim, first note that combining (\ref{NPASA8.3.1}), (\ref{NPASA8.11}), and (\ref{NPASA8.12}) yields
\begin{align}
r_{i+1} \leq c \| \bm{z}_i - \bm{z}_i^* \|. \label{NPASA8.12.1}
\end{align}
By Cauchy, we have
\begin{align}
\| \bm{z}_i - \bm{z}_i^* \| \leq 2 \| \bm{z}_i - \bm{z}_{i-1}^* \|^2 + 2 \| \bm{z}_i^* - \bm{z}_{i-1}^* \|^2 \label{NPASA8.13}
\end{align}
which combined with (\ref{NPASA8.12.1}) yields $r_{i+1} = O (r_i^2)$, as claimed.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% No longer needed since this term doesn't show up in bound but might be useful later
\iffalse 
Additionally, performing a second order Taylor expansion and applying $\nabla \bm{h} (\bm{z}_k) (\bm{x}_{k+1} - \bm{z}_k) = 0$ from the constraint in (A2) yields that
\begin{align}
\| h (\bm{x}_{k+1}) \| &\leq \| h (\bm{z}_k) \| + c \| \bm{x}_{k+1} - \bm{z}_k \|^2 \leq \| h (\bm{z}_k) \| + c \| \bm{x}_{k+1} - \bm{x}_k^* \|^2 + c \| \bm{z}_k - \bm{x}_k^* \|^2 \label{NPASA8.14}
\end{align}
As $\| h (\bm{z}_k) \| \leq c \| h (\bm{x}_k) \|^2$ from (\ref{NewtonYSchemeThm.3}) in Theorem~\ref{NewtonYSchemeThm}, substituting the bounds established in (\ref{NPASA8.2}) and (\ref{NPASA8.3.1}) into (\ref{NPASA8.14}) yields
\begin{align}
\| h (\bm{x}_{k+1}) \| &\leq c \| h (\bm{x}_k) \|^2 + c \| \bm{x}_k - \bm{x}_k^* \|^2 + c \| h (\bm{x}_k) \|^4 + c \| \bm{x}_k - \bm{x}_k^* \|^4. \nonumber
\end{align}
Hence, 
\begin{align}
\| h (\bm{x}_{k+1}) \| = O (\| h (\bm{x}_k) \|^2) + O (\| \bm{x}_k^* - \bm{x}_k \|^2). \label{NPASA8.15}
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
So there exists a constant $\gamma$ such that $r_{i+1} \leq \gamma r_i^2$. Then we have
\begin{align}
r_{i+1} 
&\leq \frac{1}{\gamma} \left( \gamma r_i \right)^2 \leq \ldots \leq \frac{1}{\gamma} \left( \gamma r_1 \right)^{2^i} = r_1 \left( \gamma r_1 \right)^{2^i - 1}.
\end{align}
Now observe that
\begin{align}
r_1
&= \| \bm{z}_1 - \bm{z}_0^* \| + \| \bm{z}_1^* - \bm{z}_0^* \| \nonumber \\
&\leq c \| \bm{z}_0 - \bm{z}_0^* \|^2 \tag{Applying \ref{NPASA8.3.1} and \ref{NPASA8.11}} \\
&\leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| \bm{z}_0^* - \bm{x}^* \|^2. \tag{Applying triangle inequality and Cauchy}
\end{align}
Using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_0)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*)$ it follows that
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \|
&\leq c \| \bm{h} (\bm{z}_0) - \bm{h} (\bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|
\end{align}
which combined with the bound on $r_1$ yields
\begin{align}
r_1 &\leq c \| \bm{z}_0 - \bm{x}^* \|^2. \label{NPASA8.14.4}
\end{align}
It now follows that $r_1 \to 0$ as $\bm{z}_0 \to \bm{x}^*$. Thus, there exists a constant $c$ such that $r_i \leq c r_1 2^{-2^i - 1}$, for all $\bm{z}_0$ sufficiently close to $\bm{x}^*$. It now follows that the sequence $\{ \bm{z}_i \}_{i = 0}^{\infty}$ is Cauchy since
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i \| 
&\leq \| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{z}_i^* - \bm{z}_{i-1}^* \| + \| \bm{z}_i - \bm{z}_{i-1}^* \| \\
&\leq r_{i+1} + r_i \\
&\leq c r_1 2^{-2^i}, \label{NPASA8.15}
\end{align}
for all $i \geq 1$. Thus, $\{ \bm{z}_i \}_{i = 0}^{\infty}$ has a limit, say $\bm{z}^*$, and it follows from (\ref{NPASA8.15}) that $\bm{z}^*$ satisfies
\begin{align}
\| \bm{z}_{i} - \bm{z}^* \| &\leq c 2^{-2^i},
\end{align}
for all $i \geq 0$, hence, establishing (\ref{ConvergenceResult.1}). In particular, note that (\ref{NPASA8.15}) also implies that $\{ \bm{z}_i^* \}_{i = 0}^{\infty}$ converges to $\bm{z}^*$.

Now we claim that $\{ \left[ \bm{\nu}_i, \bm{\eta}_i \right] \}_{i = 0}^{\infty}$ converges to a limit. Let $\varepsilon > 0$ be given. As $\bm{z}_i \to \bm{z}^*$ and $\bm{z}_i^* \to \bm{z}^*$, there exists a $M \geq 0$ such that $\| \bm{z}_i - \bm{z}_i^* \|^2 < \varepsilon$, for all $i \geq M$. Hence, 
\begin{align}
\| [\bm{\nu}_{i+1} \ \bm{\eta}_{i+1}] - [\bm{\nu}_i \ \bm{\eta}_i] \| 
&\leq \| [\bm{\nu}_{i+1} \ \bm{\eta}_{i+1}] - [\bm{\nu}_i^* \ \bm{\eta}_i^*] \| + \| [\bm{\nu}_i \ \bm{\eta}_i] - [\bm{\nu}_i^* \ \bm{\eta}_i^*] \| \\
&\leq c \| \bm{z}_i - \bm{z}_i^* \|^2 + c \| \bm{z}_i - \bm{z}_i^* \|^2 \\
&\leq 2c \varepsilon,
\end{align}
for all $i \geq M$. So $\{ \left[ \bm{\nu}_i, \bm{\eta}_i \right] \}_{i = 0}^{\infty}$ is Cauchy and therefore has a limit, say $\left[ \bm{\nu}^*, \bm{\eta}^* \right]$. Similarly, it follows that $\{ \left[ \bm{\nu}_i^*, \bm{\eta}_i^* \right] \}_{i = 0}^{\infty}$ converges to $\left[ \bm{\nu}^*, \bm{\eta}^* \right]$. As $E_{m,1}$ is continuous, we now have that
\begin{align}
\min_{\bm{\eta} \geq \bm{0}} E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}) 
&\leq E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}^*) 
= \lim_{i \to \infty} E_{m,1} (\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*). \label{NPASA8.15.1}
\end{align}
Since $E_{m,1} (\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*) = 0$ for all $i \geq 0$, it follows that %$E_{m,1} (\bm{z}^*, \bm{\nu}^*, \bm{\eta}^*) = 0$ 
from (\ref{NPASA8.15.1}) that (\ref{ConvergenceResult.0}) holds.

Recalling (\ref{NPASA8.3.1}) and (\ref{NPASA8.11}) it follows that
\begin{align}
r_1 &= \| \bm{z}_{1} - \bm{z}_0^* \| + \| \bm{z}_{1}^* - \bm{z}_0^* \| \leq c \| \bm{z}_{0} - \bm{z}_0^* \|^2 + c \| h (\bm{z}_0) \|^2. \label{NPASA8.16}
\end{align}
Using $\bm{h}(\bm{x}^*) = \bm{0}$ we have that
\begin{align}
\| \bm{h} (\bm{z}_0) \| 
= \| \bm{h}(\bm{z}_0) - \bm{h}(\bm{x}^*) \| 
= \| \nabla \bm{h}(\xi_0) (\bm{z}_0 - \bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|, \label{NPASA8.17}
\end{align}
for some $\bm{\xi}_0$ between $\bm{z}_0$ and $\bm{x}^*$. Also, using (\ref{lem:Lem13.1.3}) in Lemma~\ref{lem:Lem13.1} with $\bm{u}_1 = \bm{h} (\bm{z}_0)$ and $\bm{u}_2 = \bm{h} (\bm{x}^*) = \bm{0}$ together with the fact that $\bm{h} (\bm{z}_0^*) = \bm{h} (\bm{z}_0)$ we have that
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{h}(\bm{z}_0^*) - \bm{h}(\bm{x}^*) \| 
= c \| \bm{h}(\bm{z}_0) - \bm{h}(\bm{x}^*) \| 
\leq c \| \bm{z}_0 - \bm{x}^* \|. \label{NPASA8.17.1}
\end{align}
Hence,
\begin{align}
\| \bm{z}_0 - \bm{z}_0^* \| 
\leq \| \bm{z}_0 - \bm{x}^* \| + \| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{z}_0 - \bm{x}^* \| \label{NPASA8.17.2}
\end{align}
which, when substituted into (\ref{NPASA8.16}) with (\ref{NPASA8.17}), yields
\begin{align}
r_1 &\leq c \| \bm{z}_{0} - \bm{x}^* \|^2. \label{NPASA8.18}
\end{align}
Next, applying the triangle inequality and using (\ref{NPASA8.15}) and (\ref{NPASA8.17}) we find that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_1 \| 
&\leq \sum_{j = 1}^{i} \| \bm{z}_{j+1} - \bm{z}_{j} \| 
\leq c r_1 \sum_{j = 1}^{i} 2^{-2^i} 
\leq c r_1 
\leq c \| \bm{z}_{0} - \bm{x}^* \|^2,
\end{align}
which proves (\ref{ConvergenceResult.2}).

Next, from (\ref{NPASA8.17.1}) we have that 
\begin{align}
\| \bm{z}_0^* - \bm{x}^* \| 
\leq c \| \bm{h}(\bm{z}_0^*) - \bm{h}(\bm{x}^*) \| 
= c \| \bm{h}(\bm{z}_0) \|
\end{align}
and from (\ref{NPASA8.3.1}) and (\ref{NPASA8.17.2}) we have $\| \bm{z}_1 - \bm{z}_0^* \| \leq c \| \bm{z}_0 - \bm{x}^* \|^2$. Using these together with the triangle inequality and (\ref{ConvergenceResult.3}) we have
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| 
&\leq \| \bm{z}_{i+1} - \bm{z}_1 \| + \| \bm{z}_1 - \bm{z}_0^* \| + \| \bm{z}_0^* - \bm{x}^* \|
\leq c \| \bm{z}_0 - \bm{x}^* \|^2 + c \| \bm{h} (\bm{z}_0) \|,
\end{align}
concluding the proof of (\ref{ConvergenceResult.3}).

To prove the remaining parts of the theorem, we proceed by defining
\begin{align}
E_u \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) 
= \sqrt{ \| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{h}(\bm{z}) - \bm{u} \|^2 } \label{def:Eu}
\end{align}
where $\bm{u}$ is a fixed vector and we note that $E_u \in \mathcal{C}^2$ in a neighborhood of $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ by our hypotheses. First, we show that (\ref{ConvergenceResult.4}) holds. As $(\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*)$ is sufficiently close to $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$, by fixing $\bm{\eta} = \bm{\eta}_i^*$ we can apply Lemma 13.2 in \cite{Hager1993} to $E_u \left( \bm{z}, \bm{\nu}, \bm{\eta}_i^* \right)$ with $\bm{u} = \bm{h} (\bm{z}_i)$ to yield that
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| + \| \bm{\nu}_{i+1} - \bm{\nu}_i^* \| 
&\geq c_1 E_u \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \\
&= c_1 \sqrt{ \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|^2 + \| \bm{h}(\bm{z}_{i+1}) - \bm{h}(\bm{z}_i) \|^2 } \\
&\geq c_1 \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|, \label{NPASA8.7}
\end{align}
for some constant $c_1$. From (\ref{lem:Lem13.2.3}) in Lemma~\ref{lem:Lem13.2} with $\bm{u}_1 = \bm{z}_{i+1}$ and $\bm{u}_2 = \bm{z}_i^*$ we have that
\begin{align}
\left\| \bm{\nu}_{i+1} - \bm{\nu}_i^* \right\| = O \left( \| \bm{z}_{i+1} - \bm{z}_i^* \| \right) \label{NPASA8.7.1}
\end{align}
which combined with (\ref{NPASA8.7}) yields
\begin{align}
\| \bm{z}_{i+1} - \bm{z}_i^* \| ^2
&\geq c_1 \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) \|^2. \label{NPASA8.7.2}
\end{align}
Now recall the function $\bm{\Phi} : \mathbb{R}^m \times \mathbb{R}^m \to \mathbb{R}^m$ where the $j$th component of $\bm{\Phi}$ is defined to be $\Phi_j (\bm{a}, \bm{b}) = \min \{ a_j, b_j \}$. As $(\bm{z}_i^*, \bm{\nu}_i^*, \bm{\eta}_i^*)$ is a KKT point for problem (\ref{prob:Ru}), we have that $\eta_{ij}^* r_j (\bm{z}_i^*) = 0$, for $1 \leq j \leq m$. Now fix $j \in \{ 1, 2, \ldots, m \}$. Suppose $\eta_{ij}^* = 0$. As $\bm{r} (\bm{z}_{i+1}) \leq \bm{0}$, we have
\begin{align}
\Phi_j (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \eta_{ij}^*, -r_j (\bm{z}_{i+1}) \}^2
= \min \{ 0, -r_j (\bm{z}_{i+1}) \}^2
= 0. \label{NPASA8.7.3}
\end{align}
On the other hand, suppose $r_j (\bm{z}_i^*) = 0$. As $\bm{r} (\bm{z}) = \bm{A} \bm{z} - \bm{b}$, we have that
\begin{align}
\Phi_j (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \eta_{ij}^*, -r_j (\bm{z}_{i+1}) \}^2 \\
&\leq \left( r_j (\bm{z}_{i+1}) \right)^2 \\
&= \left( r_j (\bm{z}_{i+1}) - r_j (\bm{z}_i^*) \right)^2 \\
&\leq \| \bm{A} \|^2 \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.4}
\end{align}
Combining (\ref{NPASA8.7.3}) and (\ref{NPASA8.7.4}) we have that
\begin{align}
c_1 \| \bm{\Phi} (\bm{\eta}_i^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.5}
\end{align}
Recalling that $E_{m,1} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) = \| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{\Phi} (\bm{\eta}, -\bm{r} (\bm{z})) \|^2$ it follows from (\ref{NPASA8.7.2}) and (\ref{NPASA8.7.5}) that 
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right) 
\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.6}
\end{align}
Recalling (\ref{scheme:MS2}) we have that $\bm{\eta}_{i+1}' \in \arg\min \left\{ E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta} \right) : \bm{\eta} \geq \bm{0} \right\}$. As $\bm{\eta}_{i+1}^* \geq \bm{0}$, it follows from (\ref{NPASA8.7.6}) and (\ref{scheme:MS2}) that
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) 
&\leq c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_i^* \right)
\leq \| \bm{z}_{i+1} - \bm{z}_i^* \|^2. \label{NPASA8.7.8}
\end{align}
Next, applying Theorem~\ref{thm:E1-error-bound} to problem (\ref{prob:Ru}) with $\bm{u} = \bm{h} (\bm{z}_i)$ yields that
\begin{align}
\| \bm{z}_i - \bm{z}_i^* \|^2 
%&\leq c_2 \left( \| \nabla \mathcal{L} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \|^2 + \| \bm{h}(\bm{z}_i) - \bm{h}(\bm{z}_i) \|^2 + \| \bm{\Phi} (\bm{\eta}_i', -\bm{r} (\bm{z}_i)) \|^2 \right) \nonumber \\
&\leq c_2 \left( \| \nabla \mathcal{L} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right) \|^2 + \| \bm{\Phi} (\bm{\eta}_i', -\bm{r} (\bm{z}_i)) \|^2 \right) %\nonumber \\
= c_2 E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right). \label{NPASA8.7.9}
\end{align}
Now combining (\ref{NPASA8.3.1}), (\ref{NPASA8.7.8}), and (\ref{NPASA8.7.9}) yields
\begin{align}
E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right)
&\leq c E_{m,1} \left( \bm{z}_i, \bm{\nu}_i, \bm{\eta}_i' \right)^2, \label{NPASA8.7.10}
\end{align}
which proves (\ref{ConvergenceResult.4}).

Now we show that (\ref{ConvergenceResult.5}) holds. By definition of (\ref{def:Eu}) and the fact that $\bm{h} (\bm{x}^*) = \bm{0}$, note that $E_u \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) = \sqrt{\| \nabla \mathcal{L} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) \|^2 + \| \bm{h} (\bm{z}) \|^2}$ when $\bm{u} = \bm{h}(\bm{x}^*)$. So by fixing $\bm{\eta} = \bm{\mu}^*$ then applying Lemma 13.2 in \cite{Hager1993} to $E_u \left( \bm{z}, \bm{\nu}, \bm{\mu}^* \right)$ with $\bm{u} = \bm{h}(\bm{x}^*)$ we have that there exists a constant $c_1$ such that
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| + \| \bm{\nu}_{i+1} - \bm{\lambda}^* \|
&\geq c_1 E_u \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \\
&= c_1 \sqrt{\| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \|^2 + \| \bm{h} (\bm{z}_{i+1}) \|^2}. \label{NPASA8.8}
\end{align}
From (\ref{lem:AltLem13.2.3}) in Lemma~\ref{lem:AltLem13.2} with $\bm{u}_1 = \bm{z}_{i+1}$ and $\bm{u}_2 = \bm{x}^*$ we have
\begin{align}
\left\| \bm{\nu}_{i+1} - \bm{\lambda}^* \right\| = O \left( \| \bm{z}_{i+1} - \bm{x}^* \| \right) \label{NPASA8.8.1}
\end{align}
which combined with (\ref{NPASA8.8}) yields
\begin{align}
\| \bm{z}_{i+1} - \bm{x}^* \| ^2
&\geq c_1 \left( \| \nabla \mathcal{L} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) \|^2 + \| \bm{h} (\bm{z}_{i+1}) \|^2 \right). \label{NPASA8.8.2}
\end{align}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
Now recall the function $\bm{\Phi} : \mathbb{R}^m \times \mathbb{R}^m \to \mathbb{R}^m$ where the $j$th component of $\bm{\Phi}$ is defined to be $\Phi_j (\bm{a}, \bm{b}) = \min \{ a_j, b_j \}$. As $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ is a KKT point for problem (\ref{prob:main-nlp}), we have that $\mu_j^* r_j (\bm{x}^*) = 0$, for $1 \leq j \leq m$. Now fix $j \in \{ 1, 2, \ldots, m \}$. Suppose $\mu_j^* = 0$. As $\bm{r} (\bm{z}_{i+1}) \leq \bm{0}$, we have
\begin{align}
\Phi_j (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \mu_j^*, -r_j (\bm{z}_{i+1}) \}^2
= \min \{ 0, -r_j (\bm{z}_{i+1}) \}^2
= 0. \label{NPASA8.8.3}
\end{align}
On the other hand, suppose $r_j (\bm{x}^*) = 0$. Then
\begin{align}
\Phi_j (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1}))^2
&= \min \{ \mu_j^*, -r_j (\bm{z}_{i+1}) \}^2 \nonumber \\
&\leq \left( r_j (\bm{z}_{i+1}) \right)^2 \nonumber \\
&= \left( r_j (\bm{z}_{i+1}) - r_j (\bm{x}^*) \right)^2 \nonumber \\
&\leq c \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.4}
\end{align}
Combining (\ref{NPASA8.8.3}) and (\ref{NPASA8.8.4}) we have that there exists a constant $c$ such that
\begin{align}
\| \bm{\Phi} (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq c \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.5}
\end{align}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
By an argument similar to the one establishing (\ref{NPASA8.7.5}), we can show that
\begin{align}
c_1 \| \bm{\Phi} (\bm{\mu}^*, -\bm{r} (\bm{z}_{i+1})) \|^2
&\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.5}
\end{align}
%Recalling that $E_{m,1} \left( \bm{x}, \bm{\lambda}, \bm{\mu} \right) = \| \nabla \mathcal{L} \left( \bm{x}, \bm{\lambda}, \bm{\mu} \right) \|^2 + \| \bm{\Phi} (\bm{\mu}, -\bm{r} (\bm{x})) \|^2$ 
It now follows from (\ref{NPASA8.8.2}) and (\ref{NPASA8.8.5}) that 
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right) 
\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.6}
\end{align}
As $\bm{\mu}^* \geq \bm{0}$, using the definition of $\bm{\eta}_{i+1}'$ in (\ref{scheme:MS2}) with (\ref{NPASA8.8.6}) we now have
\begin{align}
c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) 
&\leq c_1 E_{m,1} \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\mu}^* \right)
\leq \| \bm{z}_{i+1} - \bm{x}^* \|^2. \label{NPASA8.8.8}
\end{align}
Finally, recalling that $E_1 \left( \bm{z}, \bm{\nu}, \bm{\eta} \right)^2 = E_{m,1} \left( \bm{z}, \bm{\nu}, \bm{\eta} \right) + \| \bm{h} (\bm{z}) \|^2$ it follows from (\ref{NPASA8.8.2}) and (\ref{NPASA8.8.8}) that
\begin{align}
E_1 \left( \bm{z}_{i+1}, \bm{\nu}_{i+1}, \bm{\eta}_{i+1}' \right) \leq c \| \bm{z}_{i+1} - \bm{x}^* \|, \label{NPASA8.8.9}
\end{align}
which concludes the proof of (\ref{ConvergenceResult.5}).
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% ------------------------ CMS: LOCAL CONVERGENCE ----------------------- %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Local Convergence of Phase Two of NPASA} \label{subsec:npasa-phase-two-local-conv}
Now that we have established local convergence results for the constraint and multiplier step problems, we are ready to provide a local convergence result for phase two of NPASA. Phase two of NPASA is comprised of the CMS algorithm, Algorithm~\ref{alg:cms}, and branching criterion. We note that (\ref{cor:PhaseTwoConvergence.0}) and its proof are similar to Corollary 5.1 and its proof from \cite{Hager1993}.

\begin{corollary} \label{cor:PhaseTwoConvergence}
Suppose $f, \bm{h} \in \mathcal{C}^2$ and that either assumptions (\textbf{LICQ}), (\textbf{SCS}), and (\textbf{SOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$ or assumptions (\textbf{LICQ}) and (\textbf{SSOSC}) are satisfied at $(\bm{x}^*, \bm{\lambda}^*, \bm{\mu}^*)$. Then there exists a neighborhood $\mathcal{N}_1$ of $\bm{x}^*$ and a constant $c$ such that, for every $\bm{x}_0 \in \mathcal{N}_1 \cap \Omega$ and every $k \geq 0$, the iterates of phase two of NPASA satisfy
\iffalse
\begin{itemize}
\item[(\ref{cor:PhaseTwoConvergence}.0)] $\| \bm{x}_{k+1} - \bm{x}^* \| \leq c \| \bm{x}_{k} - \bm{x}^* \|^2$,
\item[(\ref{cor:PhaseTwoConvergence}.1)] $E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) \leq c E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2$.
\end{itemize}
\fi
\begin{align}
    &\| \bm{x}_{k+1} - \bm{x}^* \| \leq c \| \bm{x}_{k} - \bm{x}^* \|^2, \label{cor:PhaseTwoConvergence.0} \\
    &E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) \leq c E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2. \label{cor:PhaseTwoConvergence.1}
\end{align}
\end{corollary}

\begin{proof}
The proof of (\ref{cor:PhaseTwoConvergence.0}) follows from applying Theorems~\ref{NewtonYSchemeThm} and~\ref{ConvergenceResult}. Observe that
\begin{align}
\| \bm{x}_{k+1} - \bm{x}^* \| 
&\leq c \| \bm{w} - \bm{x}^* \|^2 + c \| \bm{h} (\bm{w}) \| \tag{Applying \ref{ConvergenceResult.3}} \\
&\leq c \| \bm{w} - \bm{x}^* \|^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Applying \ref{NewtonYSchemeThm.3}} \\
&\leq c \left( \| \bm{w} - \bm{x}_k \| + \| \bm{x}_k - \bm{x}^* \| \right)^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Using triangle inequality} \\
&\leq c \left( \| \bm{h} (\bm{x}_k) \| + \| \bm{x}_k - \bm{x}^* \| \right)^2 + c \| \bm{h} (\bm{x}_{k}) \|^2 \tag{Applying \ref{NewtonYSchemeThm.1}} \\
&\leq \frac{5c}{2} \| \bm{h} (\bm{x}_k) \|^2 + \frac{3c}{2} \| \bm{x}_k - \bm{x}^* \|^2. \tag{Using Cauchy inequality}
\end{align}
By performing a first-order Taylor expansion of $\bm{h} (\bm{x})$ and using the fact that $\bm{h} (\bm{x}^*) = \bm{0}$, there exists some $\bm{\xi}_k$ between $\bm{x}_k$ and $\bm{x}^*$ such that $\bm{h} (\bm{x}_k) = \nabla \bm{h} (\bm{\xi}_k) (\bm{x}_k - \bm{x}^*)$. Hence, $\| \bm{h} (\bm{x}_k) \| \leq c \| \bm{x}_k - \bm{x}^* \|$. Making this substitution into our previous inequality yields
\begin{align}
\| \bm{x}_{k+1} - \bm{x}^* \| 
&\leq \frac{5c^2}{2} \| \bm{x}_k - \bm{x}^* \|^2 + \frac{3c}{2} \| \bm{x}_k - \bm{x}^* \|^2 
= C \| \bm{x}_k - \bm{x}^* \|^2,
\end{align}
which proves (\ref{cor:PhaseTwoConvergence.0}).

To prove (\ref{cor:PhaseTwoConvergence.1}), we use (\ref{ConvergenceResult.5}), (\ref{cor:PhaseTwoConvergence.0}), and Theorem~\ref{thm:E1-error-bound}. Observe that
\begin{align}
E_1 \left( \bm{x}_{k+1}, \bm{\lambda}_{k+1}, \bm{\mu}_{k+1} \right) 
&\leq C \| \bm{x}_{k+1} - \bm{x}^* \| \tag{Applying \ref{ConvergenceResult.5}} \\
&\leq C \| \bm{x}_k - \bm{x}^* \|^2 \tag{Applying \ref{cor:PhaseTwoConvergence.0}} \\
&\leq C E_1 \left( \bm{x}_k, \bm{\lambda}_k, \bm{\mu}_k \right)^2, \tag{Applying Theorem~\ref{thm:E1-error-bound}}
\end{align}
which concludes the proof.
\end{proof}
